Block Decomposable Methods for Large-Scale Optimization Problems

This dissertation explores block decomposable methods for large-scale optimization problems. It focuses on alternating direction method of multipliers (ADMM) schemes and block coordinate descent (BCD) methods. Specifically, it introduces a new proximal ADMM algorithm and proposes two BCD methods. The first part of the research presents a new proximal ADMM algorithm. This method is adaptive to all problem parameters and solves the proximal augmented Lagrangian (AL) subproblem inexactly. This adaptiveness facilitates the highly efficient application of the algorithm to a broad swath of practical problems. The inexact solution of the proximal AL subproblem overcomes many key challenges in the practical applications of ADMM. The resultant algorithm obtains an approximate solution of an optimization problem in a number of iterations that matches the state-of-the-art complexity for the class of proximal ADMM schemes. The second part of the research focuses on an inexact proximal mapping for the class of block proximal gradient methods. Key properties of this operator is established, facilitating the derivation of convergence rates for the proposed algorithm. Under two error decreases conditions, the algorithm matches the convergence rate of its exactly computed counterpart. Numerical results demonstrate the superior performance of the algorithm under a dynamic error regime over a fixed one. The dissertation concludes by providing convergence guarantees for the randomized BCD method applied to a broad class of functions, known as H\"older smooth functions. Convergence rates are derived for non-convex, convex, and strongly convex functions. These convergence rates match those furnished in the existing literature for the Lipschtiz smooth setting.

==> data/ADMM/P1-Table4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Iteration limiti: 500,000
% Absolute error: 10^{-10}



\begin{table}[htb!]
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{cccccccccccccc}
\toprule
& & \multicolumn{6}{c}{Iteration} & \multicolumn{6}{c}{Time (ms)}  \\
\cmidrule(lr){3-8} \cmidrule(lr){9-14}
$n$ & $\omega$ & AD & DP1 & DP2 & SD1 & SD2 & SD3 & AD & DP1 & DP2 & SD1 & SD2 & SD3 \\
\midrule
10 & $10^{1}$ & \textbf{18} & 76 & 83 & 427 & 223 & 976 & \textbf{1.592} & 5.402 & 4.291 & 28.192 & 13.881 & 60.184  \\
10 & $10^{3}$ & \textbf{34} & 228 & 232 & 569 & 399 & 1855 & \textbf{2.259} & 11.752 & 11.858 & 65.049 & 30.209 & 119.417  \\
10 & $10^{5}$ & \textbf{50} & 385 & 385 & * & 581 & 2778 & \textbf{3.228} & 13.374 & 13.004 & * & 35.368 & 168.964  \\
10 & $10^{7}$ & \textbf{66} & 541 & 537 & * & * & 3701 & \textbf{4.419} & 18.706 & 18.363 & * & * & 239.235  \\
10 & $10^{9}$ & \textbf{81} & 697 & 689 & * & * & 4625 & \textbf{5.866} & 24.540 & 24.237 & * & * & 323.790  \\
20 & $10^{1}$ & \textbf{22} & 62 & 68 & 433 & 298 & 1261 & \textbf{1.538} & 2.520 & 2.484 & 27.928 & 19.164 & 80.375  \\
20 & $10^{3}$ & \textbf{44} & 166 & 171 & * & 498 & 2304 & \textbf{2.560} & 6.484 & 6.153 & * & 31.821 & 152.866  \\
20 & $10^{5}$ & \textbf{65} & 273 & 275 & * & 700 & 3347 & \textbf{4.213} & 10.548 & 9.879 & * & 45.812 & 223.235  \\
20 & $10^{7}$ & \textbf{84} & 379 & 379 & * & * & 4383 & \textbf{4.684} & 13.961 & 14.009 & * & * & 290.884  \\
20 & $10^{9}$ & \textbf{103} & 485 & 483 & * & * & 5418 & \textbf{5.629} & 17.635 & 17.393 & * & * & 365.368  \\
100 & $10^{1}$ & \textbf{20} & 40 & 46 & * & 433 & 6231 & 2.072 & \textbf{1.820} & 1.831 & * & 28.705 & 420.276  \\
100 & $10^{3}$ & \textbf{33} & 78 & 77 & * & 695 & 9444 & \textbf{2.132} & 3.013 & 2.871 & * & 44.640 & 617.636  \\
100 & $10^{5}$ & \textbf{45} & 116 & 107 & * & * & 12664 & \textbf{3.148} & 4.545 & 4.041 & * & * & 898.522  \\
100 & $10^{7}$ & \textbf{57} & 155 & 137 & * & * & 15876 & \textbf{3.736} & 5.844 & 5.465 & * & * & 1051.830  \\
100 & $10^{9}$ & \textbf{68} & 193 & 167 & * & * & 19087 & \textbf{4.841} & 7.629 & 6.436 & * & * & 1267.924  \\
5000 & $10^{1}$ & \textbf{25} & 121 & 125 & * & 646 & 2257 & \textbf{13.733} & 26.455 & 27.511 & * & 206.646 & 861.279  \\
5000 & $10^{3}$ & \textbf{37} & 221 & 223 & * & 851 & 3324 & \textbf{20.084} & 52.456 & 50.828 & * & 282.999 & 1264.225  \\
5000 & $10^{5}$ & \textbf{49} & 321 & 321 & * & * & 4390 & \textbf{27.591} & 72.829 & 72.810 & * & * & 1692.375  \\
5000 & $10^{7}$ & \textbf{61} & 422 & 419 & * & * & 5449 & \textbf{32.080} & 96.010 & 97.450 & * & * & 1968.163  \\
5000 & $10^{9}$ & \textbf{72} & 522 & 517 & * & * & 6507 & \textbf{41.682} & 118.872 & 118.632 & * & * & 2440.377\\
\hline\multicolumn{14}{l}{\footnotesize\textit{Bolded values equal to the best algorithm according to iteration count or time.}}\\ 
\multicolumn{14}{l}{\footnotesize\textit{* indicates the algorithm failed to find a  stationary point meeting the tolerances by the 500,000th iteration.}}\\
\bottomrule
\end{tabular}}
\caption{Performance for all algorithms applied to the DQP problem \eqref{eq:num.problem1}, with $B=3$, $C=1$ and $\alpha=10^{-2}$ for different pair of values $(n,\omega)$. The iteration and time columns record the number of iterations and time in seconds to find a $(10^{-5},10^{-5})$-stationary point.}\label{tab:numeric.table1}
\end{table}

==> data/ADMM/P2-Table4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Relative error: rho=eta=10^{-5}
% Iteration Limit: 500,000
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[htb!]
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{cccccccccccccc}
\toprule
& & \multicolumn{6}{c}{Iteration} & \multicolumn{6}{c}{Time (sec)}  \\
\cmidrule(lr){3-8} \cmidrule(lr){9-14}
$B$ & $m$ & AD1 & AD2 & AD3 & DP1 & DP2 & DP3 & AD1 & AD2 & AD3 & DP1 & DP2 & DP3  \\
\midrule
10 & 1 & 44 & \textbf{23} & 33 & 3554 & 3560 & 3532 & 0.067 & 0.010 & \textbf{0.008} & 0.296 & 0.286 & 0.275  \\
10 & 2 & 23 & \textbf{19} & 37 & 1355 & 1282 & 1395 & 0.025 & \textbf{0.005} & 0.007 & 0.128 & 0.111 & 0.116  \\
10 & 5 & \textbf{1280} & 2421 & 1469 & * & * & * & \textbf{0.162} & 0.287 & 0.171 & * & * & *  \\
20 & 1 & \textbf{23} & 30 & 30 & 803 & 296 & 417 & 0.021 & 0.009 & \textbf{0.008} & 0.148 & 0.052 & 0.075  \\
20 & 2 & 87 & \textbf{44} & 89 & 297 & 2233 & * & 0.032 & \textbf{0.014} & 0.026 & 0.063 & 0.441 & *  \\
20 & 5 & 147 & 144 & \textbf{114} & 1862 & 6210 & * & 0.036 & 0.034 & \textbf{0.027} & 0.333 & 1.088 & *  \\
20 & 10 & 682 & 1105 & \textbf{550} & 847 & * & * & 0.168 & 0.267 & \textbf{0.132} & 0.152 & * & *  \\
20 & 15 & \textbf{1286} & 2753 & 3691 & 1808 & * & * & \textbf{0.308} & 0.656 & 0.879 & 0.329 & * & *  \\
50 & 1 & 21 & \textbf{17} & 66 & 327 & 1616 & 1385 & 0.022 & \textbf{0.014} & 0.049 & 0.176 & 0.850 & 0.746  \\
50 & 2 & 219 & \textbf{22} & 66 & 377 & 1180 & 2772 & 0.178 & \textbf{0.019} & 0.055 & 0.243 & 0.760 & 1.704  \\
50 & 5 & 188 & \textbf{123} & 226 & 1880 & 2296 & * & 0.147 & \textbf{0.098} & 0.175 & 1.208 & 1.467 & *  \\
50 & 10 & 462 & \textbf{377} & 1647 & 1456 & 699 & * & 0.352 & \textbf{0.285} & 1.229 & 0.972 & 0.466 & *  \\
50 & 20 & \textbf{1082} & 56530 & 9363 & 2058 & * & * & \textbf{0.842} & 42.686 & 7.063 & 2.173 & * & *  \\
50 & 25 & 1326 & 2361 & 2307 & \textbf{1157} & * & * & \textbf{1.230} & 1.913 & 1.835 & 1.243 & * & *  \\
50 & 30 & 3430 & \textbf{1262} & 2045 & 3981 & * & * & 2.989 & \textbf{1.044} & 1.654 & 4.412 & * & *  \\
100 & 1 & 95 & \textbf{22} & 182 & 2792 & 1476 & 9554 & 0.446 & \textbf{0.084} & 0.572 & 9.545 & 4.887 & 33.713  \\
100 & 2 & 104 & \textbf{32} & 102 & 802 & 1531 & * & 0.429 & \textbf{0.120} & 0.361 & 3.154 & 5.996 & *  \\
100 & 5 & 449 & 256 & \textbf{83} & 4603 & * & * & 1.570 & 0.902 & \textbf{0.295} & 20.776 & * & *  \\
100 & 10 & 1675 & 37263 & \textbf{427} & 3050 & 3281 & * & 5.724 & 124.269 & \textbf{1.429} & 15.528 & 16.771 & *  \\
100 & 25 & 2388 & 12916 & \textbf{2346} & 2687 & * & * & 8.041 & 43.605 & \textbf{7.885} & 15.529 & * & *  \\
100 & 50 & 4596 & 3526 & * & \textbf{3395} & * & * & 16.336 & \textbf{12.488} & * & 23.325 & * & *  \\
100 & 75 & 7070 & 27964 & 123020 & \textbf{4816} & * & * & \textbf{26.387} & 104.134 & 459.301 & 38.100 & * & *  \\
\hline\multicolumn{14}{l}{\footnotesize\textit{Bolded values equal to the best algorithm according to iteration count or time.}}\\ 
\multicolumn{14}{l}{\footnotesize\textit{* indicates the algorithm failed to find a  stationary point meeting the tolerances by the 500,000th iteration.}}\\
\bottomrule
\end{tabular}}
\caption{Performance for all algorithms applied to the QP-BC Problem \eqref{eq:num.problem2}, with $C=1$ and $\alpha=10^{-2}$, for different pair of values $(B,\omega)$. The iteration and time columns record the number of iterations and time in seconds to find a stationary point satisfying the relative error condition with $(\rho,\eta)=(10^{-5},10^{-5})$.}\label{tab:numeric.results.table2}
\end{table}



==> data/ADMM/admm.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Spring 2021.  
%
%
%  Author: Thesis Office
%  
%  Last Updated: 1/13/2021
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           SECTION I
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\pagestyle{plain} % No headers, just page numbers
%\pagenumbering{arabic} % Arabic numerals
%\setcounter{page}{1}


\chapter{\uppercase {An Adaptive Proximal ADMM for Nonconvex Linearly-Constrained Composite Programs }}\label{chapter:admm}


\begin{center}
    \textbf{Abstract}
\end{center}


   This chapter develops an adaptive Proximal Alternating Direction Method of Multipliers (\textproc{P-ADMM}) for solving linearly-constrained, weakly convex, composite optimization problems. 
   This method is adaptive to all problem parameters, including smoothness and weak convexity constants.
   It is assumed that the smooth component of the objective is weakly convex and possibly nonseparable, while the non-smooth component is convex and block-separable. The proposed method is tolerant to the inexact solution of its block proximal subproblem so it does not require that the non-smooth component has easily computable block proximal maps. Each iteration of our adaptive \textproc{P-ADMM} consists of two steps: 
   (1) the sequential solution of each block proximal subproblem, and (2) adaptive tests to decide whether to perform a full Lagrange multiplier and/or penalty parameter update(s). Without any rank assumptions on the constraint matrices, it is shown that  the adaptive \textproc{P-ADMM} obtains an approximate first-order stationary point of the constrained problem in 
   a number of iterations that matches the state-of-the-art complexity for the class of \textproc{P-ADMM}s. The two proof-of-concept numerical experiments that conclude the paper suggest our adaptive \textproc{P-ADMM} enjoys significant computational benefits.


\clearpage




\section{Introduction}
This chapter develops an adaptive Proximal Alternating Direction Method of Multipliers, called \textproc{A-ADMM}, for solving the linearly-constrained, smooth, weakly convex, composite optimization problem  

\begin{equation}\label{initial.problem}
    F^* = \min_{y\in\mathbb{R}^n} \left\{ F(y) := f(y)+\sum_{t=1}^B\Psi_t(y_t)\ \ : \ \ \sum_{t=1}^B A_ty_t=b \right\},  
\end{equation}
where $n=n_1+\ldots+n_B$, 
$y=(y_{1},\ldots,y_{B})\in\mathbb{R}^{n_{1}}\times\cdots\times\mathbb{R}^{n_{B}}$,
$b\in \mathbb{R}^l$,
$f:\mathbb{R}^n\to \mathbb{R}$ is a real-valued differentiable function which is $m$-weakly convex,
and $\Psi_t:\mathbb{R}^{n_t}\rightarrow (-\infty, \infty]$ is a  proper, closed, convex function which is $M_h$-Lipschitz continuous on its  compact domain, 
for every $t\in\{1,\ldots, B\}$. 
To ease notation, let $A(\cdot):=\sum_{t=1}^BA_t(\cdot)$ and $\Psi(\cdot):=\sum_{t=1}^B\Psi_t(\cdot)$.
The goal in this paper is to find a $(\rho,\eta)$-stationary solution of \eqref{initial.problem}, i.e., a quadruple  $(\bar x, \bar p, \bar v,\bar\varepsilon) \in (\mathrm{dom } \Psi) \times \mathbb{R}^l \times {\rm{Im}}(A^*)
\times \mathbb{R}_{+}$ satisfying 
\begin{equation}\label{eq:stationarysol}
\bar v \in \nabla f(\bar x) + \partial_{\bar\varepsilon} \Psi(\bar x) + A^*\bar p, \quad \sqrt{\|\bar v\|^2 + \bar\varepsilon}  \leq \rho , \quad \|A\bar x-b\|\leq \eta,
\end{equation}
where $(\rho,\eta)\in \mathbb{R}^2_{++}$ is 
a given tolerance pair.

A popular primal-dual algorithmic framework for solving problem \eqref{initial.problem} that takes advantage of its block structure is the Proximal Alternating Direction Method of Multipliers (\textproc{P-ADMM}), which is based on the dampened augmented Lagrangian function,
\begin{equation}\label{DP:AL:F}
{\cal L}_{c}^\theta(y;p)  :=F(y)+(1-\theta)\left\langle p,Ay-b\right\rangle +\frac{c}{2}\left\Vert Ay-b\right\Vert ^{2},
\end{equation}
where $\theta\in (0,1)$ is a dampening parameter and $c>0$ is a penalty parameter. Given $(\tilde y^{k-1}, \tilde q^{k-1},c_{k-1})$, \textproc{P-ADMM} finds the next triple $(\tilde y^k,\tilde q^k,c_k)$ as follows. Starting from $\tilde y^{k-1}$, it first performs a few cyclic block updates via an inexact proximal point method, with a fixed $B$-tuple $(\lambda_1,\cdots,\lambda_B)$ of block prox stepsizes, applied to the augmented Lagrangian function ${\cal L}_{c_{k-1}}^\theta(\cdot\,;\,\tilde q^{k-1})$ to obtain $\tilde y_k$. Next, it performs a standard dual update to obtain $\tilde q^k$. Finally, it possibly increases the penalty parameter. More formally, letting $z^0=\tilde y^{k-1}$ and $|\mathcal{I}_k|$ be a positive integer, it recursively computes the sequence $\{z^i\}_{i=1}^{|\mathcal{I}_k|}$ as follows: given $z^{i-1}$, it computes $z^i$ by sequentially solving the subproblems
\begin{align}\label{eq:x_update}
z_t^{i} \approx \argmin_{u_t\in\mathbb{R}^{n_{t}}}\left\{ \lambda_t{\cal L}^{\theta}_{c_{k-1}}(z_{<t}^{i},u_t,z^{i-1}_{>t};\tilde q^{k-1})+\frac{1}{2}\|u_t-z^{i-1}_t\|^{2}\right\} , \quad t=1,\ldots,B.
\end{align} 
It then sets $\tilde y^k=z^{|\mathcal{I}_k|}$, performs a Lagrange multiplier update according to 
\begin{equation}
    \tilde q^{k} = (1-\theta)\tilde q^{k-1}+\chi c_k\left(A\tilde y^k-b\right),\label{eq:p_update}
\end{equation}
where $\chi$ is a positive under-relaxation parameter, and chooses a scalar $c_k \ge c_{k-1}$ as the next penalty parameter. The rationale for denoting the number of cyclic updates, prior to a dual update, as $|\mathcal{I}_k|$ will become clear in Section \ref{subsection:SA-ADMM}.


In the recent publication  \cite{KongMonteiro2024}, 
the authors proposed a version of 
\textproc{P-ADMM} for solving \eqref{initial.problem}, which assumes that
$|\mathcal{I}_k|=1$,
$\lambda_1=\cdots=\lambda_B$, and
$(\chi, \theta) \in (0,1]^2$ satisfy
\begin{equation}\label{eq:assumptio:B}
2\chi B(2-\theta)(1-\theta)\le \theta^2.
\end{equation} 
One of the main contributions of \cite{KongMonteiro2024} is that its convergence guarantees do not require \textit{the last block condition}, ${\rm{Im}}(A_B)\supseteq \{b\}\cup{\rm{Im}}(A_1)\cup\ldots\cup{\rm{Im}}(A_{B-1})$ and $\Psi_B\equiv 0$, 
that hinders many instances of \textproc{P-ADMM}, see \cite{chao2020inertial,goncalves2017convergence,themelis2020douglas,zhang2020proximal}.
However, the main drawbacks of the \textproc{P-ADMM} of \cite{KongMonteiro2024} include: 
(i) the strong assumption \eqref{eq:assumptio:B} 
on $(\chi, \theta)$; (ii) subproblem \eqref{eq:x_update}
must be solved exactly;
(iii) the stepsize parameter $\lambda$ is conservative and requires the knowledge of $f$'s weak convexity parameter;
(iv) it (conservatively) updates the Lagrange multiplier after each primal update cycle (i.e. $|\mathcal{I}_k|=1$);
(v) its iteration-complexity has a high dependence on the number of blocks $B$, namely,
${\cal O}(B^8)$.
Paper \cite{KongMonteiro2024} also presents computational results comparing its \textproc{P-ADMM} with a more practical variant where $(\theta,\chi)$, instead of satisfying  \eqref{eq:assumptio:B}, it is set to $(0,1)$. Intriguingly, this $(\theta,\chi)=(0,1)$ regime substantially outperforms the theoretical regime of \eqref{eq:assumptio:B} in the provided computational experiments.  No convergence analysis for the $(\theta,\chi)=(0,1)$ regime is forwarded in \cite{KongMonteiro2024}. Thus, \cite{KongMonteiro2024} leaves open the tantalizing question of whether the convergence of \textproc{P-ADMM} with $(\theta,\chi)=(0,1)$ can be theoretically secured.\\



\noindent{\bf Contributions:}
This chapter partially addresses the convergence analysis issue raised above by studying
a {\it completely parameter-free} \textproc{P-ADMM}, with $(\theta,\chi)=(0,1)$
and  $|\mathcal{I}_k|$ adaptively chosen, called \textproc{A-ADMM}.  Rather than making the conservative determination that $|\mathcal{I}_k|=1$, the studied adaptive method ensures the dual updates are committed as frequently as possible.
It is shown that \textproc{A-ADMM} finds a $(\rho,\eta)$-stationary solution
in 
${\cal O}(B\max\{\rho^{-3}, \eta^{-3}\})$ iterations. \textproc{A-ADMM} also exhibits the following additional features:

\begin{itemize}%[itemsep=0pt]
\setlength{\itemsep}{0pt}
%\itemsep0em 
    
    \item 
    Similar to the \textproc{P-ADMM} of \cite{KongMonteiro2024}, its complexity is established without assuming that the {\it last block condition} holds;
    
    
    
    \item Compared to the 
   ${\cal O}(B^8\max\{\rho^{-3},\eta^{-3}\})$ iteration-complexity of the \textproc{P-ADMM} of \cite{KongMonteiro2024},
    the one for  \textproc{A-ADMM} vastly  {\it improves the dependence on $B$};

    \item
    \textproc{A-ADMM}  uses an adaptive scheme that aggressively computes {\it variable block prox stepsizes}, instead of fixed ones that require knowledge of the weak convexity parameters $m_1,\ldots,m_B$
    (e.g., the choice $\lambda_1=\ldots=\lambda_B \in (0, 1/(2m))$ where $m
    := \max\{m_1,\ldots,m_B\}$
    made by the \textproc{P-ADMM} of \cite{KongMonteiro2024}). In contrast to the \textproc{P-ADMM} of \cite{KongMonteiro2024}, \textproc{A-ADMM} may generate various $\lambda_t $'s which are larger than $1/m_t$
    (as observed in our computational results), and hence
    which do not guarantee convexity of \eqref{eq:x_update}.
    
    \item
    \textproc{A-ADMM} is also adaptive to Lipschitz parameters;

    \item 
    In contrast to the \textproc{P-ADMM} in \cite{KongMonteiro2024},
    \textproc{A-ADMM} allows the block proximal subproblems \eqref{eq:x_update} to be either exactly or {\it inexactly} solved.
\end{itemize}

\noindent \textbf{Related Works}:  
ADMM methods with $B=1$ are well-known to be equivalent to
augmented Lagrangian methods. Several references have studied augmented Lagrangian and proximal augmented Lagrangian methods in the convex (see e.g., \cite{Aybatpenalty,AybatAugLag,LanRen2013PenMet,LanMonteiroAugLag,ShiqiaMaAugLag16, zhaosongAugLag18,IterComplConicprog,Patrascu2017, YangyangAugLag17}) and nonconvex 
(see e.g. \cite{bertsekas2016nonlinear, birgin2,solodovGlobConv,HongPertAugLag, AIDAL, RJWIPAAL2020, NL-IPAL, RenWilmelo2020iteration, YinMoreau, ErrorBoundJzhang-ZQLuo2020, ADMMJzhang-ZQLuo2020,sun2021dual}) settings.
Moreover, ADMMs and proximal ADMMs in the convex setting have also been broadly studied in the literature (see e.g. \cite{bertsekas2016nonlinear,boyd2011distributed,eckstein1992douglas,eckstein1998operator,eckstein1994some,eckstein2008family,eckstein2009general,gabay1983chapter,gabay1976dual,glowinski1975approximation,monteiro2013iteration,rockafellar1976augmented,ruszczynski1989augmented}).
So from now on, we
just discuss \textproc{P-ADMM} variants where $f$ is nonconvex and $B > 1$.
% , as the convex case has been extensively explored in the literature (see \cite{bertsekas2016nonlinear,boyd2011distributed,eckstein1992douglas,eckstein1998operator,eckstein1994some,eckstein2008family,eckstein2009general,gabay1983chapter,gabay1976dual,glowinski1975approximation,monteiro2013iteration,rockafellar1976augmented,ruszczynski1989augmented}). 

A discussion of the existent literature on non-convex \textproc{P-ADMM} is best framed by dividing it into two different corpora: those papers that assume the last block condition and those that do not. Under the \textit{last block condition}, the iteration-complexity established is ${\cal O}(\varepsilon^{-2})$, where $\varepsilon := \min\{\rho,\eta\}$.  Specifically, \cite{chao2020inertial,goncalves2017convergence,themelis2020douglas, wang2019global} 
introduce \textproc{P-ADMM} approaches assuming $B=2$, while \cite{jia2021incremental, jiang2019structured,melo2017iterationJacobi,melo2017iterationGauss} present (possibly linearized) \textproc{P-ADMM}s assuming $B\geq 2$. 
A first step towards removing the last block condition was made by \cite{jiang2019structured} which
proposes an ADMM-type method applied to a penalty reformulation of \eqref{initial.problem} that artificially satisfies the last block condition. This method possesses an ${\cal O}(\varepsilon^{-6})$ iteration-complexity bound.

% We next discuss papers that do not assume {\it the last block condition} and are based on ADMM approaches directly applicable to \eqref{initial.problem} or some reformulation of it. An early paper in this second direction is \cite{jiang2019structured}, which establishes an ${\cal O}(\varepsilon^{-6})$ iteration-complexity bound for an ADMM-type  method applied to a  penalty reformulation of \eqref{initial.problem} that artificially satisfies the last block condition.

On the other hand, development of ADMM-type methods directly applicable to \eqref{initial.problem} is considerably more challenging and only a few works addressing this topic have surfaced. In addition to \cite{jiang2019structured}, earlier contributions to this topic were obtained in  \cite{hong2016convergence,sun2021dual,zhang2020proximal}. More specifically,
\cite{hong2016convergence,zhang2020proximal} develop a novel small stepsize ADMM-type method without establishing its complexity. Finally, \cite{sun2021dual} considers an interesting but unorthodox negative stepsize for its Lagrange multiplier update, that sets it outside the ADMM paradigm, and thus justifies its qualified moniker, ``scaled dual descent ADMM''.

\subsection{Chapter's Organization}

In this subsection, we outline this article's structure. This section's lone remaining subsection, Subsection~\ref{subsec:notation}, briefly lays out the basic definitions and notation used throughout. Section \ref{subsec:subpro:e} introduces a notion of an inexact solution of \textproc{A-ADMM}'s foundational block proximal subproblem \eqref{eq:x_update} along with  efficient subroutines designed to find said solutions. Section~\ref{adp:ADMM} presents this article's centerpiece algorithm, \textproc{A-ADMM}, and its main subprocedure and ``static" version, \textproc{S-ADMM}, along with the main theorems governing their iteration-complexity (Theorem \ref{the:dynamic} and \ref{thm:static.complexity}). Section~\ref{subsubsec:subroutine} undertakes the long proof of the \textproc{S-ADMM} complexity theorem and presents all of the supporting technical lemmas. Section~\ref{admm:sec:numerical} presents proof-of-concept numerical experiments that display the superb efficiency of \textproc{A-ADMM} for two different problem classes. Section \ref{sec:concluding} gives some concluding remarks that suggest further research directions.


\subsection{Notation and Basic Definitions}\label{subsec:notation}

This subsection lists the elementary notation deployed throughout the paper. We let $\mathbb{R}_{+}$  and $\mathbb{R}_{++}$ denote the set of non-negative and positive real numbers, respectively. We shall assume that the $n$-dimensional Euclidean space, $\mathbb{R}^n$, is equipped with an inner product, $\inner{\cdot}{\cdot}$. The associated induced norm will be written as $\|\cdot\|$. Given $\nu\in\mathbb{R}^n$, we let 
\begin{equation}\label{def:max:mu}
\max(\nu):=\max_{1\leq t\leq n} \{\nu_t\}\text{ and }\min(\nu) = \min_{1\leq t\leq n}\{ \nu_t \}.
\end{equation}
When the Euclidean space of interest has the block structure $\mathbb{R}^{n_{1}}\times\cdots\times\mathbb{R}^{n_{B}}$, we will often consider, for $x=(x_{1},\ldots,x_{ B}) \in\mathbb{R}^{n_{1}}\times\cdots\times\mathbb{R}^{n_{B}}$, the aggregated quantities 
\begin{gather}
\begin{gathered}
x_{<t}:=(x_{1},\ldots,x_{t-1}), \quad  x_{>t}:=(x_{t+1},\ldots,x_{ B}),\quad x_{\leq t}:=(x_{<t},x_{t}),\quad x_{\geq t}:=(x_{t},x_{>t}).
\end{gathered}
\label{eq:intro_agg}
\end{gather}
For a given closed, convex set $Z \subset \mathbb{R}^n$, we let $\partial Z$ designate its boundary. The distance of a point $z \in \mathbb{R}^n$ to $Z$, measured in terms of $\|\cdot\|$, is denoted ${\rm dist}(z,Z)$. 
The indicator function of $Z$, $\delta_Z$, is defined by $\delta_Z(z)=0$ if $z\in Z$, and $\delta_Z(z)=+\infty$ otherwise.

The set of points where a function $\Psi:\mathbb{R}^n\to (-\infty,\infty]$ is finite-valued, $\mathrm{dom } \Psi:= \{x\in \mathbb{R}^n : \Psi(x) < +\infty\}$, is called its domain. We say that $\Psi$ is called proper if it is finite-valued at some point $x\in\mathbb{R}^n$, i.e. if 
$\mathrm{dom } \Psi \ne \emptyset$. We call $g\in\mathbb{R}^n$ an $\epsilon$-subgradient of a proper function $\Psi:\mathbb{R}^n\to(-\infty,\infty]$ at $x\in\mathrm{dom } \Psi$, with $\epsilon\geq 0$, if  
\[
\Psi(z)\geq \Psi(x)+\inner{g}{z-x}-\varepsilon
\]
holds for all $z\in \mathbb{R}^n$.	The set of all $\epsilon$-subgradients of $\Psi$ at $x$, $\partial_\epsilon \Psi(\cdot)$, is called the $\epsilon$-subdifferential of $\Psi$. When $\epsilon=0$, the $\epsilon$-subdifferential recovers the classical subdifferential, $\partial \Psi(\cdot):=\partial_0 \Psi(\cdot)$. If $\psi$ is a real-valued function that is differentiable at $\bar z \in \mathbb{R}^n$, then its affine approximation $\ell_\psi(\cdot,\bar z)$ at $\bar z$ is the function defined, for arbitrary $z\in\mathbb{R}^n$, by the rule $z\mapsto \psi(\bar z) + \inner{\nabla \psi(\bar z)}{z-\bar z}$. The smallest positive singular value of a  nonzero linear operator $Q:\mathbb{R}^n\to \mathbb{R}^l$ is denoted $\nu^+_Q$ and its operator norm is $\|Q\|:=\sup \{\|Q(w)\|:\|w\|=1\}.$  

\section{Methods and Concepts for the Inexact Solution of \eqref{eq:x_update}}\label{subsec:subpro:e}

This section introduces a notion of an inexact stationary point for the block proximal subproblem \eqref{eq:x_update} along with two different efficient methods for discovering such points. These methods permit the application of our main algorithm, \textproc{A-ADMM}, even when \eqref{eq:x_update} is not exactly solvable. In Subsection \ref{subsec:inexact-solution}, we introduce our inexact solution concept, Definition \ref{def:BB}, for \eqref{eq:x_update}. Subsection \ref{sec:SCGM} introduces a general method for finding said inexact solutions to \eqref{eq:x_update}, while Subsection \ref{subsec:Adap-ACG} presents accelerated schemes for 
solving strongly convex or convex versions of \eqref{eq:x_update}. It also discusses how these schemes are used to tentatively solve weakly convex versions of 
\eqref{eq:x_update}.

\subsection{An Inexact Solution Concept for \eqref{eq:x_update}}\label{subsec:inexact-solution}

This subsection introduces our notion (Definition \ref{def:BB}) of an inexact solution of the block proximal subproblem \eqref{eq:x_update}. To cleanly frame this solution concept, observe that \eqref{eq:x_update} can be cast in the form 
\begin{equation}\label{ISO:problem}
\Gamma^*=\min \{\Gamma(z):=\Gamma_s(z)+\Gamma_n(z) : z\in\mathbb{R}^n\},
\end{equation} 
where
\begin{equation}\label{def:ps}
\Gamma_s(\cdot) =\lambda_t \hat {\cal L}_{c}(y_{<t}^{i},\cdot,y_{>t}^{i-1};\tilde q^{k-1})+\frac{1}{2}\|\cdot-\tilde y_{t}^{k-1}\|^{2}, \quad \Gamma_n(\cdot) = \lambda_t \Psi_t(\cdot),
\end{equation}
and  ${\cal \hat L}_{c}(\cdot\,;\tilde q^{k-1})$ is the smooth part of \eqref{DP:AL:F} with $(\theta,\chi)=(0,1)$, defined as
\begin{align}\label{def:smooth:ALM}
{\cal \hat L}_{c}(y;\tilde q^{k-1}):= f(y)+\left\langle \tilde q^{k-1},Ay-b\right\rangle +\frac{c}{2}\left\Vert Ay-b\right\Vert ^{2}.
\end{align}
The assumptions introduced in  Section \ref{adp:ADMM} regarding problem \eqref{initial.problem} will ensure that the above functional pair $(\Gamma_s, \Gamma_n)$
satisfies the following conditions:
\begin{enumerate}
    \item[(B1)] $\Gamma_n: \mathbb{R}^n\to (-\infty,+\infty]$ is a proper, closed, convex function with compact domain;

    \item[(B2)] function $\Gamma_s:\mathbb{R}^n \to \mathbb{R}$ is differentiable and there exists $M> 0$ such that
    \begin{align*}
    & \|\nabla\Gamma_s(z)-\nabla\Gamma_s(\tilde z)\|
    \leq M\|z-\tilde z\| \quad  \forall \, z,\tilde{z}\in\mathbb{R}^n.
    \end{align*}
\end{enumerate}
\noindent Hence, we assume that conditions (B1) and (B2) are valid throughout our discussion in this preliminary section.

With the technical setup now established, we are able to forward our inexact stationary point concept for \eqref{ISO:problem}, and hence for \eqref{eq:x_update}.

\begin{definition}\label{def:BB}
     For a given $z^0 \in \mathrm{dom } \Gamma_n$ and parameter triple
$(\tau_1,\tau_2, \vartheta)\in \mathbb{R}_+^3$,
a triple $(\bar z, \bar r, \bar \epsilon)\in \mathbb{R}^n\times\mathbb{R}^n\times\mathbb{R}_{+}$ satisfying
\begin{align}
\bar r \in \nabla \Gamma_s(\bar z) &+ \partial_{\bar\varepsilon} \Gamma_n(\bar z)\label{ISO:Cond:1}\\
\|\bar r\|^2 + 2 \bar\varepsilon \le 
\tau_1 
&\|z^0-\bar z\|^2+ \tau_2 [ \Gamma(z^0) - \Gamma(\bar z)]+ \vartheta^2 \label{ISO:Cond:2}  
\end{align}
is called a
$(\tau_1,\tau_2, \vartheta;z^0)$-stationary solution of \eqref{ISO:problem}.
If $\vartheta=0$, then $(\bar z, \bar r, \bar \epsilon)$ is simply referred to as a 
$(\tau_1,\tau_2;z^0)$-stationary solution of \eqref{ISO:problem}.
\end{definition}

\noindent We now make some remarks about  Definition \ref{def:BB}. First, \textproc{A-ADMM} uses
only $(\tau_1,\tau_2; z^0)$-stationary points, i.e., it always assumes that $\vartheta=0$. Second, if $(\tau_1,\tau_2, \vartheta)=(0,0,0)$, then \eqref{ISO:Cond:2} implies that $(\bar r,\bar\varepsilon)=(0,0)$ and \eqref{ISO:Cond:1} then implies that $\bar z$ is an exact stationary point of \eqref{ISO:problem}. Thus, if the triple $(\bar z, \bar r, \bar\varepsilon)$ is a $(\tau_1,\tau_2, \vartheta; z^0)$-stationary solution of \eqref{ISO:problem}, then $\bar z$ can be viewed as an approximate stationary solution of \eqref{ISO:problem} where the residual pair $(\bar r, \bar\varepsilon)$
is bounded according to \eqref{ISO:Cond:2} (instead of being zero as in the exact case).
Third, if $\bar z$ is an exact stationary point of \eqref{ISO:problem}, then the triple $(\bar z,0,0)$ is a $(\tau_1,0, \vartheta; z^0)$-stationary point of \eqref{ISO:problem} for any $(\tau_1,\vartheta) \in \mathbb{R}^2_+$. Fourth, if $\bar z$ is a stationary point of \eqref{ISO:problem} such that $\Gamma(z^0)-\psi(\bar  z)\ge 0$, then the triple $(\bar z,0,0)$ is a $(\tau_1,\tau_2, \vartheta; z^0)$-stationary point of \eqref{ISO:problem} for
any $(\tau_1,\tau_2,\vartheta) \in \mathbb{R}^3_+$. Hence, if $z^0$ is a stationary point of \eqref{ISO:problem}, then the triple $(z^0,0,0)$ is a $(\tau_1,\tau_2, \vartheta; z^0)$-stationary point of \eqref{ISO:problem} for any $(\tau_1,\tau_2,\vartheta) \in \mathbb{R}^3_+$.

\subsection{Composite Gradient Method}\label{sec:SCGM}

This subsection describes a variant of the composite gradient method, referred to as S-CGM, and its iteration-complexity, for finding a $(\tau_1,\tau_2, \vartheta; z^0)$-stationary point of \eqref{ISO:problem} regardless of whether or not the objective function $\psi$ is convex.  In fact, this method finds somewhat higher quality inexact stationary points where $\tau_1=0$. Specifically, it obtains a pair $(\bar z,\bar v)$ satisfying 
\begin{align}\label{eq:cgm.finals.conditions}
\bar v \in \nabla \Gamma_s(\bar z) + \partial \Gamma_n(\bar z) \quad \text{and} \quad
\|\bar v\|^2  \le 
 \sigma [ \Gamma(\tilde z^0) - \Gamma(\bar z)]+ \vartheta^2,
\end{align}
which implies that it is $(0,\sigma,\vartheta;z^0)$-stationary solution of \eqref{ISO:problem}. The S-CGM method is detailed below.

\begin{algorithm}[H]
%\setstretch{1.1}
    \caption{S-CGM}
    %		\label{alg:NC-FISTA}
    \begin{algorithmic}[1]
    \Require $\tilde z^0 \in \mathrm{dom } \Gamma_n$, $\sigma>0$, $\vartheta \ge 0$, $M>0$.
    \Ensure $(\bar z, \bar v)$ satisfying \eqref{eq:cgm.finals.conditions}

    %\State $z^0= z$
    \For{$j=1,2,\ldots$}
        \State Compute $(\tilde z^j,\tilde v^j)$ such that:
        \begin{align}
        &\tilde z^j \in\argmin_{z\in \mathbb{R}^{n}} \left\{ \ell_{\Gamma_s}(z, \tilde z^{j-1} )+ \Gamma_n(z)  + \frac{M}{2} \|z-\tilde z^{j-1}\|^2 \right\} \label{eq:CGM-nc2}\\
        &\tilde v^j := M(\tilde z^{j-1}-\tilde z^j) + \nabla \Gamma_s(\tilde z^j) - \nabla\Gamma_s (\tilde z^{j-1}).\label{def:resi:app}
        \end{align}
        \If{$\|\tilde v^j\|^2 \le \sigma [ \Gamma(\tilde z^0) -\Gamma( \tilde z^j)]+\vartheta^2$} $(\bar z, \bar v)=(\tilde z^j, \tilde v^j)$
            %\State \mathbb{R}eturn $(\bar z, \bar v)=(z^j,\tilde v^j)$
        \EndIf
    \EndFor		
\end{algorithmic}
\end{algorithm}

The following result, whose proof is given in Section \ref{append:cgm}, describes the
iteration-complexity 
of S-CGM.
\begin{prop}\label{main:appen:2}
S-CGM stops
in at most
\begin{equation}\label{eq:K:appe:2}
\bar K := \displaystyle
\begin{cases}
    1& \text{if $\vartheta^2 + \|\tilde v^1\|^2 = 0$}\\ 1+\displaystyle\left\lceil \frac{8M+\sigma}{\sigma}\ln \left(\frac{16M[\Gamma(\tilde z^0)-\Gamma^*]}{\vartheta^2+\|\tilde v^1\|^2 }\right)\right\rceil&\text{if $\vartheta^2 + \|\tilde v^1\|^2 > 0$} \\
\end{cases}
\end{equation}
iterations and its output $(\bar z, \bar v)$ satisfies \eqref{eq:cgm.finals.conditions}.
\end{prop}

We now make some comments about S-CGM. First, if $\sigma =0$, then it is well-known that the iteration-complexity of S-CGM is ${\cal O}(M \vartheta^{-2})$ (see for example \cite[Theorem 10.15]{beck2017}). On the other hand, if  $\sigma$ is positive, then the above result shows that the iteration-complexity of S-CGM is ${\cal O}(M\ln(\vartheta^{-2}))$.

\subsection{Accelerated Composite Gradient Methods in the Convex Setting}\label{subsec:Adap-ACG}

This subsection briefly surveys accelerated composite gradient methods from \cite{HeMonteiro2015} and \cite{sujanani2023adaptive} for finding $(\tau_1,0;z^0)$-stationary solutions of \eqref{ISO:problem} when $\psi$ is $\mu$-strongly convex for some $\mu \ge 0$ (with the convention that $\psi$ is convex for $\mu=0$). Assuming the conditions (B1) and (B2) hold, then  \cite{HeMonteiro2015} shows that an accelerated composite gradient (ACG) method variant finds a $(\tau_1,0;z^0)$-stationary solution of \eqref{ISO:problem}, namely a triple $(\bar z,\bar v,\bar \varepsilon)$ satisfying 
\[
\bar v \in \nabla \Gamma_s(\bar z) + \partial_{\bar\varepsilon} \Gamma_n(\bar z) \quad\text{and}\quad \|\bar v\|^2 + 2 \bar\varepsilon \le 
\tau_1 
\|z^0-\bar z\|^2,
\]
in at most
\[
{\cal O}\left(\left\lceil\min\left\{\sqrt{M(M+1)\lceil\tau_1^{-1}\rceil},\ 1+\left(1+\sqrt{M/\mu}\right) \max\{\log\left[M(M+1)\lceil\tau_1^{-1}\rceil\right], 1\} \right\}\right\rceil\right)
\]
iterations. Moreover, \cite{sujanani2023adaptive} describes an ACG variant that, in at most 
\[
{\cal O}\left(\sqrt{M/\mu}\max\{\log(M),1\}\right)
\]
iterations, either finds a $(\tau_1, 0\,; z^0)$-stationary solution of \eqref{ISO:problem} with $\bar \varepsilon=0$, i.e., of the form $(\bar z,\bar v,0)$, or
concludes that $\Gamma_s$ is not $\mu$-strongly convex. This method is an adaptive ACG scheme  (referred to as Adap-ACG) that searches for a stepsize $\lambda_t$ until a $(\tau_1, 0\,; z^0)$-stationary solution of \eqref{ISO:problem}, with $(\Gamma_s,\Gamma_n)$ given by \eqref{def:ps}, is found. This scheme repeatedly calls Adapt-ACG with $\lambda_t$ halved each time. Under the assumption that $\Gamma_s$ is $m_t$-weakly convex for every $t\in \{1,\ldots,B\}$,  this scheme stops after a finite number of calls to Adap-ACG because
$\Gamma_s$ given by \eqref{def:ps} is strongly convex for any $\lambda_t < 1/m_t$.

\section{An Adaptive \textproc{P-ADMM}}\label{adp:ADMM}

This section presents this paper's main algorithm, \textproc{A-ADMM}, for solving \eqref{initial.problem}. Subsection \ref{subsec:assump} details a few mild technical assumptions imposed on \eqref{initial.problem}. Subsection \ref{subsection:SA-ADMM} develops a ``static" version of \textproc{A-ADMM}, called \textproc{S-ADMM}, that maintains a constant penalty parameter throughout its execution. This ``static" version is the main subprocedure for \textproc{A-ADMM}. That subsection also presents the main complexity theorem (Theorem \ref{thm:static.complexity}) for \textproc{S-ADMM}, but the proof is deferred to Section \ref{subsubsec:subroutine}. Finally, Subsection \ref{subsection:DA:ADMM} describes \textproc{A-ADMM} and establishes its iteration-complexity (Theorem \ref{the:dynamic})

\subsection{Problem Assumptions}\label{subsec:assump}
This subsection describes a series of mild assumptions on this paper's main problem of interest \eqref{initial.problem}. We shall assume that $f, \Psi:\mathbb{R}^n\rightarrow (-\infty, \infty]$, $A:\mathbb{R}^n\rightarrow \mathbb{R}^l$, and $b\in \mathbb{R}^l$, satisfy the following conditions:

\begin{enumerate}
\item[(A1)] for every $t\in \{1,\ldots,B\}$, $\Psi_t:\mathbb{R}^{n_t}\to(-\infty,\infty]$ is proper, closed, and convex with ${\cal H}_t:=\mathrm{dom } \Psi_t$ compact;

\item[(A2)] $A$ is a nonzero linear operator and ${\cal F}:=\{x\in {\cal H}:Ax=b\}\neq \emptyset$, where ${\cal H}:= {\cal H}_1\times\cdots\times {\cal H}_B$;

\item[(A3)] $f$ is block $m$-weakly convex for $m=(m_1,\ldots,m_B)\in\mathbb{R}^B_{++}$, that is, for every $t\in \{1,\ldots,B\}$,
%\begin{gather} \label{eq:weak_cvx}
\[
f(x_{<t},\cdot,x_{>t}) + \delta_{{\cal H}_t}(\cdot) + \frac{m_{t}}{2}\|\cdot\|^{2}\text{ is convex for all } x\in{\cal H};
\]
%\end{gather}
    \item[(A4)] $f$ is differentiable on ${\cal H}$ and, for every $t\in \{1,\ldots,B-1\}$, there exists $L_{t}\ge 0$ such that
\begin{gather}
\begin{aligned}
& \|\nabla_{x_{t}}f(x_{< t},x_t,\tilde{x}_{>t})-\nabla_{x_{t}}f(x_{< t},x_t,{x}_{>t})\|
\leq L_t\|\tilde{x}_{>t}-x_{>t}\| \quad  \forall~ x,\tilde{x}\in{\cal H};
\end{aligned}
\label{eq:lipschitz_x}
\end{gather}
    \item[(A5)] for some $M_h\ge 0$, $\Psi(\cdot)$ is $M_h$-Lipschitz continuous on ${\cal H};$
    
    \item[(A6)]  there exists $\bar{z}\in {\cal F}$ such that $\bar{d}:=\text{dist}(\bar{z}, \partial {\cal H})>0$.
\end{enumerate}

Note that since ${\cal H}$ is compact, it follows from (A1) and (A2) that the scalars
\begin{equation}\label{def:damH}
       D_h:=\sup_{z \in {\cal H}} \|z-\bar{z}\|, \quad \nabla_f:=\sup_{u \in {\cal H}} \| \nabla f(u)\|, \quad \underline F := \inf_{u \in {\cal H}} F(u), \quad \overline F := \sup_{u \in {\cal H}}  F(u)  
\end{equation}
are bounded. Furthermore, throughout this paper, we let
\begin{equation}\label{eq:block_norm}
\|A\|_\dagger^2 := \sum_{t=1}^B \|A_t\|^2,
\end{equation}


\subsection{\textproc{S-ADMM}: A ``Static" Version of \textproc{A-ADMM}}\label{subsection:SA-ADMM}

This subsection presents \textproc{S-ADMM}, a static version of our \textproc{A-ADMM}, and its main complexity result (Theorem \ref{thm:static.complexity}). The qualifier ``static" is attached because this variant keeps the penalty parameter constant throughout its course. The proof of Theorem \ref{thm:static.complexity} is the focus of Section \ref{subsubsec:subroutine}. We start by elaborating \textproc{S-ADMM}.


\begin{algorithm}[H]
\setstretch{1.1}
\caption{\textproc{S-ADMM}}\label{alg:static}
\begin{algorithmic}[1]
\Statex \hskip-1.8em
\textbf{Universal Input:}  $C>0$, $\rho>0$, $\alpha>0$, $\sigma_1\le 1/8$, $\sigma_2> 0$ and $\sigma_1+\sigma_2/2\ge 0$ 

\Require $(x,p,\gamma,c)
\in {\cal H} \times \mathbb{R}^l \times \mathbb{R}^B_{++}
\times \mathbb{R}_{++}$

\Ensure  $(x^+,p^+,\gamma^+, v^+,  \varepsilon^+)$ 


\State $y^0=\tilde y^0=x,$ $\tilde q^0=p,$ $\tilde T_0=0,$ $\lambda^0=\gamma$,
$k=1$%, $\tilde S_0=0$ and $wR_0 =0$
\label{initialcondRS}
    
\For{$i\gets 1,2,\ldots$} \label{star:cycle}
        
    \For{$t\gets 1,2,\ldots, B$}\label{stat:begin.prox.admm}
    \State $\lambda_t = \lambda_t^{i-1}$\label{block:lam:t}
        \State
        set $(\Gamma_s,\Gamma_n)$  as in \eqref{def:ps} and \label{algo:psis.psin}
        \[
\tau_1=\left(\sigma_1+\frac{\sigma_2}{2}\right)\frac{\lambda_t}{1+2\lambda_t},\quad \tau_2=\frac{\sigma_2\lambda_t}{1+2\lambda_t}, \quad z^0 =y_t^{i-1},
        \]
        
        \ \ \ and find a $(\tau_1,\tau_2;z^0)$-stationary solution $(y_t,r_t,\varepsilon_t)$ of \eqref{ISO:problem}
        (see Definition \ref{def:BB})
        
        
         
        \label{stat:prox.lagrangian.update.test}
        %and
    \If {$(\lambda_t, y_{t}, r_t)$ does not satisfy
    \begin{align*}
        (1+\sigma_2)(\Delta{\cal L}_c)_t^i(y_t) \ge   \frac{1}{4\lambda_t}\|y_t-y^{i-1}_t\|^2 + \frac{c}{4} \|A_t(y_t-y^{i-1}_t)\|^2
    \end{align*}
    \label{eq:convex}
    \hskip2.3em
    }
        \State $\lambda_t =\lambda_t/2$ and go to line~\ref{stat:prox.lagrangian.update.test}. \label{stat:end.prox.admm}
        
        
    \Else

    \State  $(\lambda_t^i, y^{i}_t, r^{i}_t, \varepsilon_t^i)=(\lambda_t, y_t,r_t, \varepsilon_t)$\label{termnation:theta}
        
  \EndIf

    
    \EndFor
    
    \hfill
    
    \For{$t\gets 1,2,\ldots, B$}\label{stat:begin.loop.vi}
    \State $(\Delta f)_t^i \gets \nabla_{y_{t}}f(y_{< t}^{i}, y_{ t}^{i},y_{>t}^{i})- \nabla_{y_{t}}f(y_{< t}^{i}, y_{ t}^{i},y_{>t}^{i-1})$ \label{def:deltai}
    \State $ v_{t}^{i}\gets (\Delta f)_t^i + \frac{r_t^i}{\lambda^i_t}+ cA_{t}^{*}\sum_{s=t+1}^{ B}A_{s}(y_{s}^{i}-y_{s}^{i-1})-\frac{1}{\lambda_t^i}(y_{t}^{i}- y_{t}^{i-1})$ \label{stat:end.loop.vi}\;
    
    \EndFor
    \State $v^i=(v^i_1,\ldots, v^i_B)$, $y^i=(y^i_1,\ldots, y^i_B)$,  $\lambda^i=(\lambda^i_1,\ldots,\lambda^i_B)$, $\delta_i:=(\varepsilon^i_1/\lambda_1^i) + \ldots +  (\varepsilon^i_B/\lambda_B^i)$ \label{stat:def.vi.yi.lambdai.qi}

    \State $T_i= {\cal L}_c(\tilde y^{k-1};\tilde q^{k-1}) - {\cal L}_c(y^i;\tilde q^{k-1}) + \tilde T_{k-1}$\label{def:T:i}

    \hfill


    
    \If{$\|v^i\|^2 +\delta_i\le C^2$ and $i \ge (k \alpha T_i)/\rho^2  $}\label{stat:begin.test.cond}

        
        \State  $(\tilde y^k , \tilde v^k, \tilde \varepsilon_k) = 
        (y^i,v^i,\delta_i)$, and
        $\tilde q^{k} = \tilde q^{k-1} + c (A \tilde y^k - b) $ \label{stat:test.i.qi.ti.updates}

         \State 
         $\tilde T_k = T_i$, \  $\tilde \lambda^k = \lambda^i$, \ $i_{k}^+=i$ \label{line:update:i}

        \If{$\|\tilde v^k\|^2 +\tilde\varepsilon_k  \le \rho^2$}\label{cond:vi:stop}
\State $(x^+,p^+,\gamma^+,v^+, \varepsilon^+)=(\tilde y^k, \tilde q^k,\tilde \lambda^k, \tilde v^k, \tilde\varepsilon_k)$\label{update:stat:solu}
        \State \Return $(x^+,p^+,\gamma^+,v^+, \varepsilon^+)$ \label{stat:end.vi.rho}
        
        \Else
        \State  $k \leftarrow k+1$ \label{stat:end.test.cond}
        \EndIf
    


    

    \EndIf   
\EndFor

\end{algorithmic}
\end{algorithm}

Let us now clarify several of the steps of \textproc{S-ADMM}. The index $i$ is an iteration count for \textproc{S-ADMM}, whose iterations
are referred to as \textproc{S-ADMM} iterations throughout the paper. The $t$-th pass of the loop consisting of lines \ref{stat:begin.prox.admm} to \ref{termnation:theta} approximately solves the $t$-th augmented Lagrangian subproblem \eqref{eq:x_update} with a tentative prox stepsize $\lambda_t$ and then tests whether the descent condition of line \ref{eq:convex} holds. If it holds, then $\lambda_t$ is accepted as the prox stepsize for the $t$-th block in iteration $i$ (line \ref{termnation:theta}); otherwise, $\lambda_t$ is halved and the above steps are repeated with the updated $\lambda_t$ (line \ref{stat:prox.lagrangian.update.test}). The index $k$ counts the number of times that \textproc{S-ADMM} updates the Lagrange multiplier. The set of \textproc{S-ADMM} iterations after the $(k-1)$-th update and up to and including the $k$-th update, denoted $\Ik$, is called the $k$-th epoch. We enumerate each $\Ik$ as  
\begin{equation}
\label{eq:cy}
{\cal I}_k := \{i_k^-, \ldots, i_k^+\},\,\,\text{where}\,\,\, i_{k}^- := i_{k-1}^++1.
\end{equation}
The beginning and the end of an epoch are determined by lines \ref{stat:begin.test.cond} to \ref{stat:end.test.cond}. If the test in line \ref{stat:begin.test.cond} is passed at iteration $i$, then the Lagrange multiplier is updated. Provided \textproc{S-ADMM} does not terminate due to line \ref{cond:vi:stop}, a new epoch begins. %, then
% %line \ref{stat:test.i.qi.ti.updates} updates
% %the Lagrange multiplier and line \ref{line:update:i}
% %sets $i_k^+=i$ as the last iteration of epoch $\Ik$, which is then given by
% %\begin{equation}
% %\label{eq:cy}
% %{\cal I}_k := \{i_k^-, \ldots, i_k^+\},\,\,\text{where}\,\,\, i_{k}^- := i_{k-1}^++1,
% %\end{equation}
% (with the convention that $i_0^+=0$).
Line
\ref{cond:vi:stop} tests whether the residual vector pair $(\tilde v^k, \tilde\varepsilon_k)$, computed in line \ref{stat:test.i.qi.ti.updates}, 
satisfies the first inequality in \eqref{eq:stationarysol} that defines a $(\rho,\eta)$-stationary solution. If so, then \textproc{S-ADMM} terminates (see line \ref{update:stat:solu});
otherwise, $k$ is updated to $k+1$ and a new epoch commences. It is shown in Lemma~\ref{trivial:lemma} below that every epoch $\Ik$ terminates, and hence that the last index $i_k^+$ in \eqref{eq:cy} is well-defined. 

We now make several remarks about \textproc{S-ADMM}. First, it is shown in Lemma~\ref{lem:prop:Ine} below that if the stepsize $\lambda_t$ in \eqref{eq:x_update} satisfies $\lambda_t<1/m_t$, then the test in line~\ref{eq:convex} is satisfied. Since $\lambda_t$ is halved every time the test fails, this remark ensures that the loop in lines \ref{stat:prox.lagrangian.update.test} to \ref{termnation:theta} ends. Second, it is shown in Lemma \ref{lemm:stationary:cond} that the iterate $y^i=(y_1^i,\ldots,y_B^i)$, the residual vector $v^i=(v_1^i,\ldots,v_B^i)$ and $\delta_i:=(\varepsilon^i_1/\lambda_1^i) + \ldots +  (\varepsilon^i_B/\lambda_B^i)$ computed in
lines \ref{stat:begin.loop.vi} to \ref{stat:def.vi.yi.lambdai.qi} satisfy the stationary inclusion $v^i \in \nabla f(y^i) + \partial_{\delta_i} \Psi(y^i) + {\rm{Im}}(A^*)$.
Hence, upon termination of \textproc{S-ADMM}, its output satisfies the first two conditions in \eqref{eq:stationarysol} but not necessarily the last one. Third, if the (fixed) penalty parameter  $c$ is sufficiently large, then Theorem~\ref{thm:static.complexity}(c)  below shows that the final output of \textproc{S-ADMM} also satisfies the last condition in \eqref{eq:stationarysol}, and hence is a $(\rho,\eta)$-stationary solution of \eqref{initial.problem}.



It is not difficult to check that \textproc{S-ADMM} fits within the \textproc{P-ADMM} framework described in the introduction.  First, fixing $k\geq 0$, 
the cyclic, inexact solution of the block proximal subproblem \eqref{eq:x_update} is manifested in \textproc{S-ADMM} in lines \ref{stat:begin.prox.admm} to \ref{termnation:theta}. The damped augmented Lagrangian in this setting takes $(\theta,\chi)=(0,1)$. The sequence $\{z^j\}_{j=1}^{|\mathcal{I}_k|}$ is related to the sequence $\{y^j\}_{j=i_k^-}^{i^+_k}$ by the rule $z^j=y^{i_{k}^-+j-1}$ for $1\leq j\leq i^+_k-i_k^-+1$. By extension, $|\Ik|=i^+_k-i_k^-+1$ in accordance with \eqref{eq:cy}. Second, the dual update of \textproc{P-ADMM}, \eqref{eq:p_update}, manifests in \textproc{S-ADMM} in line \ref{stat:test.i.qi.ti.updates}.

Before stating the main result of this subsection, we define some constants that are used to express its complexity bounds. Given a triple $(\bar Q, \bar\gamma, \underline{c}) \in  \mathbb{R}_{++} \times  \mathbb{R}_{++}^B\times \mathbb{R}_{++}$, $\sigma_1\in (0,1/8]$, $\sigma_2> 0$, let
\begin{gather}
\begin{gathered}
\label{eq:def.Gamma.D3}
L:=(L_1,\ldots,L_t),\quad \bar\pi:=\overline{F}-\underline F+\frac{(\bar Q+3\kappa_p)^2}{2\underline{c}},\quad \kappa_p:=\frac{2D_h(M_h+
C +\nabla_f)+C^2}{\bar d \nu^{+}_A}\\
\bar\chi := 2(1+\sigma_2)\left[1+12\|L\|^2\max(\bar\gamma)+12(4\max (m)+\max (\bar\gamma^{-1}))+2\sigma_1\right]+\sigma_2,
\end{gathered}
\end{gather}
where $L_t$, $M_h$ and $\bar{d}$ are as in   (A4), (A5) and (A6), respectively, $C$ is part of the universal input for \textproc{S-ADMM},   $\max (m),$ $\max (\bar\gamma^{-1})$ are as in \eqref{def:max:mu}, $(D_h, \nabla_f, \underline F, \overline F)$ is as in \eqref{def:damH},  and  $\nu^{+}_A$ is the smallest positive singular value of the nonzero linear operator $A.$ 

Furthermore, define
\begin{align}\label{eq:def.constantsT}
    \Lambda_0 & :=8\kappa_p^2(1+\sigma_2)B\|A\|^2_\dagger\left[\frac{(1+\sigma_2)B\|A\|^2_\dagger}{2\alpha}+2\bar\pi\right],\quad
    \Lambda_1 := \left(\frac{\bar\chi}{\alpha}+1\right) \left(1+\frac{\bar\chi\bar\pi}{C^2}\right)\\
     \Lambda_2 &:=(1+\sigma_2)B\|A\|^2_\dagger \left[\left(\frac{\bar\chi}{\alpha}+1\right) \frac{1}{C^2} + \left( 1+ \frac{\bar\chi \bar\pi}{C^2}\right)\frac{1}{\alpha}\right], \quad 
     \Lambda_3 :=  \frac{(1+\sigma_2)^2B^2\|A\|^4_\dagger\bar\pi}{\alpha C^2}\nonumber\\
        \Lambda_4 & := 8\kappa_p^2(1+\sigma_2)B\|A\|^2_\dagger\left(\frac{\bar\chi }{\alpha}+\frac{3}{2}\right)  + \frac{8\alpha\kappa_p^2}{\underline{c}}\left(\frac{\bar\chi^2}{2\alpha^2}+\frac{3\bar \chi}{2\alpha }+1\right)
+2\alpha\bar\pi\left(\frac{\bar\chi}{\alpha}+1\right),\nonumber
\end{align}
where  $\|A\|_\dagger^2$ is as in \eqref{eq:block_norm}, $(\bar\chi, \bar\pi, \kappa_p)$ is as in \eqref{eq:def.Gamma.D3} and $\alpha\in \mathbb{R}_{++}$.

The remainder of this subsection presents and discusses one of the main results of this paper, the  iteration-complexity of \textproc{S-ADMM}. Its proof is the sole focus of Section \ref{subsubsec:subroutine}.

\begin{thm}[\textproc{S-ADMM} Complexity]\label{thm:static.complexity}

Let the tolerance pair $(\rho,\eta)\in \mathbb{R}^2_{++}$, and the triple
$(\bar Q, \bar \gamma, \underline{c})
\in  \mathbb{R}_{++} \times \mathbb{R}_{++}^B\times  \mathbb{R}_{++}$ be given.
Assume that the input $(x,p,\gamma,c) \in {\cal H} \times A(\mathbb{R}^n) \times \mathbb{R}^B_{++}
\times \mathbb{R}_{++}$ of \textproc{S-ADMM} satisfies
\begin{equation}\label{ini:cond:SA}
c \|Ax-b\| \le \bar Q, \quad  \|p\| \leq\kappa_p, \quad c \ge \underline{c},
\end{equation}
\begin{equation}\label{ini:cond:2:SA}
\min \left\{ \frac{1}{2 m}, \bar\gamma \right\} \le \gamma \le \bar \gamma, 
\end{equation}
where $\kappa_p$ and $\max (m)$ are as in \eqref{eq:def.Gamma.D3} and \eqref{def:max:mu}, respectively. Then, the \textproc{S-ADMM} method with
input $(x,p,\gamma,c)$ satisfies the following statements:
\begin{enumerate}
\item[(a)] the total  number of iterations performed by  \textproc{S-ADMM} is bounded by 
\begin{equation}\label{eq:def.T.complexity}
\Lambda(c,\rho):= \Lambda_0\frac{c}{\rho^2} +\Lambda_1+\Lambda_2c+ \Lambda_3c^2+ \Lambda_4\frac{1}{\rho^2},
\end{equation}
where  $\Lambda_0$, $\Lambda_1$, $\Lambda_2$, $\Lambda_3$, and $\Lambda_4$ are as in  \eqref{eq:def.constantsT};

\item[(b)] it outputs  $(x^+,p^+,\gamma^+, v^+, \varepsilon^+)$ satisfying the inclusion
\begin{equation}\label{residual:theorem:1}
v^+ \in \nabla f(x^+) + \partial_{\varepsilon^+} \Psi(x^+)+A^* p^+  
\end{equation}
and the following bounds
\begin{equation}\label{feasi:theorem:1}
c\|Ax^+-b\| \le 2\kappa_p ,
%\le \frac{\bar Q}2 ,
\quad \|p^+\| \le \kappa_p, \quad \|v^+\|^2+\varepsilon^+ \le \rho^2,
\end{equation}
\begin{equation}\label{bounds:gamma:initial}
\min\left
\{\frac{1}{2m_t}, \bar\gamma_t \right\}\leq \gamma^+_t \leq \bar\gamma_t \quad \forall  t\in\{1,\ldots, B\};
\end{equation}

\item[(c)] if $
   c\geq 2 \kappa_p/\eta$,
then the output triple $(x^+, p^+, v^+)$ of \textproc{S-ADMM}
  is a $(\rho,\eta)$-stationary solution of \eqref{initial.problem} as in \eqref{eq:stationarysol}. 
\end{enumerate}

\end{thm}

We now make several comments about Theorem~\ref{thm:static.complexity}. 
First, this result will be used in the next subsection to analyze the iteration-complexity of this paper's main algorithm, \textproc{A-ADMM}, which repeatedly invokes
\textproc{S-ADMM}  using a warm-start scheme, i.e.
if $c$ is the  penalty parameter and $(x^+,p^+,\gamma^+)$ is the output of the current \textproc{S-ADMM} call, then
the input  
of the next \textproc{S-ADMM} call 
is $(x^+,p^+,\gamma^+,2c)$.

Second, in the above setting, the quantities
$(\bar Q, \bar\gamma,\underline{c})$ should be viewed as uniform (upper or lower) bounds on the quantities $(c\|Ax-b\|, \gamma, c)$ associated with the input
$(x,p,\gamma, c)$
of all \textproc{S-ADMM} calls.
Moreover, the iteration-complexity bounds 
of Theorem~\ref{thm:static.complexity} are expressed in terms of $(\bar Q, \bar\gamma, \underline{c})$ 
instead of its  counterpart
$(c\|Ax-b\|, \gamma, c)$.

Third,
it is shown in Lemma~\ref{lemm:stationary:cond} and Lemma~\ref{lem:Ikfinite}
below that every quadruple
$(\tilde y^k, \tilde q^k,\tilde v^k, \tilde\varepsilon_k)$ satisfies the
stationary inclusion $\tilde v^k  \in \nabla f (\tilde y^k)+ \partial \Psi_{\tilde\varepsilon_k}(\tilde y^k) + A^* \tilde q^k$ and the
feasibility condition
$c\|A\tilde y^k-b\| \le 2 \kappa_p$.
    The assertion in Theorem~\ref{thm:static.complexity}(b) that \textproc{S-ADMM} outputs a quadruple $(x^+,p^+,v^+, \varepsilon^+)$ satisfying the inclusion  \eqref{residual:theorem:1}
and the feasibility bound \eqref{feasi:theorem:1}
follow from this fact and lines \ref{def:deltai} and \ref{stat:end.loop.vi} of \textproc{S-ADMM}. 
Moreover, \textproc{S-ADMM} stops whenever it
finds a quadruple $(x^+,p^+, v^+, \varepsilon^+)=(\tilde y^k, \tilde q^k,\tilde v^k, \tilde\varepsilon_k)$ satisfying $\|\tilde v^k\|^2+ \tilde\varepsilon_k\le \rho^2$, but not
necessarily the condition that
$\|A\tilde y^k-b\| \le \eta.$
However, if $c$ is sufficiently large, i.e., it
satisfies the condition in Theorem~\ref{thm:static.complexity}(c), then the latter condition would also hold because
$c\|A\tilde y^k-b\| \le 2 \kappa_p$ for every $k$, in which case $(\tilde y^k, \tilde q^k,\tilde v^k, \tilde\varepsilon_k)$ 
would be the desired $(\rho,\eta)$-stationary solution of \eqref{initial.problem}.


Fourth, we now formally argue how Theorem~\ref{thm:static.complexity} implies that a single \textproc{S-ADMM} call finds
a $(\rho,\eta)$-stationary solution of \eqref{initial.problem}  in at most ${\cal O}(\eta^{-1}\rho^{-2}+\rho^{-2}+\eta^{-1}+\eta^{-2})$
iterations (assuming that all other quantities in
\eqref{eq:def.constantsT} are ${\cal O}(1)$)
under the following assumptions:
i) the initial iterate $x \in {\cal H}$  satisfies $\|Ax-b\|= {\cal O}(\sqrt{\eta})$;
ii)
the constant $\kappa_p$ as in \eqref{eq:def.Gamma.D3}, which is generally not computable, and the weak convexity parameters $m$ as in assumption (A3), are known. Indeed, choose the quantities $\bar Q,\underline{c},c,p,\bar\gamma$ and $\gamma$ in Theorem~\ref{thm:static.complexity}
 as
\begin{equation}\label{cond:c0:Q0}
\bar Q =  \frac{2\kappa_p\|Ax-b\|}{\eta}, \quad \underline{c}=c= \frac{2\kappa_p}{\eta}, \quad p=0,
\quad \bar\gamma=\gamma =\frac{1}{2m}
\end{equation} 
and observe that $\bar \Gamma$ as in \eqref{eq:def.Gamma.D3} satisfies 
$\bar\pi ={\cal O}(1+\|Ax-b\|^2/\eta)={\cal O}(1)$, and hence
 all the $\Lambda_i's$ as in \eqref{eq:def.constantsT} are also ${\cal O}(1)$.
Since the  quantities in \eqref{cond:c0:Q0} satisfy the assumptions of Theorem~\ref{thm:static.complexity},
it follows from its statement (c), the latter observation, and the fact that $c={\cal O}(\eta^{-1})$,
that the iteration-complexity
of \textproc{S-ADMM} is 
$
{\cal O}(\eta^{-1}\rho^{-2}+\rho^{-2}+\eta^{-1}+\eta^{-2})$, and
hence $ {\cal O}(\epsilon^{-3})
$ where $\epsilon:=\min\{\rho, \eta\}$.



The next subsection shows that \textproc{A-ADMM}, up to a logarithmic term,  has the same complexity as in the fourth remark above, but now without assuming the knowledge of $\kappa_p$ nor that $x^+$ is near feasible. To obtain such complexity, \textproc{A-ADMM} invokes \textproc{S-ADMM} iteratively and doubles the penalty parameter until a $(\rho,\eta)$-stationary solution of \eqref{initial.problem} is obtained.


\subsection{A-ADMM: Description \& Complexity}\label{subsection:DA:ADMM}

This subsection describes this paper's focal algorithm, \textproc{A-ADMM}, and establishes its accompanying main complexity result (Theorem \ref{the:dynamic}). \textproc{A-ADMM} repeatedly calls \textproc{S-ADMM} as a subroutine, each time with the penalty parameter double the one used in the previous call. \textproc{A-ADMM} is formally stated below.

\begin{algorithm}[H]
\setstretch{1.1}
\caption{\textproc{A-ADMM}}\label{alg:dynamic}
\begin{algorithmic}[1]

\Statex \hskip-1.8em
\textbf{Universal Input:} $C>0,$ pair $(\rho,\eta) \in \mathbb{R}^2_{++}$, $\alpha>0$, $\sigma_1\le 1/8$, $\sigma_2> 0$ and $\sigma_1+\sigma_2/2 \ge 0$ 
\Require $(x^0, p^0, \gamma^0, c_0)\in {\cal H}\times A(\mathbb{R}^n)\times \mathbb{R}^B_{++}\times \mathbb{R}_{++}$ 
\Ensure $(\hat x,\hat p,\hat \gamma, \hat v, \hat{\varepsilon})$
    
\For{$\ell \gets 1,2,\ldots$}
    \State $(x^\ell ,p^\ell,\gamma^{\ell},v^\ell, \varepsilon_\ell )=\textproc{\textcolor{blue}{\textproc{S-ADMM}}}(x^{\ell-1},p^{\ell-1}, \gamma^{\ell-1}, c_{\ell-1})$ \label{dyn:stat.call}
    \If{$\|Ax^\ell-b\|\leq \eta$}\label{test:DA:ADMM}

        \State $(\hat x,\hat p,\hat \gamma, \hat v , \hat\varepsilon)=(x^\ell,p^\ell,\gamma^\ell, v^\ell, \varepsilon_\ell)$
        \State \Return $(\hat x,\hat p,\hat \gamma, \hat v , \hat\varepsilon)$   
    \Else    
        \State $c_{\ell}=2c_{\ell-1}$ \label{dyn:penalty.update}
    \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}

We now make some remarks about \textproc{A-ADMM}. First,
the initial penalty parameter $c_0$ can be chosen to be any positive scalar. Second, the initial Lagrange multiplier $p^0$ is required to be in $A(\mathbb{R}^n)$, e.g., it can be set to zero. Third, it uses a ``warm-start" strategy for calling \textproc{S-ADMM}, i.e.,  after the first call to \textproc{S-ADMM},  the input of  any %$\ell$-th 
 \textproc{S-ADMM} call is the output %$(x^{\ell-1},p^{\ell-1}, \gamma^{\ell-1}, c_{\ell-1})$ 
of the previous \textproc{S-ADMM} call. 
Fourth, Lemma~\ref{lemma:translate} below and Theorem~\ref{thm:static.complexity}(b) imply that each  \textproc{S-ADMM} call in line \ref{dyn:stat.call} of \textproc{A-ADMM} generates a 
triple $(x^\ell, p^\ell, v^\ell)$ satisfying the first two conditions in \eqref{eq:stationarysol}. 
Finally, \textproc{A-ADMM} stops
if the test in line~\ref{test:DA:ADMM} is satisfied;
if the test fails,
 then \textproc{S-ADMM} is called again with  $c_\ell$ set to $2 c_{\ell-1} = 2^{\ell}c_0.$ 

The next result guarantees that all of the hypotheses used in the iteration-complexity theorem for \textproc{S-ADMM} (Theorem~\ref{thm:static.complexity}) hold each time \textproc{A-ADMM} calls \textproc{S-ADMM}.




\begin{lemma}\label{lemma:translate}
Assume that $p^0=0$ and define
\begin{equation}\label{def:Q0}
\bar Q := \max\{4\kappa_p, c_0\|Ax^0-b\|\},  \quad \bar \gamma =\gamma^0,\quad \underline{c}=c_0
\end{equation}
where $\kappa_p$ is as in \eqref{eq:def.Gamma.D3}.
If \textproc{A-ADMM} performs the $\ell$-th iteration, then
\begin{gather}
\begin{gathered}
\label{eq:prop:input.bounds}
c_{\ell-1} \|Ax^{\ell-1} -b \|
\le \bar Q, \quad \|p^{\ell-1}\| \le \kappa_p, \quad \|v^{\ell}\|^2+\varepsilon_\ell \le \rho^2,\\
\min\left
\{\frac{1}{2\max (m)},\bar\gamma_t \right\}\leq \gamma^{\ell-1}_t \leq \bar \gamma_t,\text{ }\forall t\in\{1,\ldots,B\},
\end{gathered}
\end{gather}
where $\max (m)$ is as in \eqref{def:max:mu}. Moreover, the number of \textproc{S-ADMM} iterations performed
in the $\ell$-th call in line~\ref{dyn:stat.call} is bounded by $\Lambda(c_{\ell-1},\rho).$
\end{lemma}

\begin{proof}
First, note that all inequalities in \eqref{eq:prop:input.bounds}  hold trivially with $\ell=1$, except the third one. This is due to the assumption $p^0=0$ and the definitions of $\kappa_p$ and $\bar Q$ as in \eqref{eq:def.Gamma.D3} and \eqref{def:Q0}, respectively. Second, it follows from the logic of \textproc{A-ADMM} that
$c_{\ell}/2 = c_{\ell-1} \ge  c_0=\underline{c}$.
This observation and Theorem~\ref{thm:static.complexity}(b) 
 with $(x,p,\gamma,c)=(x^{\ell-1},p^{\ell-1},\gamma^{\ell-1}, c_{\ell-1})$ imply that if all inequalities in \eqref{eq:prop:input.bounds}, except the third one, hold for
$\ell$, then all the inequalities in \eqref{eq:prop:input.bounds} hold for $\ell+1$. These two observations and a simple induction argument show that the first conclusion of the lemma holds. 
The second one follows from \eqref{eq:prop:input.bounds} and Theorem~\ref{thm:static.complexity}(a) with $(x,p,\gamma,c)=(x^{\ell-1},p^{\ell-1},\gamma^{\ell-1}, c_{\ell-1}).$ 
\end{proof}

\begin{theorem}[\textproc{A-ADMM} Complexity]\label{the:dynamic}
The following statements about \textproc{A-ADMM} hold:
   \begin{itemize}
       \item[(a)]
       it obtains a $(\rho,\eta)$-stationary solution of \eqref{initial.problem} in no more than $
   \log_2 \left[\bar Q/(\underline{c}\eta) \right]+2$ calls to \textproc{S-ADMM};
   \item[(b)]
   the total number of \textproc{S-ADMM} iterations performed by it
   is no more than
%\begin{equation}\label{eq:dynamic.general.complex}
\[
\left(\frac{ \Lambda_0}{\rho^2}+\Lambda_2\right)\frac{4\bar Q}{\eta} +\left( \Lambda_1+\frac{ \Lambda_4}{\rho^2}\right)\left[\log_2\left(\frac{\bar Q}{\underline{c}\eta} \right)+2\right]+16\Lambda_3\frac{\bar Q^2}{\eta^2},
\]
\end{itemize} 
where $(\bar Q, \underline{c})$ and $(\Lambda_0, \Lambda_1, \Lambda_2, \Lambda_3, \Lambda_4)$ are the constants that appears in \eqref{def:Q0} and    \eqref{eq:def.constantsT},
respectively. 

\end{theorem}
\begin{proof}
(a)
  Assume for the sake of contradiction that \textproc{A-ADMM} generates an iteration index $\hat \ell$ such that $\hat \ell -2 > \log_2 \left[\bar Q/(\underline{c}\eta) \right]$, and hence 
  satisfying
    \[
    c_{\hat \ell-2} = \underline{c} 2^{\hat \ell-2}>\underline{c}2^{\log_2 [\bar Q/(\underline{c}\eta)]}=\frac{\bar Q}{\eta}.
    \]

    \noindent Combining Lemma~\ref{lemma:translate}, with $\ell=\hat\ell-2$, and Theorem~\ref{thm:static.complexity}(a) and (c),  with $(x,p,\gamma,c)=(x^{\hat\ell-2},p^{\hat\ell-2},\gamma^{\hat\ell-2}, c_{\hat\ell-2})$, we conclude that the output $(x^{\hat\ell-1},p^{\hat\ell-1},v^{\hat\ell-1},\gamma^{\hat\ell-1})$ of the call to \textproc{S-ADMM} in the $(\hat\ell-1)$-th iteration of \textproc{A-ADMM} is a $(\rho,\eta)$ stationary solution of \eqref{initial.problem}, and hence satisfies $\|Ax^{\hat\ell-1}-b\| \le \eta$.
    This yields the desired contradiction since the method should have terminated in the $(\hat \ell -1)$-th iteration in view of the stopping criterion in its line~\ref{test:DA:ADMM}.
    
    
(b) It follows from Lemma~\ref{lemma:translate} that the number of \textproc{S-ADMM} iterations is bounded by ${\Lambda}(c_{\tilde\ell-1},\rho),$   where $\tilde\ell$ is the last iteration performed by it. Then, we conclude from the previous item (a) that 
$\tilde{\ell}\le\log_2[\bar Q/(\underline{c}\eta)]+2.$ As a consequence, we can deduce that
\begin{equation}\label{triv.conseq}
2^{\tilde\ell}\le \frac{4\bar Q}{\underline{c}\eta}.
\end{equation}
Hence, these conclusions imply that the overall number of iterations performed by \textproc{S-ADMM} is bounded by
\begin{align*}
\sum_{\ell=1}^{\tilde\ell}\Lambda(c_{\ell-1},\rho)
&\overset{\eqref{eq:def.T.complexity}}= \sum_{\ell=1}^{\tilde \ell}\left(  \Lambda_0\frac{c_{\ell-1}}{\rho^2}+ \Lambda_1 + \Lambda_2 c_{\ell-1}+  \Lambda_3 c_{\ell-1}^2+\Lambda_4\frac{1}{\rho^2}\right)\\
&= 
\Lambda_1\tilde \ell+\frac{\underline{c} \Lambda_0}{\rho^2}\sum_{\ell=1}^{\tilde\ell}2^{\ell-1}+\frac{\Lambda_4}{\rho^2}\tilde \ell+  \Lambda_2\underline{c}\sum_{\ell=1}^{\tilde\ell}2^{\ell-1}+ \Lambda_3 \underline{c}^2\sum_{\ell=1}^{\tilde \ell}2^{2(\ell-1)} \\
&=\left(\Lambda_1+\frac{\Lambda_4}{\rho^2}\right)\tilde \ell+\left(\frac{\underline{c} \Lambda_0}{\rho^2}+\Lambda_2\underline{c}\right)(2^{\tilde \ell}-1)+ \frac{\Lambda_3 \underline{c}^2(4^{\tilde \ell}-1)}{3} \\
&\overset{\eqref{triv.conseq}}< \left( \Lambda_1+\frac{\Lambda_4}{\rho^2}\right)\left[\log_2\left(\frac{\bar Q}{\underline{c}\eta}\right)+2\right]+\left(\frac{\Lambda_0}{\rho^2}+\Lambda_2\right)\frac{4 \bar Q}{\eta} + 16 \Lambda_3\frac{\bar Q^2}{\eta^2}.
\end{align*}
\end{proof}


We now make some comments about Theorem~\ref{the:dynamic}.
First, it follows from Theorem~\ref{the:dynamic}(a)  that \textproc{A-ADMM} ends with a $(\rho,\eta)$-stationary solution of \eqref{initial.problem} by calling
\textproc{S-ADMM} no more than ${\cal O} (\log_2(\eta^{-1}))$ times.
Second,  Theorem~\ref{the:dynamic}(b) implies that the complexity of \textproc{A-ADMM}, in terms of the tolerances only, is
\[
{\cal O} (\rho^{-2}+\rho^{-2}\eta^{-1}+\eta^{-2}).
\]
Third, if $\epsilon:=\min\{\rho, \eta\}$ then the iteration-complexity of  \textproc{A-ADMM} is ${\cal O}(\epsilon^{-3})$.   

\section{The Proof of \textproc{S-ADMM}'s Complexity Theorem (Theorem \ref{thm:static.complexity})}
\label{subsubsec:subroutine}

The goal of this section is proving the theorem governing the iteration-complexity of \textproc{S-ADMM} (Theorem \ref{thm:static.complexity}). Our approach is comprised of three main steps. First, Subsection \ref{subsec:numberofcycles} bounds the number of epochs, $\mathcal{I}_1,\mathcal{I}_2,\ldots$. Second, Subsection \ref{subsec:totaliteration} derives a uniform bound on the size of each of the epochs. Third and finally, Subsection \ref{subsec:static.complexity.proof} synthesizes the results of the previous two steps to prove Theorem \ref{thm:static.complexity}.

\subsection{Step 1: Bounding the Number of Epochs}
\label{subsec:numberofcycles}

The goal of this subsection is to bound the total number of epochs $\mathcal{I}_1,\mathcal{I}_2,\ldots$ generated by \textproc{S-ADMM}. Before presenting the main result of this subsection, we state and prove some preliminary technical results. 
The first one summarizes some straightforward facts about $\textproc{S-ADMM}$.

\begin{lemma}\label{lemma:trivial:1}
    The following statements about  an  epoch $\Ik$ generated by $\textproc{S-ADMM}$ hold:
\begin{itemize}        
\item[(a)] if $\Ik$ ends, then $\tilde v^{k}=v^{i_k^+}$, $\tilde y^{k}=y^{i_k^+}$, $\tilde\varepsilon_k=\delta_{i_k^+}$ and  $\tilde T_{k}=T_{i_k^+}$; moreover,
        \begin{equation}\label{eq:lema1:test}
        \|\tilde v^k\|^2 +\tilde\varepsilon_k\le C^2\quad \text{and}\quad i_k^+ \ge \frac{k \alpha}{\rho^2} \tilde T_{k};
        \end{equation}
    \item[(b)] if $i<j$ are indices lying in $\Ik\cup\{i_{k-1}^+\}$, then
    $
    T_j-T_i = {\cal L}_c(y^i;\tilde 
    q^{k-1}) - {\cal L}_c(y^j;\tilde q^{k-1})$.
    \end{itemize}
\end{lemma}


\begin{proof} (a) Recalling from \eqref{eq:cy} that $i_k^+$ is the last index of $\Ik$, the identities $\tilde v^{k}=v^{i_k^+}$, $\tilde y^{k}=y^{i_k^+}$, $\tilde\varepsilon_k=\delta_{i_k^+}$ and  $\tilde T_{k}=T_{i_k^+}$ immediately follow from lines \ref{stat:test.i.qi.ti.updates} and \ref{line:update:i} of \textproc{S-ADMM}.  Thus, the inequalities in \eqref{eq:lema1:test} readily result from the tests in line~\ref{stat:begin.test.cond} with $i=i_k^+$, and the aforementioned identities.

   (b) We first note that if $i=i_{k-1}^+$ then the previous item of this lemma, applied with $k-1$ replacing $k$, implies that $\tilde T_{k-1}=T_{i_{k-1}^+}$ and $\tilde y^{k-1}=y^{i_{k-1}^+}$. Hence, the conclusion follows from the definition of $T_i$ in line~\ref{def:T:i} of \textproc{S-ADMM} with $i=j$. Now, if $i<j$ are indices lying in $\Ik$, then the statement is also a direct consequence of the definition of $T_i$ and $T_j$ as in line~\ref{def:T:i} of \textproc{S-ADMM}.
\end{proof}

The following result describes the properties of the iterate $(y_t,r_t,\varepsilon_t)$ 
obtained in line \ref{stat:prox.lagrangian.update.test} of \textproc{S-ADMM} 
using the data of subproblem \eqref{ISO:problem}.


\begin{lemma}
Every triple $(y_t,r_t,\varepsilon_t)$ generated in line \ref{stat:prox.lagrangian.update.test} of \textproc{S-ADMM} 
satisfies 
\begin{align}\label{set:inclu:translate}
r_t\in \nabla\left[\lambda_t{\cal \hat L}_{c}(y_{<t}^{i},\cdot,y_{>t}^{i-1};\tilde q^{k-1})+\frac{1}{2}\|\cdot-y_{t}^{i-1}\|^2\right](y_t)+\partial_{\varepsilon_t}(\lambda_t\Psi_t)(y_t),
\end{align} 
\begin{align}
(\lambda_t^{-1}+2) \|r_t\|^2 + 2 \varepsilon_t \le \sigma_1\|y_t-y_{t}^{i-1}\|^2+\lambda_t\sigma_2
         (\Delta{\cal L}_c)_t^i(y_t), \label{algo:eq.error.ineq}
\end{align}
where ${\cal \hat L}_{c}(\cdot\,;\,\tilde q^{k-1})$ is as in \eqref{def:smooth:ALM} and
\begin{equation}\label{def:Pot:Fun:i:t}
(\Delta{\cal L}_c)_t^i(\cdot):={\cal L}_c(y^i_{<t},y^{i-1}_{t},y^{i-1}_{> t};\tilde q^{k-1})-{\cal L}_c(y^i_{< t},\cdot,y^{i-1}_{>t};\tilde q^{k-1}).
\end{equation}
\end{lemma}

\begin{proof}
We first prove \eqref{set:inclu:translate}. It follows from line \ref{stat:prox.lagrangian.update.test} of \textproc{S-ADMM} that $(y_t,r_t,\varepsilon_t)$ is a $(\tau_1,\tau_2, 0;z^0)$-stationary solution of \eqref{ISO:problem} with $(\Gamma_s,
\Gamma_n)$ given by \eqref{def:ps}.
Hence, in view of Definition \ref{def:BB}
 and the definition of 
$(\tau_1,\tau_2, z^0)$ in line \ref{stat:prox.lagrangian.update.test} of \textproc{S-ADMM}, 
 we conclude that \eqref{set:inclu:translate} holds
and 
\begin{align*}
\|r_t\|^2+2\varepsilon_t &\overset{\eqref{ISO:Cond:2}}\leq \left(\sigma_1+\frac{\sigma_2}{2}\right)\frac{\lambda_t}{1+2\lambda_t}\|y_t-y_t^{i-1}\|^2+\frac{\sigma_2\lambda_t}{1+2\lambda_t}[ (\Gamma_s+\Gamma_n)(y_t^{i-1}) -(\Gamma_s+\Gamma_n) (y_t)] \\
&= \frac{\sigma_1\lambda_t}{1+2\lambda_t}\|y_t-y_t^{i-1}\|^2+\frac{\sigma_2\lambda_t}{1+2\lambda_t}\lambda_t (\Delta{\cal L}_c)_t^i(y_t),
\end{align*}
where the equality is due to
the fact that
 \eqref{def:ps} and \eqref{def:Pot:Fun:i:t} imply that
\begin{align*}
    (\Gamma_s+\Gamma_n)(y_t^{i-1}) - (\Gamma_s+\Gamma_n)(y_t)=\lambda_t (\Delta{\cal L}_c)_t^i(y_t) - \frac12 \|y_t - y^{i-1}_t\|^2.
\end{align*}

\end{proof}
The next result shows that the loop consisting of lines \ref{stat:prox.lagrangian.update.test} to  \ref{termnation:theta}  of \textproc{S-ADMM} ends and describes a property of its output. %Its proof is given in Appendix~\ref{technical lagrange multiplier}. 

\begin{lemma}\label{pro:lem:kong:new:Ine}
   Let $i \in {\cal I}_k$, $t \in \{1,\ldots,B\}$, and the triple $(\lambda_t,y_t, r_t)$ be obtained from lines~\ref{block:lam:t} and \ref{stat:prox.lagrangian.update.test} of \textproc{S-ADMM}.
   If $\lambda_t $ lies in the interval $(0,1/m_t)$,
   then $(\lambda_t,y_t, r_t)$ satisfies  
\begin{align}
\label{tes:SA:line:search:Ine:1}
(1+\sigma_2)(\Delta {\cal L}_c)^i_t(y_t)  &\ge  \frac{1}{4\lambda_t}\|y_t- y^{i-1}_t\|^2
+ \frac{c}{4} \|A_t (y_t-y^{i-1}_t)\|^2+\frac{\|r_t\|^2}{\lambda_t^2},
\end{align}
where $\sigma_2> 0$ is part of the input for \textproc{S-ADMM} and
$(\Delta {\cal L}_c)^i_t(y_t)$ is as in \eqref{def:Pot:Fun:i:t}.
\end{lemma}
\begin{proof}
    Let $i\in \Ik$, $t \in \{1,\ldots,B\}$,  and 
     $\lambda_t \in (0,1/m_t)$ be given.
     We first claim that, for every $u_t\in {\cal H}_t$,
     the quadruple $(\lambda_t,y_t, r_t, \varepsilon_t)$ 
     obtained in lines~\ref{block:lam:t} and \ref{stat:prox.lagrangian.update.test} of \textproc{S-ADMM} satisfies
\begin{align}\label{test:line:search:Ine:1}
    {\cal L}_c(y^i_{<t}, u_t,y^{i-1}_{>t};\tilde q^{k-1}) &-
{\cal L}_c(y^i_{<t}, y_{t},y^{i-1}_{>t};\tilde q^{k-1}) + \frac{1}{2\lambda_t}\|u_t-y_t^{i-1}\|^2 \nonumber\\
&\ge  \frac1{2\lambda_t}\|y_t- y^{i-1}_t\|^2 + \frac{c}{4} \|A_t ( u_t- y_t)\|^2-\frac{1}{\lambda_t} \left( \|r_t\| \|y_t-u_t\| + 2\varepsilon_t \right).
\end{align}
Since $\lambda_t \in (0,1/m_t)$, the matrix $B_t : = (1-\lambda_t m_t)I+\lambda_t cA_t^*A_t$ satisfies
    $B_t \succ 0$, and hence defines the norm
    $\|\cdot\|_{B_t}$ whose square satisfies 
    \begin{equation}\label{def:norm:Bt:Ine}
\|\cdot\|_{B_t}^2:=\langle\;\cdot\;, \, B_t(\cdot) \, \rangle 
\ge
\lambda_t c \|A_t (\cdot)\|^2.
\end{equation}
    Moreover, using assumption (A3), we can easily see that the function 
    \[
    \lambda_t {\cal L}_c(y_{<t}^{i},\cdot,y_{>t}^{i-1};\tilde q^{k-1})+\frac{1}{2}\|\cdot-y_t^{i-1}\|^2 - \inner{r_t}{u_t}
    \]
%line~\ref{stat:prox.lagrangian.update.test}  
    is $1$-strongly convex with respect to this norm.
    Using that the triple $(y_t,r_t,\varepsilon_t)$ satisfies 
    \begin{align*}
         r_t\in \partial_{\varepsilon_t} \left(\lambda_t \hat {\cal L}_{c}(y_{<t}^{i},\cdot,y_{>t}^{i-1};\tilde q^{k-1})+\frac{1}{2}\|\cdot-y_{t}^{i-1}\|^{2}+\lambda_t \Psi_t(\cdot)\right)(y_t), 
        \end{align*}
   due to \eqref{set:inclu:translate},  we can apply Lemma \ref{conv:result}  with $(\xi,\tau, Q, \hat\eta)=(1, 1, B_t, \varepsilon_t)$, to conclude that
    \begin{align*}
    \lambda_t &{\cal L}_c(y_{<t}^{i},u_t,y_{>t}^{i-1};\tilde q^{k-1})+\frac{1}{2}\|u_t-y_t^{i-1}\|^2-\frac{1}{4}\|u_t-y_t\|_{B_t}^2
    \\
    &\ge \lambda_t {\cal L}_c(y_{<t}^{i},y_t ,y_{>t}^{i-1};\tilde q^{k-1}) +\frac{1}{2}\|y_t- y_t^{i-1}\|^2-2\varepsilon_t+\langle r_t, u_t-y_t\rangle.
\end{align*}
The preliminary claim \eqref{test:line:search:Ine:1} follows
by dividing the previous inequality by $\lambda_t$, and using both \eqref{def:norm:Bt:Ine} and the Cauchy-Schwarz inequality. 


We now prove \eqref{tes:SA:line:search:Ine:1}. 
Using \eqref{test:line:search:Ine:1} with  $u_t=y^{i-1}_t$ and the definition of $(\Delta {\cal L}_c)^i_t(y_t)$ (see  \eqref{def:Pot:Fun:i:t}), we have
\begin{align}
\label{tes:SA:line:search:Ine}
& (\Delta {\cal L}_c)^i_t(y_t)  
\ge  \frac{1}{2\lambda_t}\|y_t- y^{i-1}_t\|^2 + \frac{c}{4} \|A_t (y^{i-1}_t-y_t)\|^2  -\frac{1}{\lambda_t}(\|r_t\| \|y_t-y^{i-1}_t\|+ 2\varepsilon_t).
\end{align}
Using the inequality $2 a b \le a^2 + b^2$ with $(a,b)=(2\|r_t\|, (1/2)\|y_t-y^{i-1}_t\|)$ 
and the condition on the error $(r_t, \varepsilon_t)$ as in \eqref{algo:eq.error.ineq},  we conclude that
\begin{align*}
   & \frac{1}{\lambda_t}\left( \frac{1}{\lambda_t} \|r_t\|^2+ \|r_t\| \|y_t-y^{i-1}_t\|+ 2\varepsilon_t \right) \\
   & \le
\frac{1}{\lambda_t} 
\left(\frac{1}{\lambda_t} \|r_t\|^2 + 2 \|r_t\|^2 +   \frac{1}{8} \|y_t-y^{i-1}_t\|^2 + 2 \varepsilon_t\right) \\
&= \frac{1}{\lambda_t}
%\left(\frac{\beta}{2} + \bar \chi \right) 
\left[(\lambda_t^{-1}+2)\|r_t\|^2
+ \frac{1}{8} \|y_t-y^{i-1}_t\|^2 + 2  \varepsilon_t\right] 
\\
&=
\frac{1}{\lambda_t} \left[(\lambda_t^{-1}+2)\|r_t\|^2 + 2 \varepsilon_t \right]  + \frac{1}{8\lambda_t} \|y_t-y^{i-1}_t\|^2 \\
&\overset{\eqref{algo:eq.error.ineq}}\le \frac{\sigma_1+(1/8)}{\lambda_t}\|y_t-y^{i-1}_t\|^2
+\sigma_2(\Delta {\cal L}_c)^i_t(y_t)\\
&\le \frac{1}{4\lambda_t}\|y_t-y^{i-1}_t\|^2+\sigma_2 (\Delta {\cal L}_c)^i_t(y_t),
\end{align*} 
where the last inequality is due to the assumption $\sigma_1\le 1/8$. The conclusion now follows by combining the previous  inequality with \eqref{tes:SA:line:search:Ine}.
\end{proof}


To shorten the formulas in this subsection, for each $i\in \mathbb{N}$ and $t \in \{1,\ldots,B\}$, we define the quantity
\begin{equation}
\label{def:Delta}
\Delta y^i_t := y^i_t - y^{i-1}_t.
\end{equation}


\begin{lemma}\label{lem:prop:Ine}
Let $i \in {\cal I}_k$, $t \in \{1,\ldots,B\}$, and the triple $(\lambda_t,y_t, r_t)$ be obtained from lines~\ref{block:lam:t} and \ref{stat:prox.lagrangian.update.test} of \textproc{S-ADMM}. 
Then, the loop consisting of lines \ref{stat:prox.lagrangian.update.test} to \ref{termnation:theta} terminates with a triple 
$(\lambda_t^i, y_t^i, r_t^i)\in \mathbb{R}^B_{++}  \times {\cal H}\times {\cal H}$ 
satisfying
\begin{eqnarray}\label{test:adativeness:Ine}
(1+\sigma_2)(\Delta {\cal L}_c)^i_t(y_t^i) \ge \frac{1}{4\lambda_t^i}\|\Delta y^i_t\|^2 + \frac{c}4 \|A_t \Delta y^i_t\|^2+\frac{\|r_t^i\|^2}{(\lambda_t^i)^2}
\end{eqnarray}
and 
\begin{equation}\label{test:q:adativeness:Ine}
\min \left\{ \frac{1}{2m_t},\gamma_t \right\}\leq \lambda^i_t\leq \gamma_t,
\end{equation}
where $(c,\gamma, \sigma_2)\in \mathbb{R}_{++}\times\mathbb{R}_{++}^B\times \mathbb{R}_{++}$ is part  of the input for \textproc{S-ADMM},  
$\Delta y_t^i$ is as in \eqref{def:Delta}, and $(\Delta {\cal L}_c)^i_t(\cdot)$ is as in \eqref{def:Pot:Fun:i:t}.
\end{lemma}


\begin{proof}
First, note that if
$(\lambda_t, y_t,r_t)$, as in line~\ref{stat:prox.lagrangian.update.test} of \textproc{S-ADMM}, is such that $\lambda_t \in (0,1/m_t)$, then it follows from 
Lemma~\ref{pro:lem:kong:new:Ine} that the loop consisting of lines \ref{stat:prox.lagrangian.update.test} to \ref{termnation:theta} terminates with
$(\lambda_t^i, y_t^i, r_t^i)= (\lambda_t, y_t, r_t)$.
% The result now follows from 
The above  observation, in conjunction with the facts  that the loop is initialized with $\lambda_t=\lambda_t^{i-1}$ and
$\lambda_t$ is halved every time a loop iteration fails to satisfy \eqref{tes:SA:line:search:Ine:1}, then imply that
\begin{equation*}
%\label{bound:q:lambda}
\min \left\{ \frac{1}{2m_t},\lambda_t^{i-1} \right\}\leq \lambda^i_t\leq \lambda_t^{i-1}.
\end{equation*}
This conclusion together with the fact that
$\lambda_t^0 = \gamma_t$
can now be easily seen to imply the conclusion of the lemma.
\end{proof}


 
The next result shows that $v^i$, computed in line~\ref{stat:def.vi.yi.lambdai.qi} of \textproc{S-ADMM}, is a stationary residual for the
pair $(y^i,q^i)$ and also establishes an upper bound for it.

\begin{lemma}    
\label{lemm:stationary:cond}
Let $\Ik$  be an epoch generated by \textproc{S-ADMM} and define
\begin{equation}\label{def:q:i:Ine}
q^i:=\tilde q^{k-1}+c(Ay^i-b) \quad  \forall i \in \Ik.
\end{equation}
Then, 
for every $i \in \Ik$, we have
\begin{equation}\label{lemma:residual:vi:Ine}
v^i  \in \nabla f (y^i)+ \partial_{\delta_i} \Psi(y^i) + A^* q^i
\end{equation}
and
\begin{align}\label{lemma:norm:residual:Ine}
\|v^{i}\|^2 +\delta_i &\le 
(\chi(\gamma)  + (1+\sigma_2) c B \|A\|_\dagger^2)(\Delta {\cal L}_c)^i
\end{align}
where $(c,\gamma, \sigma_2)\in \mathbb{R}_{++}\times\mathbb{R}_{++}^B\times\mathbb{R}_{++}$ is part  of the input for \textproc{S-ADMM}, $(v^i, \delta_i)$ is as in line \ref{stat:def.vi.yi.lambdai.qi} of \textproc{S-ADMM}, 
\begin{equation}\label{poten:func:i}
(\Delta {\cal L}_c)^i:= {\cal L}_c(y^{i-1};\tilde q^{k-1}) - {\cal L}_c(y^{i};\tilde q^{k-1})
\end{equation}
and 
\begin{equation}\label{eq:def.chi.gamma:Ine}
\chi(\gamma):= 2(1+\sigma_2)\left[1+12\|L\|^2\max(\gamma)+12(2\max (m)+\max (\gamma^{-1}))+2\sigma_1\right]+\sigma_2.
\end{equation}
\end{lemma}

\begin{proof}
We first prove that \eqref{lemma:residual:vi:Ine} holds. 
For each $t\in\{1,\ldots, B\}$, let $(\lambda_t^i, y_t^i, r_t^i,\varepsilon_t^i)$ be the quadruple obtained in line~\ref{termnation:theta} of \textproc{S-ADMM}. 
Using \eqref{set:inclu:translate} with $(\lambda_t, y_t, r_t,\varepsilon_t) =(\lambda_t^i, y_t^i,r^{i}_t,\varepsilon_t^i)$, we have
\begin{align}\label{eq:COA1}
\frac{r_t^i}{\lambda^i_t}
&\overset{\eqref{set:inclu:translate}}\in \nabla_{y_{t}}f(y_{< t}^i,y_{t}^i, y_{>t}^{i-1})+A_{t}^{*}\left[\tilde q^{k-1}+c[A(y_{< t}^i,y_{t}^i,y_{>t}^{i-1})-b]\right]+\frac{1}{\lambda^i_t}\Delta y_{t}^{i}+\partial_{(\varepsilon_t^i/\lambda^i_t)}\Psi_t(y_t^i)\nonumber \\
& \overset{\eqref{def:q:i:Ine}}=\nabla_{y_{t}}f(y_{< t}^i,y_{t}^i, y_{>t}^{i-1})+A_{t}^{*}\left({q}^{i} - c\sum_{s=t+1}^{ B}A_s \Delta y_{s}^{i}\right)+\frac{1}{\lambda^i_t}\Delta y_{t}^{i}+\partial_{(\varepsilon_t^i/\lambda^i_t)}\Psi_t(y_t^i), \nonumber
\end{align}
where in the inclusion above we used the well-known $\varepsilon$-subdifferential property that $\partial_{\varepsilon_t} \lambda_t \Psi(y_t) = \lambda_t \partial_{\varepsilon_t/\lambda_t} \Psi(y_t)$ (e.g., see \cite[Proposition 1.3.1]{lemarechal1993}). 
 By rearranging the above inclusion and using the definition of $(\Delta f)_t^i$, as in line~\ref{def:deltai} of \textproc{S-ADMM}, we have
\[
(\Delta f)_t^i+ \frac{r_t^i}{\lambda^i_t}+cA_t^*\sum_{s=t+1}^{ B}A_s \Delta y_{s}^{i}-\frac{1}{\lambda^i_t}\Delta y_{t}^{i}\in \nabla_{y_{t}}f(y^i)+\partial_{(\varepsilon_t^i/\lambda^i_t)}\Psi_t(y_t^i)+A_t^*q^i.
\]
Noting that
the left-hand side of the above inclusion equals $v_t^i$ (see line~\ref{stat:end.loop.vi} of \textproc{S-ADMM})
and using the well-known fact that
$\delta_i=(\varepsilon^i_1/\lambda_1^i) + \ldots +  (\varepsilon^i_B/\lambda_B^i)$ implies that
\[
\partial_{\delta_i}\Psi(y^i) \supset  \partial_{(\varepsilon_1^i/\lambda^i_1)}\Psi_1(y_1^i) \times \ldots \times
\partial_{(\varepsilon_B^i/\lambda^i_B)}\Psi_B(y_B^i),
\]
we conclude that
inclusion \eqref{lemma:residual:vi:Ine} holds.



We now prove \eqref{lemma:norm:residual:Ine}. It follows from the definition of $(\Delta f)_t^i$ and $v_{t}^{i}$  in lines \ref{def:deltai} and \ref{stat:end.loop.vi}  of \textproc{S-ADMM}, respectively, the triangle and Cauchy-Schwarz inequalities, and assumption (A4), that

\begin{align}\label{eq:bound:vi:first:Ine}
&\left\|v_{t}^{i}-\frac{r_t^i}{\lambda_t^i}\right\|^2  =\left\|\nabla_{y_{t}}f(y_{< t}^{i},y_{t}^{i}, y_{>t}^{i})-\nabla_{y_{t}}f(y_{< t}^i,y_{t}^{i}, y_{>t}^{i-1})+cA_{t}^{*}\sum_{s=t+1}^{ B}A_{s}\Delta y_{s}^{i}-\frac{1}{\lambda_t^i}\Delta y_{t}^{i}\right\|^2\nonumber\\
&\leq 3\left( \|\nabla_{y_{t}}f(y_{< t}^{i},y_{t}^{i}, y_{>t}^{i})-\nabla_{y_{t}}f(y_{< t}^i,y_{t}^{i}, y_{>t}^{i-1})\|^2+c^2\|A_t\|^2 \left\|\sum_{s=t+1}^{B}A_{s}\Delta y_{s}^{i} \right\|^2+\frac{1}{(\lambda^i_t)^2}\|\Delta y_{t}^{i}\|^2\right)\nonumber\\
&\overset{\eqref{eq:lipschitz_x}}\leq 3\left( L_t^2 \|y_{>t}^{i}-y_{>t}^{i-1}\|^2+c^2\|A_t\|^2 (B-t)\sum_{s=t+1}^{B}\|A_{s}\Delta y_{s}^{i} \|^2+\frac{1}{(\lambda^i_t)^2}\|\Delta y_{t}^{i}\|^2 \right) \nonumber \\
&\leq 3\left( L_t^2 \sum_{s=1}^B\|\Delta y^i_s\|^2+Bc^2\|A_t\|^2 \sum_{s=1}^{B}\|A_{s}\Delta y_{s}^{i} \|^2+\frac{1}{(\lambda^i_t)^2}\|\Delta y_{t}^{i}\|^2 \right).
\end{align}
 We now upper bound the first and third terms of the right-hand of \eqref{eq:bound:vi:first:Ine}. For the first term, we have
\begin{equation}\label{eq:bound:vi:interm1}
    \sum_{s=1}^B\|\Delta y^i_s\|^2 = \sum_{s=1}^B\lambda_s^i\cdot \frac{1}{\lambda_s^i}\|\Delta y^i_s\|^2 \overset{\eqref{test:q:adativeness:Ine}}\leq \sum_{s=1}^B\gamma_s\cdot \frac{1}{\lambda_s^i}\|\Delta y^i_s\|^2 \overset{\eqref{def:max:mu}}\leq \max(\gamma) \cdot \sum_{s=1}^B\frac{1}{\lambda_s^i}\|\Delta y^i_s\|^2.
\end{equation}
To bound the third term of \eqref{eq:bound:vi:first:Ine}, first note that for $t\in \{1,\ldots, B\}$, 
\begin{equation}\label{bound:inver:lam}
\frac{1}{\lambda^i_t}\overset{\eqref{test:q:adativeness:Ine}}\leq \left( \min \left\{ \frac{1}{2m_t},\gamma_t \right\} \right)^{-1} =  \max\left\{ 2m_t,\frac1{\gamma_t}\right\}
\overset{\eqref{def:max:mu}}\leq 2\max (m)+\max (\gamma^{-1})=:\hat{m},
\end{equation}
which yields
\begin{equation}\label{eq:bound:vi:interm2}
    \frac{1}{(\lambda^i_t)^2}\|\Delta y_{t}^{i}\|^2  = \frac{1}{\lambda^i_t}\cdot \frac{1}{\lambda^i_t}\|\Delta y_{t}^{i}\|^2 \leq\frac{\hat{m}}{\lambda^i_t}\|\Delta y_{t}^{i}\|^2 .
\end{equation}
Combining the inequalities \eqref{eq:bound:vi:first:Ine},  \eqref{eq:bound:vi:interm1}, \eqref{bound:inver:lam}, and \eqref{eq:bound:vi:interm2},  and using \eqref{test:adativeness:Ine}, we have
\begin{align}
 \left\|v_{t}^{i}-\frac{r_t^i}{\lambda_t^i}\right\|^2 &\leq
 3\left( L_t^2  \max(\gamma) \sum_{s=1}^B\frac{1}{\lambda_s^i}\| \Delta y^{i}_s\|^2+ Bc^2\|A_t\|^2\sum_{s=1}^{B}\|A_{s}\Delta y_{s}^{i} \|^2+\frac{\hat{m}}{\lambda^i_t}\|\Delta y_{t}^{i}\|^2\right).\nonumber \\
 &\overset{\eqref{test:adativeness:Ine}}\le 3\left[4 L_t^2  \max(\gamma)
 (1+\sigma_2)(\Delta {\cal L}_c)^i +  4Bc \|A_t\|^2 (1+\sigma_2)(\Delta {\cal L}_c)^i+4\hat{m}  (1+\sigma_2)(\Delta {\cal L}_c)^i_t \right]\nonumber \\
 &= 12 (1+\sigma_2) \left[ L_t^2  \max(\gamma)
(\Delta {\cal L}_c)^i +  Bc \|A_t\|^2 (\Delta {\cal L}_c)^i+\hat{m} (\Delta {\cal L}_c)^i_t \right],\nonumber
\end{align}
where $(\Delta {\cal L}_c)^i$ and $(\Delta {\cal L}_c)^i_t(\cdot)$ are as in \eqref{poten:func:i} and \eqref{def:Pot:Fun:i:t}, respectively.
Using the reverse triangle inequality in the left-hand side of the previous inequality, we conclude after simple manipulations that 
\begin{align}
 \|v_{t}^{i}\|^2-2\frac{\|r_t^i\|^2}{(\lambda_t^i)^2} \leq
 24(1+\sigma_2) \left[ L_t^2  \max(\gamma)
(\Delta {\cal L}_c)^i +  Bc \|A_t\|^2 (\Delta {\cal L}_c)^i+\hat{m} (\Delta {\cal L}_c)^i_t \right].\nonumber
\end{align}
Now, summing up the last inequality  from $t=1$ to $t=B$ and using \eqref{eq:block_norm} and \eqref{poten:func:i}, one has
\begin{align*}%\label{pri:stat:resi}
\|v^{i}\|^2&+\sum_{t=1}^B\frac{\varepsilon_t^i}{\lambda_t^i}  \overset{ \eqref{eq:block_norm}} \leq \left(\sum_{t=1}^B\frac{2\|r_t^i\|^2}{(\lambda_t^i)^2}+\frac{\varepsilon_t^i}{\lambda_t^i}\right)
+24(1+\sigma_2)\left[\|L\|^2\max(\gamma) +  Bc\|A\|_\dagger^2+\hat{m} \right](\Delta {\cal L}_c)^i\nonumber\\
&\overset{\eqref{test:adativeness:Ine}}\le\sum_{t=1}^B\frac{\varepsilon_t^i}{\lambda_t^i}+ 2(1+\sigma_2)[1+12(\|L\|^2\max(\gamma) +  Bc\|A\|_\dagger^2+\hat{m})](\Delta {\cal L}_c)^i\nonumber\\
&\le [4\sigma_1(1+\sigma_2)+\sigma_2](\Delta {\cal L}_c)^i+2(1+\sigma_2)[1+12(\|L\|^2\max(\gamma) +  Bc\|A\|_\dagger^2+\hat{m})](\Delta {\cal L}_c)^i,
\end{align*}
where the last inequality above is due to \eqref{algo:eq.error.ineq} with $(\lambda_t^i, y^{i}_t, \varepsilon_t^i)=(\lambda_t, y_t, \varepsilon_t)$ and \eqref{test:adativeness:Ine}.
The conclusion now follows from the previous inequality and the definitions of $\hat{m}$ and $\chi(\gamma)$ as in \eqref{bound:inver:lam} and \eqref{eq:def.chi.gamma:Ine}, respectively.
\end{proof}


The following result shows that
$\|v^i\|^2 = {\cal O}(T_i-T_{i-1})$, and hence that $\{\|v^i\|^2\}$ is summable.

\begin{lemma}\label{prop:stationary.vi.bound:Ine}
For any iteration $i\geq 1$ of \textproc{S-ADMM},  we have
\begin{eqnarray}\label{eq:Ti.Ti-1.bound:Ine}
\frac{1}{\chi (\gamma) + (1+\sigma_2) c B \|A\|_\dagger^2 }\left(\|v^i\|^2 +\delta_i\right)\leq  T_i-T_{i-1},
\end{eqnarray}
where $( \delta_i, T_i)$ is as in lines \ref{stat:def.vi.yi.lambdai.qi} and \ref{def:T:i}  of \textproc{S-ADMM} 
(with
$T_0:=0$ by convention),
$(\gamma,c)\in \mathbb{R}_{++}^B\times\mathbb{R}_{++}$ is part  of the input for \textproc{S-ADMM}, and $\chi (\gamma)$ is as in \eqref{eq:def.chi.gamma:Ine}.
As a consequence,
$T_i\le T_j$ for any two iterations $i<j$ of \textproc{S-ADMM}.
\end{lemma}

\begin{proof}
Consider an arbitrary iteration index $i$ of \textproc{S-ADMM} and assume that
the $k$-th epoch $\Ik$ is the one that contains this index. Then,
\begin{align*}
 &(\Delta {\cal L}_c)^i\overset{\eqref{lemma:norm:residual:Ine}}\geq \frac{1}{[\chi(\gamma)  + (1+\sigma_2) c B \|A\|_\dagger^2 ]}\left(\|v^i\|^2 +\delta_i \right).
\end{align*}
Thus, it follows from the definition of $(\Delta {\cal L}_c)^i$ as in \eqref{poten:func:i} and Lemma~\ref{lemma:trivial:1} with $(i,j)=(i-1,i)$, that the left-hand side of the previous inequality is equal to $T_{i}-T_{i-1}$, and this concludes the proof.
\end{proof}


We now present the main result of this subsection, which establishes an upper bound on the number of
epochs generated by \textproc{S-ADMM}.

\begin{prop}\label{lem:number.of.cycles}
The total number of epochs performed by \textproc{S-ADMM} is bounded by
\begin{equation}\label{def:bar:K:Ine}
\bar K :=  \left\lceil\frac{\chi (\gamma) + (1+\sigma_2) c B \|A\|_\dagger^2 }{\alpha}\right\rceil,
\end{equation}
where  $(\gamma,c,\sigma_2)\in \mathbb{R}_{++}^B\times\mathbb{R}_{++}\times\mathbb{R}_{++}$ are part  of the input for \textproc{S-ADMM}, and $\chi(\gamma)$ is as in \eqref{eq:def.chi.gamma:Ine}.
\end{prop}

\begin{proof}
Assume for the sake of contradiction, that \textproc{S-ADMM} generates an epoch $\Ik$ such that $k \ge  \bar K+1$. 
Summing the inequality \eqref{eq:Ti.Ti-1.bound:Ine} from $i=1$ to $i=i_{k-1}^+$ and using the fact that $T_0=0$ and $T_{i_{k-1}^+}=\tilde T_{k-1}$, due to Lemma~\ref{lemma:trivial:1}(a), we have
\begin{align}\label{eq:v:i:prop:Ine}
    \sum_{i=1}^{i_{k-1}^+}\left(\|v^{i}\|^2+\delta_i\right)
&\overset{\eqref{eq:Ti.Ti-1.bound:Ine}} \le [\chi (\gamma) + (1+\sigma_2) c B \|A\|_\dagger^2 ][ T_{i_{k-1}^+}-T_0] =[\chi (\gamma) + (1+\sigma_2) c B \|A\|_\dagger^2 ] 
 \tilde T_{k-1}.
\end{align}
Since \textproc{S-ADMM} did not terminate during epochs ${\cal I}_1,\ldots,{\cal I}_{k-1}$, it follows from its termination criterion in line~\ref{cond:vi:stop} that 
$\|v^i\|^2+\delta_i > \rho^2$ for every
iteration $i \le i_{k-1}^+$. This observation and \eqref{eq:v:i:prop:Ine} then imply that
\begin{align*}%\label{bound:vi:K}
\rho^2
&< \frac{1}{i_{k-1}^+} \sum_{i=1}^{i_{k-1}^+}\left(\|v^{i}\|^2+\delta_i\right)
\overset{\eqref{eq:v:i:prop:Ine}}\leq [\chi (\gamma) + (1+\sigma_2) c B \|A\|_\dagger^2 ]\frac{\tilde T_{k-1}}{i_{k-1}^+}\\
&\leq [\chi (\gamma) + (1+\sigma_2) c B \|A\|_\dagger^2 ]\frac{\rho^2}{(k-1)\alpha}\overset{\eqref{def:bar:K:Ine}}\le \frac{\bar K}{k-1}\rho^2,
\end{align*}
where the second last inequality is due to the last inequality  of
Lemma~\ref{lemma:trivial:1}(a) with $k=k-1$ .
Since by assumption $k-1 \ge \bar K$,
the above inequality yields the desired contradiction.
\end{proof}




%%%%%%%%%%%%%%%%%%%%%%%%%%%SUBROUTINE ANALYSIS
\subsection{Step 2: Bounding the Epoch Size}
\label{subsec:totaliteration}
The goal of this subsection is to prove a uniform bound on sizes of the epochs $\mathcal{I}_1,\mathcal{I}_2,\ldots$. The first result of this subsection, which  establishes a bound on the difference of the augmented Lagrangian function evaluated at two different pairs, will be used a few times later on.



\begin{lemma}\label{lem:lowerbound.L}
Given triples $(z^j, u^j, c) \in {\cal H} \times \mathbb{R}^l \times  \mathbb{R}_{++}$ with $j=1,2$. If $\bar \zeta = \max_j  \|u^j\|$, then 
\begin{equation}\label{def:diff:lagrangian}
{\cal L}_{c}(z^1; u^1)
- {\cal L}_{c}(z^2 ; u^2 )
\le \overline{F}-\underline{F}
+ \frac{(c\|Az^1-b\| + \bar \zeta)^2}{2c}
\end{equation}
where  $(\overline F,\underline{F} )$ is as in \eqref{def:damH}.
\end{lemma}

\begin{proof}
Using the definitions of ${\cal L}_c(\cdot\,;\,\cdot)$ (with $(\theta,\chi)=(0,1))$ and $\underline F$ as in \eqref{DP:AL:F} and \eqref{def:damH}, respectively, we have
\begin{align*}
{\cal L}_{c}(z^2 ; u^2)-\underline F &\overset{\eqref{def:damH}}\geq  {\cal L}_{c}(z^2 ; u^2)-(f+h)(z^2) \\
&\overset{\eqref{DP:AL:F}}=\langle u^2, A z^2-b\rangle +\frac{c}{2}\|A z^2-b\|^2=\frac{1}{2}\left\|\frac{u^2}{\sqrt{c}}+\sqrt{c}(A z^2-b)\right\|^2-\frac{\|u^2\|^2}{2c} \ge -\frac{\bar \zeta^2}{2c},
\end{align*}
where the last inequality is due to the definition of $\bar \zeta$. 
On the other hand, using the definitions of ${\cal L}_{c}(\, \cdot \,;\, \cdot \, )$ (with $(\theta,\chi)=(0,1))$ and $\bar F$ as in \eqref{DP:AL:F} and \eqref{def:damH},
respectively, and the Cauchy-Schwarz inequality, we have
\begin{align*}
{\cal L}_{c}(z^1; u^1) - \overline F 
&\overset{\eqref{def:damH}}\le {\cal L}_{c}(z^1; u^1)-(f+h)(z^1)  \overset{\eqref{DP:AL:F}}= \langle u^1, A z^1 -b\rangle +\frac{c}{2}\|A z^1-b\|^2\\
&\le \|u^1\|\|A z^1-b\|+\frac{c}{2}\|A z^1-b\|^2 \le \bar \zeta\|A z^1-b\|+\frac{c}{2}\|A z^1-b\|^2,
\end{align*}
where the last inequality is due to the definition of $\bar \zeta$.
Combining the above two relations we then conclude that \eqref{def:diff:lagrangian} holds.
\end{proof}

For any $k\geq 1$, let
\begin{equation}\label{def:I:k:C1}
    {\cal I}_k(C) := \{i\in {\cal I}_k:\|v^{i}\|^2+\delta_i\leq C^2\},
\end{equation}
where $C>0$ is part of the input for \textproc{S-ADMM} and $(v^i, \delta_i)$ is as in line \ref{stat:def.vi.yi.lambdai.qi} of \textproc{S-ADMM}. 
The next result shows that the Lagrange multiplier $q^j$ remains bounded 
as long as $j\in \Ik(C)$.
It also shows that if $i \in \Ik(C)$ and epoch ${\Ik}$ does not terminate  at the $i$-th iteration, then it generates another index 
$j\in \Ik(C)$ such that
$0<j-i = {\cal O}(c)$.

\begin{lemma}\label{lem:inner.v.bound}
The following statements about an epoch $\Ik$ generated by \textproc{S-ADMM} hold:
\begin{enumerate}

\item[(a)] for every $j \in \Ik$, we have
\begin{equation}\label{eq:Tj:T}
T_j - \tilde T_{k-1}
\le \pi_{k-1}
\end{equation}
where 
\begin{equation}\label{def:Gamma:0}
\pi_{k-1} := \overline{F}-\underline{F}+ \frac{(c\|A\tilde y^{k-1}-b\|+\|\tilde q^{k-1}\|)^2}{2c};
\end{equation}

\item[(b)] if  either $i = i_{k-1}^+$ or $i \in \Ik(C)$ and $\Ik$ does not terminate at  the $i$-th iteration,
then there exists $j \in \Ik(C)$ such that
\begin{equation}\label{eq:UpperSSi}
0 < j-i \le 
\left\lceil\frac{\chi (\gamma) + (1+\sigma_2) c B \|A\|_\dagger^2}{C^2}\pi_{k-1}\right\rceil,
\end{equation}
where $\chi(\gamma)$ is as in \eqref{eq:def.chi.gamma:Ine} and
$\sigma_2$ is part of the input for \textproc{S-ADMM};



\item[(c)] if $\tilde q^{k-1}\in A(\mathbb{R}^n)$ and  $\|\tilde q^{k-1}\|\le \kappa_p$, then for every $j \in {\mathcal{I}}_k(C)$,
the pair $(y^j,q^j)$, where $q^j$ as in \eqref{def:q:i:Ine}, satisfies
\begin{equation}\label{eq:UpperpF}
q^j \in A(\mathbb{R}^n),  \quad \|q^j\| \le \kappa_p \quad \text{and} \quad  c\|Ay^j-b\|
 \le 2\kappa_p.
\end{equation}

%\vspace{0.5cm}
%\textcolor{blue}{\textbf{\eqref{eq:UpperpF} is used to show \eqref{eq:feasible}.}}

\end{enumerate}
\end{lemma}
\begin{proof}
(a) Assume that $j\in\Ik$. Using the definition of $T_j$ as in line~\ref{def:T:i} of \textproc{S-ADMM}, and Lemma~\ref{lem:lowerbound.L} with 
$(u^1,u^2)=(\tilde q^{k-1},\tilde q^{k-1})$ and  $(z^1,z^2)=(\tilde y^{k-1}, y^{j})$, we have
\begin{align*}
T_{j}- \tilde T_{k-1} &= {\cal L}_c(\tilde y^{k-1};\tilde q^{k-1}) - {\cal L}_c(y^j;\tilde q^{k-1})
\overset{\eqref{def:diff:lagrangian}}\leq  \overline{F}-\underline{F}+\frac{(c\|A\tilde y^{k-1}-b\|+\|\tilde q^{k-1}\|)^2}{2c}\overset{\eqref{def:Gamma:0}}=  \pi_{k-1},
\end{align*}
which yields \eqref{eq:Tj:T}.

(b) Assume that $i \in \Ik(C)\cup\{i_{k-1}^+\}$ is an iteration for which the termination criterion of the $k$-th epoch is not satisfied
 and assume for the sake of contradiction that $j \notin \Ik(C)$ for every $j \in
 \{i+1,\ldots, i+s\}$, where
\begin{equation}\label{def:vartheta}
 s:= \left\lceil\frac{\chi (\gamma) + (1+\sigma_2) c B \|A\|_\dagger^2}{C^2}\pi_{k-1}\right\rceil.
 \end{equation}
Since by assumption the $k$-th epoch does not stop at
iteration $i$
and it can only stop
at some iteration $j$ lying in $\Ik(C)$ (see line~\ref{stat:begin.test.cond} of \textproc{S-ADMM}), we conclude that
every $j \in \{i+1,\ldots, i+s\}$
lies in $\Ik$ and $\|v^j\|^2 +\delta_j>C^2$. 
Using this conclusion, \eqref{eq:Tj:T},
Lemma~\ref{prop:stationary.vi.bound:Ine}, the fact
% s that
% $i_{k-1}^++1=i_k^-$ and
$\tilde T_{k-1}=T_{i^+_{k-1}}$ (see  Lemma~\ref{lemma:trivial:1}(a)), 
and the nondecreasing property of the sequence $T_i$ (see Lemma~\ref{prop:stationary.vi.bound:Ine}), we conclude that 
\begin{align*}
   & \pi_{k-1}\overset{\eqref{eq:Tj:T}}\ge T_{i+s}- \tilde T_{k-1}
   =T_{i+s}- T_{i_{k-1}^+}
   \ge T_{i+s}-T_i=\sum_{l=i+1}^{i+s}(T_l-T_{l-1})\\
   &\overset{\eqref{eq:Ti.Ti-1.bound:Ine}}\ge \frac{1}{\chi (\gamma) + (1+\sigma_2) c B \|A\|_\dagger^2}\sum_{l=i+1}^{i+s}(\|v^l\|^2+\delta_l) 
   >\frac{sC^2} {\chi (\gamma) + (1+\sigma_2) c B \|A\|_\dagger^2} \ge \pi_{k-1},
 \end{align*}
 where the last inequality is due to  \eqref{def:vartheta}.
 Since the above inequality is not possible,
 statement (b) follows.

 (c)  The inclusion in \eqref{eq:UpperpF} 
follows from the definition of $q^j$ in \eqref{def:q:i:Ine} and the assumption that $\tilde q^{k-1}\in A(\mathbb{R}^n)$.
We now prove the first inequality in \eqref{eq:UpperpF}.
Relations \eqref{def:q:i:Ine} and \eqref{lemma:residual:vi:Ine}
imply that the triple $(z,q,r)=(y^j, q^j, v^j  - \nabla f (y^j))$ satisfies the 
conditions in  \eqref{eq:cond:Lem:A1} of Lemma~\ref{lem:qbounds-2}
with $(\chi, \delta)=(c, \delta_j)$, and hence
the conclusion of this lemma implies that 
\[
 \|q^j\| \leq \max\left\{\|\tilde q^{k-1}\|,\frac{2D_h(M_h+\|v^j-\nabla f(y^j)\|)+\delta_j}{\bar d \nu^{+}_A} \right\},
\]
where $M_h,$ $\bar d>0$ and $D_h$ are as in assumptions (A5), (A6) and \eqref{def:damH}, respectively, and $\nu^+_A$ denotes  the smallest positive singular value of $A$. 
This inequality together with the triangle inequality, the facts that $\|v^j\|\le C$, $\delta_j\le C^2$, and $\|\nabla f(y^j)\|\le \nabla_f,$ due to \eqref{def:I:k:C1} and \eqref{def:damH}, respectively, and the assumption that $\|\tilde q^{k-1}\|\le \kappa_p$, imply that 
\begin{align*}
  \|q^j\|  \overset{\eqref{def:damH}}\le \max\left\{\kappa_p,\frac{2D_h(M_h+C +\nabla_f)+C^2}{\bar d \nu^{+}_A} \right\}  \overset{\eqref{eq:def.Gamma.D3}}= \kappa_p,
\end{align*}
and hence the first inequality in
\eqref{eq:UpperpF} holds.
%{\bf what about $\nabla_f$????"? how do you show $q^i$ is in $A(\mathbb{R}^n)$}
Moreover, using the definition of $q^j$ in \eqref{def:q:i:Ine}, the first inequality in \eqref{eq:UpperpF}, and the assumption that $\|\tilde q^{k-1}\|\le \kappa_p$,
we have
\[
c\|Ay^j-b\|\overset{\eqref{def:q:i:Ine}}=\|q^j-\tilde q^{k-1}\|\le \|q^j\|+\|\tilde q^{k-1}\|\overset{\eqref{eq:UpperpF}}\le 2\kappa_p,%\leq \frac{Q_0}{2},
\]
and hence  
the second inequality in \eqref{eq:UpperpF} also holds.
\end{proof}

The next result shows that every epoch of \textproc{S-ADMM} ends. 

\begin{lemma}\label{trivial:lemma}
Every epoch $\Ik$ generated by \textproc{S-ADMM} terminates and the following relations hold:
 \begin{equation}\label{eq:Lagrange:monotonicity}
   {\cal L}_c(\tilde y^{k};\tilde q^{k-1})\le {\cal L}_c(y^i;\tilde q^{k-1})\quad  \forall i \in \Ik,
\end{equation} 
\begin{equation}\label{eq:lagra:update:tilde:k}
{\cal L}_c(\tilde y^k;\tilde q^{k-1})+ \frac{\|\tilde q^k-\tilde q^{k-1}\|^2}{c}={\cal L}_c(\tilde y^k;\tilde q^{k}).
\end{equation} 
\end{lemma}
%\textcolor{blue}{\textbf{\eqref{eq:Lagrange:monotonicity} and \eqref{eq:lagra:update:tilde:k} are used in Lemma~\ref{lem:Ikfinite}(b)}}

\begin{proof}
 We first show that every epoch $\Ik$ generated by \textproc{S-ADMM} terminates. Assume for the sake of contradiction that ${\cal I}_k$ is infinite.
 Lemma~\ref{lem:inner.v.bound}(b) then implies that  
${\cal I}_k(C)$ is also infinite.
This in turn implies that
$i<(\alpha k T_i)/\rho^2$ 
for every $i \in {\cal I}_k(C)$
since otherwise
the $k$-epoch would terminate at the first iteration $i \in {\cal I}_k(C)$ that violates this condition
(see line~\ref{stat:begin.test.cond} of \textproc{S-ADMM}).
This conclusion together with \eqref{eq:Tj:T}
then imply that any $i \in {\cal I}_k(C)$ satisfies
% this observation and the fact that inequality in \eqref{eq:Tj:T} with $j=i$ holds, then imply that
\begin{align*}
i< \frac{\alpha k }{\rho^2}T_i\overset{\eqref{eq:Tj:T}}\leq \frac{\alpha k}{\rho^2}\left( \tilde T_{k-1} +\pi_{k-1}\right),
\end{align*}
and  hence that $\Ik$
is finite as the right-hand side of the above inequality is independent of $i \in \Ik$.
Since this contradicts our
previous assumption that
$\Ik$ is infinite, we conclude that $\Ik$ terminates.

We now prove  \eqref{eq:Lagrange:monotonicity}. First, observe that,
by Lemma~\ref{lemma:trivial:1}(a), we have $\tilde y^k=y^{i_k^+}$.
Hence, it follows from Lemma~\ref{lemma:trivial:1}(b) with $i=i_k^+$ and $j=i$ that ${\cal L}_c(y^i;\tilde q^{k-1}) - {\cal L}_c(\tilde y^{k};\tilde q^{k-1})= \tilde T_{k} - T_i.$ 
Inequality \eqref{eq:Lagrange:monotonicity} now follows from the last conclusion of Lemma~\ref{prop:stationary.vi.bound:Ine}.  
Finally, the identity in \eqref{eq:lagra:update:tilde:k} follows from the definition of the augmented Lagrangian function in \eqref{DP:AL:F} (with $(\theta,\chi)=(0,1))$ and the fact that $\tilde q^k =  \tilde{q}^{k-1} + c(A\tilde y^k-b),$ due to line~\ref{stat:test.i.qi.ti.updates} of \textproc{S-ADMM}. 
\end{proof}

% The next result shows that if \textproc{S-ADMM} does not terminate at the end of its $(k-1)$-th cycle %and if $\tilde q^{k-1}$ satisfies some assumptions, 
% then the $k$-cycle ends. 
The next result provides some preliminary 
bounds on the Lagrangian multiplier sequence $\{\tilde q^k\}$, the feasibility residual sequence $\{\|A\tilde y^k-b\|\}$, and the sequence $\{T_i\}$.



\begin{lemma}\label{lem:Ikfinite}
 If the final iterate of the $(k-1)$-th epoch
satisfies the conditions that  $\tilde q^{k-1}\in A(\mathbb{R}^n)$ and  $\|\tilde q^{k-1}\| \leq\kappa_p$, then the following statements hold:
 \begin{itemize}
     \item [(a)]
 the pair $(\tilde y^k,\tilde q^k)$ satisfies
\begin{equation}\label{eq:feasible}
    \tilde q^{k}\in A(\mathbb{R}^n), \quad \|\tilde q^k\| \le \kappa_p \quad\text{and}\quad  c\|A\tilde y^k-b\| \le 2\kappa_p;
\end{equation}
%\vspace{0.5cm}
%\textcolor{blue}{\textbf{\eqref{eq:feasible} is used to show \eqref{eq:Ti:Gamma:k-1}, Lemma~\ref{lem:inner.I.k}(a) and Theorem~\ref{thm:static.complexity}(b)-(c).}}

% where  $\tilde q^k$ is as in line~\ref{stat:test.i.qi.ti.updates} of \textproc{S-ADMM} and $\tilde y^k$ is as in Lemma~\ref{lemma:trivial:1}(a);

\item[(b)] for every $i\in \Ik(C)$, there holds
\begin{align}\label{eq:Ti:Gamma:k-1}
 T_i &\leq \tilde T_{k-1} + \frac{4\kappa_p^2}{c} + \Delta_k,
\end{align}
where 
\begin{equation}\label{def:Delta:k}
\Delta_k := {\cal L}_c(\tilde y^{k-1};\tilde q^{k-1}) -{\cal L}_c(\tilde y^k;\tilde q^{k});
\end{equation}

\item[(c)] there holds
\begin{equation}\label{eq:tT:Gamma0}
 \tilde T_k - \tilde T_{k-1} \le \frac{4\kappa_p^2}{c}+\Delta_k,
\end{equation}
where $\tilde T_k$ is as in Lemma~\ref{lemma:trivial:1}(a).
\end{itemize}

\end{lemma}

\begin{proof}
Assume that the conditions $\tilde q^{k-1}\in A(\mathbb{R}^n)$ and  $\|\tilde q^{k-1}\| \leq\kappa_p$ hold.

(a) The conclusion that the pair $(\tilde y^k,\tilde q^k)$ satisfies \eqref{eq:feasible}  follows from \eqref{eq:UpperpF} with $j=i_k^+$ and the fact that $(\tilde y^k,\tilde q^k)=(y^{i_{k}^+}, q^{i_k^+})$.

(b) Using the definition of $T_i$ as in line~\ref{def:T:i} of \textproc{S-ADMM}, inequality \eqref{eq:Lagrange:monotonicity}, and the identity in \eqref{eq:lagra:update:tilde:k}, we have
\begin{align*}%\label{property:tilde:T:k}
 T_i - \tilde T_{k-1}
 &=   {\cal L}_c(\tilde y^{k-1};\tilde q^{k-1}) - {\cal L}_c(y^i;\tilde q^{k-1})\nonumber
 \overset{\eqref{eq:Lagrange:monotonicity}}\leq  {\cal L}_c(\tilde y^{k-1};\tilde q^{k-1}) - {\cal L}_c(\tilde y^k;\tilde q^{k-1}) \nonumber\\
 &\overset{\eqref{eq:lagra:update:tilde:k}}=  {\cal L}_c(\tilde y^{k-1};\tilde q^{k-1}) - {\cal L}_c(\tilde y^k;\tilde q^{k}) + \frac{\|\tilde q^k-\tilde q^{k-1}\|^2}{c}.
\end{align*} 
Inequality \eqref{eq:Ti:Gamma:k-1}
now follows from the above identity,
the definition of $\Delta_k$ in \eqref{def:Delta:k}, the triangle inequality for norms, and the first inequality in \eqref{eq:feasible}.

(c) Inequality  \eqref{eq:tT:Gamma0} follows from  \eqref{eq:Ti:Gamma:k-1} with $i=i_k^+$ and the fact that $\tilde T_k = T_{i_k^+}$ (see Lemma~\ref{lemma:trivial:1}(a)).
\end{proof}

The main purpose of the next result is to
provide a preliminary bound on the cardinality of the $k$-th epoch.

\begin{lemma}\label{lem:inner.I.k}
%\emph{(Cycle-Size)}
Assume that the initial Lagrange multiplier satisfies 
$p\in A(\mathbb{R}^n)$ and  $\|p\| \leq\kappa_p$, and define
\begin{equation}\label{eq:Gamma:x:c}
\pi(x;c) := \overline{F}-\underline F+\frac{(\|Ax-b\|+3\kappa_p)^2}{2c}, 
\end{equation}
where $(x,c)$ is part of the input for \textproc{S-ADMM}. 
Then, the following statements about any epoch ${\Ik}$ generated  \textproc{S-ADMM} hold:
\begin{itemize}
\item[(a)] 
%it terminates and its final iterate $(\tilde y^k,\tilde q^k)$ satisfies \eqref{eq:feasible}; moreover,
$\pi_{k-1} \le \pi(x;c)$, where $\pi_{k-1}$ is as in \eqref{def:Gamma:0};
\item[(b)]
there hold
\begin{equation}\label{eq:sum:Delta:l}
\sum_{l=1}^k \Delta_l \le \pi(x;c), \quad \sum_{l=1}^k l \Delta_l \le k\pi(x;c)
\end{equation}
where $\Delta_l$ is as in \eqref{def:Delta:k}; 
moreover, 
\begin{equation}\label{eq:tT:Gamma}
 \tilde T_k \le \frac{4k\kappa_c^2}{c} + 
 \pi(x;c);
 \end{equation}
 \item[(c)] 
its length satisfies
\begin{equation}\label{eq:sizecy}
|{\cal I}_k| \le\frac{\alpha}{\rho^2}\left(\frac{8k\kappa_p^2}{c} + \pi(x;c) +  k \Delta_k\right)+
1+
\frac{(\chi (\gamma) + (1+\sigma_2) c B \|A\|_\dagger^2)\pi(x;c)}{C^2},
\end{equation}
where $\chi(\gamma)$ is as in \eqref{eq:def.chi.gamma:Ine} and
$\sigma_2$ is part of the input for \textproc{S-ADMM}.
\end{itemize}
\end{lemma}

\begin{proof}
(a) %The first two results follow from Lemma~\ref{lem:Ikfinite}(a), the fact that $\tilde q^0=p$, and a straightforward induction argument.
Recalling the definitions of $\pi_{k-1}$ and $\pi(x;c)$ in \eqref{def:Gamma:0} and 
\eqref{eq:Gamma:x:c}, respectively,  the inequality $\pi_{k-1}\le \pi(x;c)$ for $k=1$ follows from the facts that $\tilde y^0=x$ and $\tilde q^0=p$ (see line~\ref{initialcondRS} of \textproc{S-ADMM}) and the assumption $\|p\|\le \kappa_p$, and for $k \ge 2$ follows from both inequalities in \eqref{eq:feasible}.%, which holds in view of the second part of statement (a).
 
(b) We first claim that ${\cal L}_c(\tilde y^{l-1};\tilde q^{l-1})  -  {\cal L}_c(\tilde y^{k};\tilde q^{k}) \le \pi(x;c)$ for every $l\in \{1,\ldots,k\}.$ Using the fact that \eqref{eq:feasible}  implies that
$\|\tilde q^l \| \le \kappa_p$
and
$c \|A\tilde y^l-b\| \le 2 \kappa_p$ for every $l \in \{1,\ldots,k\}$, 
Lemma~\ref{lem:lowerbound.L} with 
$(u^1, u^2)=(\tilde q^{l-1}, \tilde q^{k})$, $(z^1, z^2)=(\tilde y^{l-1},\tilde y^{k})$, the assumption that $\|p\|\le \kappa_p$, 
%and the definition of $\pi_{l-1}$ in  \eqref{def:Gamma:0},
we conclude that 
\[{\cal L}_c(\tilde y^{l-1};\tilde q^{l-1})  -  {\cal L}_c(\tilde y^{k};\tilde q^{k}) \le \overline{F}-\underline{F}
+\frac{(c\|A\tilde y^{l-1}-b\| + \kappa_p)^2}{2c}\le \pi(x;c)
\] 
for every $l\in \{1,\ldots,k\},$ where the last inequality above follows by repeating the same argument as in statement (a).
%Combining this latter inequality with $\pi_{l-1}\le \pi(x;c)$ from statement (a), 
Thus, we conclude that the claim holds. 
We now prove the first inequality in \eqref{eq:sum:Delta:l}. Using the definition of $\Delta_l$ in \eqref{def:Delta:k}, we have
    \[
    \sum_{l=1}^k \Delta_l=\sum_{l=1}^k\left({\cal L}_c(\tilde y^{l-1};\tilde q^{l-1}) - {\cal L}_c(\tilde y^l;\tilde q^{l})\right)
    =
    {\cal L}_c(\tilde y^0;\tilde q^0) - {\cal L}_c(\tilde y^k;\tilde q^{k})\le \pi(x;c),
    \]
where the last inequality above follows from the previous claim with $l=1$ and
the fact that $(\tilde y^0,\tilde q^0)=(x,p)$ (see line~\ref{initialcondRS} of \textproc{S-ADMM}). We now prove the second inequality in \eqref{eq:sum:Delta:l}. Using the identity in \eqref{def:Delta:k} and simple algebraic manipulations, we have
\begin{align*}%\label{eq:k:Delta:k:cons}
\sum_{l=1}^{k}  l \Delta_l &\overset{\eqref{def:Delta:k}}= \sum_{l=1}^{k}  l[{\cal L}_c(\tilde y^{l-1};\tilde q^{l-1}) -{\cal L}_c(\tilde y^l;\tilde q^{l})]\nonumber\\
&=\sum_{l=1}^{k} {\cal L}_c(\tilde y^{l-1};\tilde q^{l-1}) + \sum_{l=1}^{k} [ (l-1){\cal L}_c(\tilde y^{l-1};\tilde q^{l-1}) - l {\cal L}_c(\tilde y^{l};\tilde q^{l})]\nonumber\\
&=\sum_{l=1}^{k} ({\cal L}_c(\tilde y^{l-1};\tilde q^{l-1}))  - k {\cal L}_c(\tilde y^{k};\tilde q^{k})=\sum_{l=1}^{k} \left({\cal L}_c(\tilde y^{l-1};\tilde q^{l-1})  -  {\cal L}_c(\tilde y^{k};\tilde q^{k})\right)\le k\pi(x;c),
\end{align*} 
where the last inequality above follows from the previous claim. 

Inequality \eqref{eq:tT:Gamma} follows by summing inequality in \eqref{eq:tT:Gamma0} from $k=1$ to $k=k$, using the fact that $(\tilde y^0,\tilde q^0,\tilde T_0)=(x,p,0)$ (see line~\ref{initialcondRS} of \textproc{S-ADMM}), and the first inequality in \eqref{eq:sum:Delta:l}.

    (c) We now prove \eqref{eq:sizecy}.  First, we recall from Lemma~\ref{trivial:lemma} that $\Ik$ is finite. Let $i$ be the largest index in $\Ik(C)\cup \{i_{k-1}^+\}$ satisfying $i<i_k^+$ (with the convention that $i_0^+=0$). Then, since $i$ and $i_k^+$ are consecutive indices in $\Ik(C)$, it follows from Lemma~\ref{lem:inner.v.bound}(b) and the fact that $\pi_{k-1}\le \pi(x;c)$ from statement (a), that
\begin{equation}\label{eq:FS} 
|{\cal I}_k| =i_k^+ - i_{k-1}^+ = ( i - i_{k-1}^+) + (i_k^+ - i) \overset{\eqref{eq:UpperSSi}}\leq i-i_{k-1}^+ + 1+\frac{(\chi (\gamma) + (1+\sigma_2) c B \|A\|_\dagger^2 )\pi(x;c)}{C^2}.
\end{equation}
If $i=i_{k-1}^+$ then \eqref{eq:FS} implies that \eqref{eq:sizecy} holds. Suppose now that $i\in \Ik(C)$. Using the facts that
$i \in \Ik(C)\setminus \{i_k^+\}$
and 
$i_k^+$ is the only index in $\Ik(C)$
satisfying the second condition in line~\ref{stat:begin.test.cond} of \textproc{S-ADMM}, we then conclude that
\begin{align*}\label{eq:rho:i:tilde:T}
\frac{\rho^2 i}{ \alpha} &<  kT_i
\overset{\eqref{eq:Ti:Gamma:k-1}}\leq k\left( \tilde T_{k-1} + \frac{4\kappa_p^2}{c}+\Delta_k \right) = (k-1)\tilde T_{k-1}+\tilde T_{k-1} + \frac{4k\kappa_p^2}{c}+k\Delta_k\\
&\overset{\eqref{eq:lema1:test}}\le \frac{\rho^2i_{k-1}^+}{\alpha}+\tilde T_{k-1}+ \frac{4k\kappa_p^2}{c}+k\Delta_k \\
&\overset{\eqref{eq:tT:Gamma}}\leq \frac{\rho^2i_{k-1}^+}{\alpha} + \left[\frac{4(k-1)\kappa_p^2}{c}+\pi(x;c)\right] + \frac{4k\kappa_p^2}{c} + k\Delta_k \\ &\le \frac{\rho^2i_{k-1}^+}{\alpha} +  \frac{8k\kappa_p^2}{c}+\pi(x;c) + k\Delta_k,
\end{align*}
where the second last inequality is due to the second inequality in \eqref{eq:lema1:test} with $k=k-1$,
and the third inequality is due to \eqref{eq:tT:Gamma} with $k=k-1$.
Inequality \eqref{eq:sizecy} follows by combining \eqref{eq:FS} and
the last inequality.
\end{proof}


\subsection{Step 3: Proof of Theorem~\ref{thm:static.complexity}}\label{subsec:static.complexity.proof}

In this subsection, we marshal all of the results of the previous subsections to finally prove \textproc{S-ADMM}'s main iteration-complexity result (Theorem \ref{thm:static.complexity}).

We first show that the assumptions \eqref{ini:cond:SA} and \eqref{ini:cond:2:SA} implies that
\begin{equation}\label{eq:chi:Gamma}
\chi(\gamma)\le \bar\chi, \quad \pi(x;c)\le \bar\pi,
\end{equation}
where $\chi(\gamma)$ and $(\bar \chi, \bar\pi)$ are as in \eqref{eq:def.chi.gamma:Ine} and \eqref{eq:def.Gamma.D3}, respectively. Indeed, the lower bound \eqref{ini:cond:2:SA} on $\gamma_t$ 
implies that
$\gamma^{-1} \leq \max \{2 m, {\bar\gamma}^{-1}\}
\le 2 m+ {\bar\gamma}^{-1}$.
This inequality,
the second inequality in \eqref{ini:cond:2:SA}, and the definition of $\chi(\gamma)$  in \eqref{eq:def.chi.gamma:Ine}, then imply that
$\chi(\gamma) \le \bar \chi$. The second inequality in  \eqref{eq:chi:Gamma} follows immediately from the first and third inequality in \eqref{ini:cond:SA} combined with \eqref{eq:def.Gamma.D3} and \eqref{eq:Gamma:x:c}.


(a)  By Proposition~\ref{lem:number.of.cycles}, \textproc{S-ADMM} performs a finite number $K$ of epochs that is bounded by $\bar K$
as in \eqref{def:bar:K:Ine}.
Since $|{\cal I}_k|$ is the number of iterations performed during the $k$-epoch, it suffices to show that
$\sum_{k=1}^{K} |{\cal I}_k| \le \Lambda(c,\rho)$ where $\Lambda(c,\rho)$ is as in \eqref{eq:def.T.complexity}.
Using the bound in \eqref{eq:sizecy}, second inequality in \eqref{eq:chi:Gamma}, and the second inequality in \eqref{eq:sum:Delta:l}, we have
\begin{align*} 
&\sum_{k=1}^{K}  
|{\cal I}_k|  \overset{\eqref{eq:sizecy}}  \le \sum_{k=1}^{ K}\left[\frac{8k\alpha\kappa_p^2}{\rho^2c} + \frac{\alpha\pi(x;c)}{\rho^2} + \frac{\alpha k \Delta_k}{\rho^2}+ 1+\frac{(\chi (\gamma) + (1+\sigma_2) c B \|A\|_\dagger^2)\pi(x;c)}{C^2}\right]\nonumber\\
&\overset{\eqref{eq:sum:Delta:l}}\leq  \frac{K(K+1)}{2}\cdot   \frac{8\alpha  \kappa_p^2}{c\rho^2}+K\left[ 1+\left(\frac{2\alpha}{\rho^2}+\frac{(\chi (\gamma) + (1+\sigma_2) c B \|A\|_\dagger^2)}{C^2}\right)\pi(x;c) \right]
\nonumber\\
&\overset{\eqref{eq:chi:Gamma}}\le \frac{K(K+1)}{2}\cdot   \frac{8\alpha  \kappa_p^2}{c\rho^2}+K\left[ 1+\left(\frac{2\alpha}{\rho^2}+\frac{(\chi (\gamma) + (1+\sigma_2) c B \|A\|_\dagger^2)}{C^2}\right)\bar \Gamma \right].\nonumber
\end{align*}
After some algebraic manipulations, we can easily see that the previous inequality, the fact that  $K\le \bar K\leq [\bar\chi+ (1+\sigma_2) c B \|A\|_\dagger^2 ]/\alpha+1$ (see Proposition~\ref{lem:number.of.cycles}), and the first inequality in \eqref{eq:chi:Gamma}, imply that
\[
\sum_{k=1}^{K}  
|{\cal I}_k| \leq \Lambda_0\frac{c}{\rho^2} +\Lambda_1+\Lambda_2c+ \Lambda_3c^2+ \Lambda_4\frac{1}{\rho^2}=\Lambda(c,\rho),
\]
where $\Lambda_0,$ $\Lambda_1,$ $\Lambda_2,$ $\Lambda_3,$ and $\Lambda_4$  are as in  \eqref{eq:def.constantsT}.

(b) Since $K$ is the last epoch generated by \textproc{S-ADMM} and the inclusion in \eqref{lemma:residual:vi:Ine} holds for every $i\in {\cal I}_K$, we conclude that $(y^{i_K^+}, q^{i_K^+}, v^{i_K^+}, \delta_{i_K^+})=(x^+,p^+,v^+,\varepsilon^+)$ satisfies \eqref{lemma:residual:vi:Ine}, and hence that \eqref{residual:theorem:1} holds. 
The two first inequalities in \eqref{feasi:theorem:1} follows from Lemma~\ref{lem:Ikfinite}(a), due to the fact that $(y^{i_K^+}, q^{i_K^+})=(\tilde y^K, \tilde q^K)$. 
Finally, the last inequality in \eqref{feasi:theorem:1} follows from the fact that \textproc{S-ADMM} terminates on  line~\ref{cond:vi:stop} with the condition $\|v^+\|^2+\varepsilon^+ = \|v^{i_K^+}\|^2+\delta_{i_K^+}\le \rho^2$ satisfied.
We now prove the inequalities in  \eqref{bounds:gamma:initial}. First, observe that $\gamma^+=\lambda^{i_K^+}$ (see lines \ref{stat:test.i.qi.ti.updates} and \ref{update:stat:solu} of \textproc{S-ADMM}). 
Second, using \eqref{ini:cond:2:SA} and \eqref{test:q:adativeness:Ine}, we have
\[
\bar \gamma_t\overset{\eqref{ini:cond:2:SA}}\ge\gamma_t\overset{\eqref{test:q:adativeness:Ine}}\ge \lambda^{i_K^+}_t\overset{\eqref{test:q:adativeness:Ine}}\ge \min \left\{\frac{1}{2m_t},\gamma_t\right\}\overset{\eqref{ini:cond:2:SA}}\ge \min \left\{\frac{1}{2m_t},\bar \gamma_t\right\},
\]
for every $t\in\{1,\ldots , B\}$. Combining these two observations we conclude that \eqref{bounds:gamma:initial} holds.

(c) Using the assumption that $
   c\geq 2 \kappa_p/\eta$,  Lemma~\ref{lem:Ikfinite}(a)  guarantees that \textproc{S-ADMM} output $y^{i_K^+}=x^+$ satisfying
\[
\|Ax^+-b\|\leq \frac{2\kappa_p}{c}\le \eta.
\]
Hence, the conclusion that $(x^+,p^+,v^+, \varepsilon^+)=(\tilde y^K, \tilde q^K,\tilde v^K,\tilde\varepsilon_K)$ satisfies \eqref{eq:stationarysol} follows from the previous inequality, the inclusion in \eqref{residual:theorem:1}, and the last inequality in \eqref{feasi:theorem:1}.

\section{Numerical Experiments}\label{admm:sec:numerical}

This section showcases the numerical performance of \textproc{A-ADMM} on two linearly and box constrained, non-convex, quadratic programming problems. Subsection \ref{sub:numerics.Problem1} summarizes the performance of \textproc{A-ADMM} on a distributed variant of our experimental problem, while Subsection \ref{sub:numerics.Problem2} focuses on a non-distributable variant. The distributed variant employs a small number of high-dimensional blocks while the non-distributable variant conversely has a large number of uni-dimensional blocks. These two proof-of-concept experiments indicate that \textproc{A-ADMM} may not only substantially outperform the relevant benchmarking methods in practice, but also be relatively robust to the relationship between block counts and sizes.

All experiments were implemented and executed in  MATLAB 2021b and run on a macOS machine with a 1.7 GHz Quad-Core Intel processor, and 8 GB of memory.

\subsection{Distributed Quadratic Programming Problem}\label{sub:numerics.Problem1}

This subsection studies the performance of \textproc{A-ADMM} for finding stationary points of a  box-constrained, nonconvex block distributed quadratic programming problem with $B$ blocks (DQP).  

The $B$-block DQP is formulated as
\begin{align}\label{eq:num.problem1}
\min_{(x_{1},\ldots,x_{B})\in\mathbb{R}^{Bn}}\  & -\sum_{i=1}^{B-1}\left[\frac{\alpha_{i}}{2}\|x_{i}\|^{2}+\left\langle x_{i},\beta_{i}\right\rangle \right]\nonumber\\
\text{s.t.}\  & \|x\|_{\infty}\leq \omega\\
& x_i-x_B=0\quad \text{ for }i=1,\ldots,B-1
\end{align}
where $\omega > 0$, $n\in\mathbb{N}$, $\{\alpha_i\}_{i=1}^{B-1}\subseteq [0,1]$, and $\{\beta_i\}_{i=1}^{B-1}\subseteq [0,1]^n$. It is not difficult to see that DQP fits the template of \eqref{initial.problem}. The smooth component is taken to be
    \[
f(x)= -\sum_{i=1}^{B-1}\left[\frac{\alpha_{i}}{2}\|x_{i}\|^{2}+\left\langle x_{i},\beta_{i}\right\rangle \right].
\]
The non-smooth function $\Psi_i$ is set to the indicator of the set $\{x\in \mathbb{R}^n~:~ \|x_i\|_\infty\leq \omega\}$ for $1\leq i\leq B$. For $1\leq i\leq B-1$, we take $A_i\in\mathbb{R}^{n\times Bn}$ to be the operator which includes $A_i\in\mathbb{R}^n$ into the $i$-th block of  $\mathbb{R}^{Bn}$, i.e. 
    \[
    A_i=\begin{bmatrix} 0_{(i-1)n\times n}\\ I_{n\times n}\\ 0_{(B-i)n\times n}\end{bmatrix}
    \]
where $0_{j\times k}$ denotes a $j\times k$ zero matrix. The matrix $A_B\in\mathbb{R}^{n\times Bn}$ is defined by the action $A_Bx=(-x,\ldots,-x)^\top$.


We shall now outline how we conducted our DQP experiments. The number of blocks, $B$, for each experiment was set to $3$, while for the block-size, $n$, the dimensions $n=10,20,100,500$ $(5000) ???$ were considered. For each setting of $n$, we ran experiments where $\omega=10^1,10^3,10^5,10^7,10^9$. The values of $\{\alpha_i\}_{i=1}^{B-1}\subseteq [0,1]$, and $\{\beta_i\}_{i=1}^{B-1}\subseteq [0,1]^n$ were sampled uniformly at random. To generate $b$, we sampled $x_b\in [-\omega,\omega]^{Bn}$ uniformly at random, then set $b=Ax_b$. The initial iterate $x_0$ was also selected uniformly at random from $[-\omega,\omega]^{Bn}$. 

For this problem,  \textproc{A-ADMM} was applied with $c_0=1$, $C=1$, $\alpha=10^{-2}$, $p^0=\mathbf{0}$, and each block's initial stepsize set to $10$, i.e. $\gamma^0_i=10$ for $1\leq i\leq B$. To provide an adequate benchmark for \textproc{A-ADMM}, we compared its performance against two instances of the method from \cite{KongMonteiro2024} and three instances of the method from \cite{sun2021dual}. The method of \cite{KongMonteiro2024} was deployed with two different choices of $(\theta,\chi)$: $(0,1)$ and $(1/2,1/18)$. We call these two instances DP1 and DP2, respectively. Both DP1 and DP2 set $(\lambda, c_1)=(1/2, 1)$. The method of \cite{sun2021dual} was deployed with three different settings of the penalty parameter $\rho$: $0.1$, $1.0$, and $10.0$. We call the resultant instances SD1, SD2, and SD3, respectively. Moreover, all three instances make the parameter selections $(\omega,\theta,\tau)=(4,2,1)$ and $(M_h,K_k,J_h,L_h)=(4\gamma,1,1,0)$ in accordance with \cite[Section 5.1]{sun2021dual}. We reiterate that \cite{KongMonteiro2024} provides no convergence guarantees for the pragmatic choice of $(\theta,\chi)=(0,1)$. All executed algorithms were run for a maximum of $500,000$ iterations. Any algorithm that met this limit took at least $10$ milliseconds to complete.


\input{data/ADMM/P1-Table4}

Table \ref{tab:numeric.table1}, the record of the performance of all algorithms on this experimental problem, lays bare the superior performance of \textproc{A-ADMM}. In this table, we label \textproc{A-ADMM} as AD for the sake of concision. In terms of iterations, \textproc{A-ADMM} outperforms all other algorithms for all settings of $B$ and $m$. Along the dimension of time, \textproc{A-ADMM} is faster than all algorithms, for all settings of $n$ and $\omega$, except DP1 when $n=100$ and $\omega=10$.


\subsection{Nonconvex QP with Box Constraints}\label{sub:numerics.Problem2}

In this subsection, we evaluate the performance of \textproc{A-ADMM} for solving a general nonconvex quadratic problem with box constraints (QP-BC). The QP-BC problem is formulated as
\begin{equation}\label{eq:num.problem2}
\min_{\|x\|_\infty\leq \omega } \left\{f(x) := \frac{1}{2}\inner{x}{Px} + \inner{r}{x}: Ax=b \right\}.    
\end{equation}
where $P\in \mathbb{R}^{B\times B}$ is negative definite, $A\in \mathbb{R}^{m\times B}$, $r,b\in \mathbb{R}^m \times\mathbb{R}^m$ and $\omega\in \mathbb{R}_{++}$. As for the previous problem, it is not difficult to check that QP-BC fits within the template of \eqref{initial.problem}. For this problem, we take our blocks to be single coordinates. Consequently, each column of $A$ gives rise to a $A_i$ matrix. The non-smooth components of the objective are again picked to be the indicator functions of the sets $\{x_i\in \mathbb{R}: |x_i|\le \omega\}$ for $i\in \{1,\ldots, B\}$.

We now describe how we orchestrated our QP-BC experiments. In all instances, $\omega=1$. To generate $\tilde r\in \mathbb{R}^m$, $\tilde P\in\mathbb{R}^{B\times B}$ and $\tilde A\in\mathbb{R}^{m\times B}$, we started by generating a diagonal matrix $D\in\mathbb{R}^{B\times B}$ whose entries are selected uniformly at random in $[1,1000]$. Next, we generated $\tilde r\in [-1,1]^m$, $\tilde P\in[-1,1]^{B\times B}$ negative definite, and $\tilde A\in[-1,1]^{m\times B}$ uniformly at random. Finally, we set $P=D\tilde P D$, $A=\tilde A D$, and $r=D\tilde r$. The vector $b\in\mathbb{R}^m$ was set as $b=Ax_b,$ where $x_b$ is a uniformly at random selected vector in $[-1,1]^B$. The initial starting point $x^0$ was chosen in this same fashion. 

For this problem,  three instances of \textproc{A-ADMM}, referred to as AD1, AD2, and AD3, were applied with $C=1$, $\alpha=10^{-2}$, $p^0=\mathbf{0}$, and each block's initial stepsize set to $10$, i.e. $\gamma^0_i=1000$ for $1\leq i\leq B$. The three methods differ only in their choice of initial penalty parameter $c_0$: $c_0=10$ for AD1, $c_0=1$ for AD2, and $c_0=.1$ for AD3.
The benchmarking algorithms for this experiment were three instances of the method from \cite{KongMonteiro2024}, which we refer to as DP1, DP2 and DP3. Like the three instances of \textproc{A-ADMM}, these instances differ only in their choice of $c_0$: $c_0=10$ in DP1, $c_0=1$ in DP2 and $c_0=0.1$ in DP3. Each of these three methods were applied with $(\theta,\chi)=(0,1)$. Yet again, we remind the reader that \cite{KongMonteiro2024} provides no convergence guarantees for this choice of $(\theta,\chi)$.  To ensure timely execution of all algorithms, each algorithm terminated upon meeting a 500,000 iteration limit or the discovery of an approximate stationary triple $(x^+, p^+, v^+)$ satisfying the relative error criterion
\[
v^+ \in \nabla f(x^+) + \partial \Psi(x^+) + A^*p^+, \quad \frac{\|v^+\|}{1+\|\nabla f(x^0)\|}\leq \rho , \quad \frac{\|Ax^+-b\|}{1+\|Ax^0-b\|}\leq \eta.
\]
for $\rho=\eta=10^{-5}$.

\input{data/ADMM/P2-Table4}

The results for this experiment, shown in Table \ref{tab:numeric.results.table2}, echo those for its predecessor by again displaying the computational superiority of \textproc{A-ADMM}. Measured by iteration count, \textproc{A-ADMM} performed better in $87\%$ of the problem instances. In terms of time, \textproc{A-ADMM} performed better in $100\%$ of the instances. It is worth mentioning that \textproc{A-ADMM} converged for all instances, while the same cannot be said for the DP1, DP2, and DP3 benchmark methods. DP1 converged for $96\%$ instances, DP2 converged for $54\%$ instances, and DP3 converged only for $27\%$ instances. For $m=1,2,5$, our method was at least $10$ times faster in terms of iteration count and time than any DP variant. Notably, we attempted to apply multiple versions of the method from \cite{KongMonteiro2024} with choices of $(\theta,\chi)$ that theoretically should ensure convergence. None of the methods managed to find the desired point within the iteration limit, so we omitted their results from the table.


\section{Chapter's Conclusion}\label{sec:concluding}

We now discuss some further related research directions. First, the ability of \textproc{A-ADMM} to allow for the inexact solution of its block subproblem opens up many possible avenues for application. A systematic numerical study of its performance when applied to problems requiring inexact computation would be intriguing. Second, it would be interesting to develop a \textproc{P-ADMM} that performs Lagrange multiplier updates
with 
$(\theta,\chi)=(0,1)$ at every iteration, rather than
just at the last iteration of each epoch. This \textproc{P-ADMM} would then be an instance of the class of ADMMs outlined in the Introduction with
$|\mathcal{I}_k|=1$. The \textproc{P-ADMM} of \cite{KongMonteiro2024} satisfies this last property but chooses $(\theta,\chi)$ in a very conservative way, namely, satisfying
\eqref{eq:assumptio:B}.
Third, it would be interesting to
consider inexact \textproc{P-ADMM}s that solve the prox subproblems based on the more relaxed error criterion \eqref{ISO:Cond:2} with $\vartheta>0$ since this generalization would possibly 
allow us to develop an inexact
\textproc{P-ADMM} in the setting of \eqref{initial.problem} with $f$ being non-smooth.
Finally, we have assumed in this paper that $\mathrm{dom } \Psi$ is bounded (see assumption (A1)). It would be interesting to extend its analysis  to  the case where ${\cal H}$
is unbounded.

%\appendix



\section{Technical Results for Proof of Lagrange Multipliers}\label{technical lagrange multiplier}

This section provides some technical results to show that under certain conditions the Lagrangian multiplier is bound. 


The next two results,  used in Lemma~\ref{lem:qbounds-2},  can be found in  \cite[Lemma B.3]{goncalves2017convergence} and 
\cite[Lemma 3.10]{kong2023iteration}, respectively. 

\begin{lemma}\label{lem:linalg} 
Let $A:\mathbb{R}^n \to \mathbb{R}^l$ be a  nonzero linear operator. Then,
\[
\nu^+_A\|u\|\leq \|A^*u\|,   \quad \forall u \in A(\mathbb{R}^n).
\]
\end{lemma}


\begin{lemma}\label{lem:bound_xiN}
Let $\Psi$ be a function as in (A5).
Then, for every $\delta \ge 0$, $z\in {\mathcal H}$,   and $\xi \in \partial_{\delta} \Psi(z)$, we have
\begin{equation*}\label{bound xi}
\|\xi\|{\rm dist}(u,\partial {\mathcal H}) \le \left[{\rm dist}(u,\partial {\mathcal H})+\|z-u\|\right]M_h + \inner{\xi}{z-u}+\delta \quad \forall u \in {\mathcal H}
\end{equation*}
where $\partial {\cal H}$ denotes the boundary of ${\cal H}$.
\end{lemma}

\begin{lemma}\label{lem:qbounds-2}
Assume that $\Psi$ is a function as in assumption (A5) and  $A:\mathbb{R}^n \to \mathbb{R}^l$ is a nonzero linear operator satisfying assumption (A2).  
If $(q^-,\chi) \in \mathbb{R}^l \times (0,\infty)$ and $(z,q,r) \in  \mathrm{dom } \Psi \times A(\mathbb{R}^n) \times \mathbb{R}^n$ satisfy
\begin{equation}\label{eq:cond:Lem:A1}
r \in \partial_\delta \Psi(z)+A^{*}q\quad\text{and}\quad 
q=q^-+\chi(Az-b),
\end{equation}
then we have 
\begin{equation}\label{q bound-2}
 \|q\|\leq \max\left\{\|q^-\|,\frac{2D_h(M_h+\|r\|)+\delta}{\bar d \nu^{+}_A} \right\},
\end{equation}
where $M_h,$ $\bar d>0$, and $D_h$ are as in (A5), (A6), and \eqref{def:damH}, respectively, and $\nu^+_A$ denotes  the smallest positive singular value of $A.$
\end{lemma}	
\begin{proof}
 We first claim that
\begin{equation}\label{ineq:aux9001-2}
 \bar{d}\nu_A^{+}\|q\|
\leq  2 D_h\left(M_h + \|r\| \right)  - \inner{q}{Az-b}+\delta
\end{equation}
holds.
The assumption on $(z,q,r)$ implies that $r-A^{*}q \in \partial_{\delta} \Psi(z)$. Hence, using the Cauchy-Schwarz inequality, the definitions of $\bar d$ and $\bar z$ in (A6), and
Lemma~\ref{lem:bound_xiN} with $\xi=r-A^{*}q$, and  $u=\bar z$, we have:
 \begin{align}\label{first inequality p-2}
   \bar d\|r-A^{*}q\|-\left[\bar d+\|z-\bar z\|\right]M_h &\overset{\eqref{bound xi}}{\leq}  \inner{r-A^{*}q}{z-\bar z}\leq \|r\| \|z-\bar z\| - \inner{q}{Az-b}+\delta.
 \end{align}
 Now, using the above inequality,
 the triangle inequality, the definition of $D_h$ in \eqref{def:damH}, and the facts that $\bar d \leq D_h$ and $\|z-\bar z\|\leq D_h$, we conclude that:
 \begin{align}\label{second inequality p-2}
 \bar d \|A^*q\| + \inner{q}{Az-b}
 &\overset{\eqref{first inequality p-2}}{\leq} \left[\bar d+\|z-\bar z\|\right]M_h + \|r\| \left(D_h + \bar d\right) \leq 2 D_h\left(M_h + \|r\| \right)+\delta.
 \end{align}
 Noting the assumption that
$q \in A(\mathbb{R}^n)$,
inequality
 \eqref{ineq:aux9001-2} now follows
from the above inequality
and
Lemma~\ref{lem:linalg}.

We now prove \eqref{q bound-2}. Relation \eqref{eq:cond:Lem:A1}  implies that $\inner{q}{Az-b}=\|q\|^2/\chi-\inner{q^-}{q}/\chi$, and hence that
\begin{equation}\label{q relation-2}
    \bar d \nu^{+}_A\|q\|+\frac{\|q\|^2}{\chi}\leq 2D_h(M_h+\|r\|)+\frac{\inner{q^-}{q}}{\chi}\leq 2D_h(M_h+\|r\|)+\frac{\|q\| }{\chi}\|q^-\|+\delta,
\end{equation}
where the last inequality is due to the Cauchy-Schwarz inequality.
Now, letting
$K$ denote the right hand side of \eqref{q bound-2} and using \eqref{q relation-2},
we conclude that
\begin{equation}\label{prelim q bound-2}
\left(\bar d \nu^+_A+\frac{\|q\|}{\chi}    \right)\|q\|\overset{\eqref{q relation-2}}{\leq} \left(\frac{2D_h(M_h+\|r\|)+\delta}{K}+\frac{\|q\| }{\chi}\right)K\leq \left(\bar d \nu^+_A+\frac{\|q\|}{\chi}    \right) K,
\end{equation}
and hence that \eqref{q bound-2} holds.
\end{proof}

We conclude this section with a technical result of convexity which is used in the proof of Lemma \ref{pro:lem:kong:new:Ine}.
Its proof can be found in \cite[Lemma A1]{melo2023proximal}.

\begin{lemma}\label{conv:result}
    Assume that $\xi>0$, $\psi$ is a proper, closed, and convex function, and $Q$ is a $n\times n$ positive definite matrix such that $\psi-(\xi/2)\|\cdot\|_Q^2$ is convex and let $(y,v,\hat\eta)\in \mathbb{R}^n\times\mathbb{R}^n\times\mathbb{R}_+$ be such that $y\in \partial_{\hat\eta}\psi(y).$ Then, for any $\tau>0$,
    \[
    \psi(u)\ge \psi(y)+\langle v, u-y\rangle-(1+\tau^{-1})\hat\eta+\frac{(1+\tau^{-1})\xi}{2}\|u-y\|_Q^2 \quad\forall u\in \mathbb{R}^n.
    \]
\end{lemma}



\section{Proof of Proposition \ref{main:appen:2}}
\label{append:cgm}

This section contains the proof of Proposition \ref{main:appen:2}.

Before giving the proof of Proposition \ref{main:appen:2}, we present a preliminary result related to S-CGM.

\begin{lemma}
\label{lm:cgm-0}
For every $j \ge 1$,
the vector $\tilde v^j \in \mathbb{R}^{n}$ defined in \eqref{def:resi:app}
satisfies
\begin{equation}\label{inclu: Apen}
\tilde v^j \in \nabla \Gamma_s(\tilde z^j) + \partial \Gamma_n(\tilde z^j) \quad\text{and}\quad 8M[\Gamma(\tilde z^{j-1})-\Gamma(\tilde z^j)]\ge \|\tilde v^j\|^2.
\end{equation}
\end{lemma}

\proof
The optimality condition for \eqref{eq:CGM-nc2}
implies that 
\[
0 \in \nabla \Gamma_s(\tilde z^{j-1})+\partial \Gamma_n(\tilde z^j)+M(\tilde z^j-\tilde z^{j-1}). 
\]
The inclusion \eqref{inclu: Apen}  now follows from the above inclusion and the definition of $\tilde v^j$ in \eqref{def:resi:app}.
We now prove the inequality in \eqref{inclu: Apen}.
Using the definition of $\tilde v^j$ in \eqref{def:resi:app}, the triangle inequality, and assumption (B2), we have
\begin{align}\label{eq:tv:displ}
\norm{\tilde v^j} &\le M \norm{\tilde z^{j-1}-\tilde z^j} + \norm{\nabla \Gamma_s(\tilde z^j) - \nabla\Gamma_s (\tilde z^{j-1})}
\le 2M\|\tilde z^{j-1}-\tilde z^j\|.
\end{align}

On the other hand, using the fact that the objective function in \eqref{eq:CGM-nc2} is $M$-strongly convex and that $\tilde z^j$ is its optimal solution, we have
\begin{align*}
       \ell_{\Gamma_s}(w, \tilde z^{j-1})& +\Gamma_n(w)  + \frac{M}{2} \|w-\tilde z^{j-1}\|^2 -
     \frac{M}{2} \|w-\tilde z^{j}\|^2 
     \ge \ell_{\Gamma_s}(\tilde z^j, \tilde z^{j-1}) + \Gamma_n(\tilde z^j)+ \frac{M}{2} \|\tilde z^j-\tilde z^{j-1}\|^2, 
    \end{align*}
for every $w\in \mathbb{R}^n$.    Thus, using the previous inequality with $w=\tilde z^{j-1}$ and the facts that,
for every $\tilde x \in \mathbb{R}^n$, we have
$\ell_{\Gamma_s}(\tilde x;\tilde x)=\Gamma_s(\tilde x)$
and $\ell_{\Gamma_s}(\tilde z^j,\tilde z^{j-1}) \ge \Gamma_s(\tilde z^j) - (M/2) \|\tilde z^j-\tilde z^{j-1}\|^2$, which is a consequence of assumption (B2), we obtain that
\begin{equation}\label{eq:cgm-2}
\Gamma(\tilde z^{j-1}) - \Gamma(\tilde z^{j})\ge
     \frac{M}{2} \|\tilde z^{j}-\tilde z^{j-1}\|^2.
\end{equation}
The conclusion now follows by combining \eqref{eq:tv:displ} and \eqref{eq:cgm-2}. 
\endproof

\vgap

\noindent
{\bf Proof of Proposition \ref{main:appen:2}}  
 
Assume for the sake of contradiction that 
\begin{equation}\label{conta:assum:app:2}
\|\tilde v^j\|^2> \sigma [\Gamma(\tilde z^0)-\Gamma(\tilde z^j)] + \vartheta^2\quad \forall  j\in \{1,\ldots,  \bar K\}.
\end{equation}
Inequality \eqref{inclu: Apen} and the previous inequality, both with $j=1$, imply that

\begin{equation}\label{diff:psi:0:1}
\Gamma(\tilde z^{0})-\Gamma(\tilde z^1) \overset{\eqref{inclu: Apen}}\ge  \frac{ \|\tilde v^1\|^2 }{8M} \overset{\eqref{conta:assum:app:2}}> \frac{\vartheta^2+\|\tilde v^1\|^2}{16M}.
\end{equation}
Combining inequalities  \eqref{inclu: Apen} and \eqref{conta:assum:app:2}, we have that for $j\in \{1,\ldots,  \bar K-1\}$,
\begin{equation}\label{eq:main:appen:2:proof}
8M [ \Gamma(\tilde z^j) - \Gamma(\tilde z^{j+1})] \overset{\eqref{inclu: Apen}}\ge \|\tilde v^{j+1}\|^2 \overset{\eqref{conta:assum:app:2}}>  \sigma [ \Gamma(\tilde z^0) - \Gamma(\tilde z^{j+1})].
\end{equation}

Hence, for every $j\in \{1,\ldots,  \bar K-1\}$, we have
\begin{align*}
8M [ \Gamma(\tilde z^0) - \Gamma(\tilde z^{j+1})] &= 8M [ \Gamma(\tilde z^0) - \Gamma(\tilde z^{j})] + 
8M[ \Gamma(\tilde z^{j}) - \Gamma(\tilde z^{j+1})]\\ 
& \overset{\eqref{eq:main:appen:2:proof}}{>} 8M [ \Gamma(\tilde z^0) - \Gamma(\tilde z^{j})] + 
\sigma [ \Gamma(\tilde z^0) - \psi(z^{j+1})]\\
& \overset{\eqref{eq:cgm-2}}{\ge} 8M [ \Gamma(\tilde z^0) - \Gamma(\tilde z^{j})] + 
\sigma [\Gamma(\tilde z^0) - \Gamma(\tilde z^{j})] =   \left (8M + \sigma \right)  [ \Gamma(\tilde z^0) - \psi(z^{j})].
\end{align*}
As a consequence, the previous inequality and \eqref{diff:psi:0:1} imply that 
\begin{align*}
\Gamma(\tilde z^0)- \psi^{*} \geq \Gamma(\tilde z^0) - \psi(z^{\bar K}) &> \left(1+\frac{\sigma}{8M} \right)^{\bar K-1}(\Gamma(\tilde z^0) - \Gamma(\tilde z^1))\\
&>\left(1+\frac{\sigma}{8M} \right)^{\bar K-1}\frac{\vartheta^2+ \|\tilde v^1\|^2}{16M},
\end{align*}
and hence that
\[
\ln\left(\frac{16M[\Gamma(\tilde z^0)-\Gamma^*]}{\vartheta^2+ \|\tilde v^1\|^2}\right)>(\bar K-1)\ln \left(1+\frac{\sigma}{8M} \right)>(\bar K-1)\frac{\sigma/(8M)}{1+\sigma/(8M)}=\frac{\sigma(\bar K-1)}{8M+\sigma},
\]
where in the last inequality above, we used the fact that $\ln(1+x)>x/(1+x)$ for every $x \in (-1,\infty)$. Thus,
\[
\bar K - 1<\frac{8M+\sigma}{\sigma} \ln\left(\frac{16M[\Gamma(\tilde z^0)-\Gamma^*]}{\vartheta^2+ \|\tilde v^1\|^2}\right).
\]
Since the last inequality contradicts with the definition of $\bar K$ in \eqref{eq:K:appe:2}, the conclusion of the proposition follows. 


%\bibliography{relax_admm_ref.bib}

%\bibliographystyle{plain}
%\bibliography{relax_admm_ref}



==> data/TR/tr.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Spring 2021.  
%
%
%  Author: Thesis Office
%  
%  Last Updated: 1/13/2021
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           SECTION I
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\pagestyle{plain} % No headers, just page numbers
\pagenumbering{arabic} % Arabic numerals
\setcounter{page}{1}


\chapter{\uppercase {AN Inexact Weighted Proximal Trust-Region Method}}



% Include your abstract here.
\begin{abstract}
In [R.~J.~Baraldi and D.~P.~Kouri, {\em Math.~Program.}, 201:1 (2023), pp.~559-598], the authors introduced a trust-region method for minimizing the sum of a smooth nonconvex and a nonsmooth convex function, the latter of which has {an} analytical proximity operator. 
While many functions satisfy this criterion, e.g., the $\ell^1$-norm defined on $\ell^2$, many others are precluded by either the topology or the nature of the nonsmooth term.
Using the $\delta$-Fr\'{e}chet subdifferential, we extend the definition of the inexact proximity operator and enable its use within the aforementioned trust-region algorithm. Moreover, we augment %generalize
the analysis for the standard trust-region convergence theory to handle proximity operator inexactness %. To conclude, we restrict our attention to 
with weighted inner products.  We first introduce an algorithm to generate a point in the inexact proximity operator and then apply the algorithm within the trust-region method to solve an optimal control problem constrained by Burgers' equation.
\end{abstract}

\section{Introduction}
Our goal is the efficient numerical solution to the nonsmooth, nonconvex optimization problem
\begin{equation}\label{eq:optprob}
  \min_{x\in X}\; \left\{f(x)+\phi(x)\right\},
\end{equation}
where $X$ is a real Hilbert space, $f:X\to\R$ is a smooth nonconvex function and $\phi:X\to(-\infty,+\infty]$ is a proper, closed and convex function. 
The method developed in \cite{Baraldi2023} solves \eqref{eq:optprob} via a trust-region method that permits inexact evaluations of the smooth objective function $f$ and its gradient.
The convergence analysis for the trust-region method is contingent on the proximity operator of $\phi$ being exact, i.e. analytically
computable. 
In this paper, we extend the inexact proximal trust-region algorithm in \cite{Baraldi2023} to leverage certain inexact evaluations of the proximity operator of $\phi$.
The proximity operator of $\phi$ at $x$ with stepsize $r$ is defined as the unique solution to the minimization problem
\begin{equation}\label{eq:exact.prox}
  \Proxrphi(x) :=
  \Argmin_{y\in X}\left\{ \frac{1}{2r}\|y-x\|^2 + \phi(y)\right\}
\end{equation}
and is a powerful tool to deal with composite nonsmooth optimization problems like \eqref{eq:optprob}.
Algorithms that leverage the proximity operator, like ISTA and FISTA \cite{Beck17}, are typically first-order and only apply to convex optimization problems.
Like \cite{Baraldi2023}, these methods require that the proximity operator be computed exactly---a requirement that is often computationally expensive or even impossible to satisfy. For instance, if $X$ is finite dimensional with dot product defined by a diagonal matrix $D$ and $\phi$ is the $\ell^1$ norm, then the proximity operator has an analytical expression. 
In contrast, if the dot product is defined by a non-diagonal symmetric positive definite (spd) matrix $M$, then evaluating the proximity operator requires a specialized iterative method to obtain an approximate solution.
Although preliminary studies on optimization with inexact proximity operators {exist} \cite{Devolder14,MaiaInexactCyclic,Hua12,Kim-chuan12,salzo2012inexact,Richtarik14},
these works only apply to convex problems and often exhibit slow convergence rates.  Using these methods as motivation, we develop a proximal Newton method---tailored to the case of diagonal and non-diagonal dot products---that can handle inexact proximity operators.  We define our inexact proximity operator as
\begin{align}\label{intro:inexact.prox}
    \Proxrphi(x,\delta) :=  \Big\{p\in X\,\Big\vert\, &\frac{1}{2r}\|p-x\|^2+\phi(p) \nonumber \\
    &\le\frac{1}{2r}\|z-x\|^2+\phi(z)+\delta\|z-p\|\;\;\forall\,z\in X\Big\}
\end{align}
The inclusion of the term $\delta\|z-u\|\ge 0$ on the right-hand side of \eqref{intro:inexact.prox} allows the proximity operator to be computed inexactly.
%In Section~\ref{sec:inexact.subgradient.proximal}, we detail this new proximity operator and relate it to the $\delta$-Fréchet subdifferential \cite{mordukhovich2006variational}.

\if(0)
Our goal in this paper is twofold:
\begin{itemize}
    \item[1.] Develop an algorithm to obtain one solution to the inexact proximal defined in \ref{intro:inexact.prox}, for a some classes of matrices $M$.
    \item[2.] Apply our novel inexact proximal map to \cite{Baraldi2023} to solve \textit{{Burgers'}} equation \textcolor{red}{[reference]}.
\end{itemize}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Drew´s comment
% By relaxing this condition,

% 1. theory of inexact prox map for the trust region method.

% 2. what is a prox operator.

% 3. How is it used inside of the algorithm (cauchy point -> decrease). To satisfy these conditions, we need an specific tolerance....

% 4. depending on the innner product, the proximity can be very hard (or easy) to calculate...example: diagonal is easy(separable)..on the other other, for general SPD you cannot separate the problem.


The remainder of the article is structured as follows.
In Section~\ref{sec:trust}, we review the inexact trust-region method introduced in \cite{Baraldi2023}, presenting the main components of the algorithm. 
We also include a lemma that enables the use of our inexact proximal map. In Section~\ref{sec:inexact.subgradient.proximal}, we lay out our definition of inexact proximity operator based on the Fr\'{e}chet subdifferential. 
In Section~\ref{sec:inexact.subgradient.proximal}, we present the main technical results of this work, where we establish the relationship between the $\delta$-Fr\'{e}chet subdifferential \cite{mordukhovich2006variational} and the $\delta$-proximal map. We conclude with Section~\ref{sec:M.weighted.prox}, where we present numerical results for the optimal control of Burgers' equation. 

%Section \textcolor{red}{X} gives some concluding remarks that sugget further research directions.

\section{Notation and Problem Assumptions}
\label{sec:notation}
Throughout, $X$ denotes a real Hilbert space with inner product $\inner{x}{y}$ and norm $\|x\|=\inner{x}{x}^{1/2}$.  
To simplify the presentation, we associate the topological dual space $X^*$ with $X$ through Riesz representation.
We assume that $\phi:X\to(-\infty,+\infty]$ is proper, closed and convex with effective domain
\[
  \textup{dom}\,\phi:= \{x\in X\,\vert\, \phi(x)<+\infty\}.
\]
We further assume that $f:X\to\R$ is Fr\'{e}chet differentiable on an open set containing $\textup{dom}\,\phi$ and its derivative is Lipschitz continuous on that set.  We denote the derivative of $f$ at $x\in X$ by $f'(x)\in X^*$ and its gradient (i.e., Riesz representer) by $\nabla f(x)\in X$.  Finally, we assume that the total objective function $F(x):= f(x)+\phi(x)$ is bounded from below.

The main focus of this paper is the use of inexact proximity operators arising from weighted inner products.  To this end, we define $a:X\times X\to\mathbb{R}$ to be a symmetric, coercive and continuous bilinear form, i.e., there exists $0<\alpha_1\le\alpha_2<\infty$ such that
\[
    a(x,y) = a(y,x),\quad \alpha_1\|x\|^2\le a(x,x), \qquad\text{and}\quad a(x,y) \le \alpha_2\|x\|\|y\| 
\qquad\forall\,x,\,y\in X.
\]
We associate $a$ with the invertible (cf.~the Lax-Milgram lemma), self-adjoint, positive and continuous linear operator $A:X\to X$ defined by its action:
\[
  \inner{Ax}{y} = a(x,y)\qquad\forall\,x,\,y\in X.
\]
Recall that $a(\cdot,\cdot)$ defines an inner product on $X$ and its associated norm $\|\cdot\|_a = \sqrt{a(\cdot,\cdot)}$ is equivalent to $\|\cdot\|$.  We denote the (inexact) proximity operator associate with $a$ by $\Proxrphi^a$.

For our numerical results, we will work with $X=\R^n$ endowed with the dot product
\[
  \inner{x}{y}=\inner{x}{y}_M :=  x^\top M y = \sum_{i=1}^n\sum_{j=1}^n m_{i,j}x_i y_j,
\]
where $M\in\R^{n\times n}$ is a non-diagonal spd matrix.  In many common choices of $\phi$, the proximity operator associated with the $M$-weighted dot product lacks an analytical form.  In this case, we replace $\inner{\cdot}{\cdot}$ with the equivalent dot product
\[
  a(x,y) = \inner{x}{y}_D :=  x^\top D y = \sum_{i=1}^n d_i x_i y_i,
\]
where $D=\textup{diag}(d)\in\R^{n\times n}$ is a positive diagonal matrix.  In this setting, the linear operator $A$ is given by
\[
  A = M^{-1}D.
\]
For clarity, we denote $\Rn$ endowed with the $M$-weighted dot product by $X_M$ and analogously for $X_D$.
We further denote the proximity operator defined on $X_M$ by $\Proxrphi^M$ and similarly on $X_D$ by $\Proxrphi^D$.


%\subsection{Notation and Basic Definitions}
%We shall assume throughout this work that

%\begin{itemize}
%    \item [A1.] $X$ is a subset of $\Rn$.
%    \item [A2.] $\phi:X \rightarrow \R$ is proper, closed and convex function with a compact domain $H=\text{dom } (\phi)$, and also a nonsmooth function.
%\end{itemize}



\section{A Proximal Trust{-}Region Method}
\label{sec:trust}

Trust{-}regions are iterative methods for computing approximate solutions to general nonconvex optimization problems \cite{conn2000trust} and are ideal for leveraging inexact computations \cite{Baraldi2023,kouri2018inexact}.
In the recent work \cite{Baraldi2023}, the authors developed a proximal trust-region method for nonsmooth optimization problems with the form \eqref{eq:optprob} that exploits inexact function and gradient evaluations with guaranteed convergence.  At the $k$-th iteration of \cite[Algorithm~1]{Baraldi2023}, we compute a trial iterate $x_k^+$ that approximately solves the trust-region subproblem
\begin{equation}\label{eq:tr-sub}
  \min_{x\in X}\{m_k(x):= f_k(x)+\phi(x)\} \qquad \text{subject to}\qquad \|x-x_k\|\le \Delta_k,
\end{equation}
where $x_k \in \textup{dom}\,\phi$ is the current iterate, $f_k$ is a smooth local model of $f$ around $x_k$, and $\Delta_k > 0$ is the trust-region radius. In particular, we require that the trial iterate $x_k^+$ satisfies the fraction of Cauchy decrease condition: there exist positive constants $\krad$ and $\kfcd$, independent of $k$, such that
\begin{subequations}\label{eq:FCD.condition}
\begin{align}
  \|x_k^+-x_k\| &\le \krad \Delta_k \\
  m_k(x_k)-m_{k}(x_k^+) &\ge \kfcd h_k\min\left\{\frac{h_k}{1+\omega_k},\Delta_k\right\},
\end{align}
\end{subequations}
where $\omega_k$ is a measure of the curvature of $f_k$ given by
\begin{equation*}\label{eq:def.curvature}
  \omega_k:= \sup \{|\omega(f_k,x_k,s)| \,\vert\, 0<\|s\|\le \krad\Delta_k \},
\end{equation*}
$\omega(g,x,s)$ is the curvature of the Fr\'{e}chet differentiable function $g:X\to\R$ at $x\in X$ in the direction $s\in X$, i.e.,
\[
  \omega(g,x,s) :=  \frac{2}{\|s\|^2}[g(x+s)-g(x)-\inner{\nabla g(x)}{s}],
\]
and $h_k$ is our stationarity metric given by
\begin{equation}
    \label{eq:hk_exact}
  h_k := \frac{1}{r_0}\|\Proxrzerophi(x_k-r_0\nabla f(x_k))-x_k\|.
\end{equation}
    
Given a trial iterate $x_k^+$ that satisfies \eqref{eq:FCD.condition}, we decide whether to accept or reject $x_k^+$ using the ratio of computed ($\cred_k$) and predicted ($\pred_k$) reductions,
\begin{align}\label{eq:rho}
  \rho_k:=\frac{\cred_k}{\pred_k}.
\end{align}
The computed reduction $\cred_k$ is an approximation of the actual reduction
\begin{align}
  \ared_k := F(x_{k})-F(x_k^+) 
\end{align}
and the predicted reduction $\pred_k$ is the decrease predicted by the model $m_k$,
\begin{align}
  \pred_k := m_k(x_k)-m_k(x_k^+).
\end{align}
If $\rho_k\ge \eta_1$, we accept $x_k^+$, i.e., $x_{k+1}=x_k^+$. Otherwise, we reject it, setting $x_{k+1}=x_k$. We furthermore use $\rho_k$ to increase or decrease the trust-region radius $\Delta_k$.  Here, $\eta_1\in(0,1)$ is a user-specified parameter.


Algorithm~\ref{alg:cap} states the inexact proximal trust-region method from \cite[Algorithm~1]{Baraldi2023}.
To ensure convergence, Algorithm~\ref{alg:cap} requires the following assumptions on the inexact evaluations $f$ and its gradient. The first assumption ensures that the computed reduction $\cred_k$ is a sufficiently accurate approximation of the actual reduction $\ared_k$.

\begin{assumption}[Inexact Objective]
\label{assump:inexact.object}
    There exists a positive constant $\kobj$, independent of $k$, such that
    \begin{equation}\label{eq:assump.inexact.objective}
        |\ared_k-\cred_k| \leq \kobj\left[ \eta\min\{\pred_k,\theta_k\}\right]^{\zeta}
    \end{equation}
where
\[
\zeta>1,\quad 0<\eta<\min\{\eta_1,(1-\eta_2)\}\quad \text{and}\quad \lim_{k\to+\infty}\theta_k=0
\]
are used provided parameters.
\end{assumption}

{It is noteworthy mentioning that the right-hand side in~\eqref{eq:assump.inexact.objective} is easily computable. Hence, this enables the framework to avoid the computation of the actual reduction.}

Similarly, the following assumption enables approximations of the gradient of $f$ within a prescribed tolerance that depends on the state of the algorithm.

\begin{assumption}[Inexact Gradient]
\label{assump:inexact.gradient}
The model $f_k: X \rightarrow \R$ has Lipschitz continuous derivatives on an open set containing $\dom\, \phi$ and there exists a positive constant $\kgrad$, independent of $k$, such that
\[
\|g_k - \nabla f(x_k)\|\leq \kgrad\min \{h_k,\Delta_k\},
\]
where $g_k := \nabla f_k(x_k)$.
\end{assumption}


\begin{algorithm}
\caption{Nonsmooth Trust-Region Algorithm}\label{alg:cap}
\begin{algorithmic}[1]
\Require $x_1\in \dom \psi$, $\Delta_1>0$, $0<\eta_1<\eta_2<1$, and $0<\gamma_1\leq \gamma_2 \leq \gamma_3$
%\Ensure $y = x^n$
\For{$k=1,2,\ldots$}
    \State \textbf{Model Selection:} Choose $m_k$ that satisfies Assumption~\ref{assump:inexact.gradient} \label{alg:assump.model.inexact}
    \State \textbf{Step Computation:} Compute $x_k^+\in X$ satisfying equation~\eqref{eq:FCD.condition} \label{alg:exact.inexact}
    \State \textbf{Computed Reduction:} Compute $\cred_k$ satisfying Assumption~\ref{assump:inexact.object}
    \State \textbf{Step Acceptance and Radius Update:} Compute $\rho_k$ as in \eqref{eq:rho}

    \If{$\rho_k<\eta_1$}
        \State $x_{k+1}\gets x_k$
        \State $\Delta_{k+1}\in [\gamma_1\Delta_k,\gamma_2\Delta_k]$

    \Else
        \State $x_{k+1}\gets x_k^+$
        \If{$\rho_k\in [\eta_1,\eta_2)$}
            \State $\Delta_{k+1}\in[\gamma_2\Delta_k,\Delta_k]$
        \Else
            \State $\Delta_{k+1}\in[\Delta_k,\gamma_3\Delta_k]$
        \EndIf
    \EndIf

\EndFor
\end{algorithmic}
\end{algorithm}




%Drew´s comment
% their algorithm..

% [introduce the algorithm with exact prox...explain how we should change to accommodate the inexact prox.]

% -inn grad
% -inn $h_k$
% -Cauchy decrease

% Cauchy point: the change (accommodate the inexact prox)...this motivates this work

% We need to ensure the inexact produces sufficient decrease.



A critical component of the convergence theory for Algorithm~\ref{alg:cap} is that the trial iterate satisfies \eqref{eq:FCD.condition}.
In the smooth case (i.e., $\phi\equiv 0$), this condition is satisfied if $x_k^+$ produces at least a fraction of the decrease achieved by the steepest descent step.
In the nonsmooth case, \cite{Baraldi2023} instead defines sufficient decrease using the proximal gradient step.  
In particular, \cite[Lemma~7]{Baraldi2023} illustrates the relationship between the proximal gradient stepsize, $r$, and the required model decrease. 
Before stating this important lemma, we first define the proximal gradient path
\begin{equation}\label{eq:path}
p_k(r):= \Proxrphi(x_k-rg_k)-x_k \quad \text{and} \quad x_{k}(r):= x_{k}+p_k(r).
\end{equation}
We also define the quantity
\begin{equation}\label{eq:model.decrease}
    Q_k(r):=\inner{g_k}{p_k(r)}+\left(\phi(x_k(r)) - \phi(x_k)\right),
\end{equation}
which is used to measure the model decrease of the iterate $x_k(r)$.

The main descent lemma derived in \cite{Baraldi2023} plays the same role in our analysis, and we defer the proof of this lemma to maintain the focus of our exposition. We directly quote \cite[Lemma~7]{Baraldi2023} below.
\begin{lemma}
\label{lem:qk}
    The function $r \mapsto Q_k (r )$ is continuous and nonincreasing. In fact, if $r >t > 0$ then $Q_k (t) > Q_k (r )$ whenever $x_k (t) \neq x_k(r)$. Moreover, if $h_k > 0$ then
\[
Q_{k}(r)=\inner{g_k}{p_k(r)} + \left(\phi(x_k(r))-\phi(x_k)\right) \leq -\frac{1}{r}\|p_k(r)\|^2 < 0
\]
\end{lemma}

Lemma~\ref{lem:qk} is an inherent property of the proximal gradient map, which is used in \cite{Baraldi2023} to verify the conditions defining the Cauchy point
\cite[Eq.~(25)]{Baraldi2023}.
In the subsequent sections, we extend Algorithm~\ref{alg:cap} and Lemma~\ref{lem:qk} to handle the case of inexact proximity operators.



\section{Inexact Proximity Operator}
\label{sec:inexact.subgradient.proximal}
We first present a general definition of inexact proximity operators, which is motivated by the $\delta$-Fr\'{e}chet subgradient.  We will later demonstrate how to compute a $\delta$-proximity operator for the case of weighted inner products.

\begin{definition}[$\delta$-Proximity Operator]
\label{def:inexactProximal}
Let $x\in\text{dom}\,\phi$, $r>0$, and $\delta>0$ be given. We define the $\delta$-proximity operator at $x$ as the following set-valued map
\begin{align}\label{eq:inex.prox}
    \Proxrphi(x,\delta) :=  \Big\{p\in X\,\Big\vert\, &\frac{1}{2r}\|p-x\|^2+\phi(p) \nonumber \\
    &\le\frac{1}{2r}\|z-x\|^2+\phi(z)+\delta\|z-p\|\;\;\forall\,z\in X\Big\}.
\end{align}
\end{definition}

As claimed, the notion of $\delta$-proximity operator introduced in Definition~\ref{def:inexactProximal} is closely related the the $\delta$-Fr\'{e}chet subdifferential, which we define next.

\begin{definition}[$\delta$-Subgradient]
\label{def:subgradient}
    Let $x\in\text{dom}\,\phi$ and $\delta>0$ be given. We say that $s\in X$ is a $\delta$-Fr\'{e}chet subgradient, or simply a $\delta$-subgradient, of $\phi$ at $x$ if
    \[
    \phi(y)\ge \phi(x) + \inner{s}{y-x}-\delta\|y-x\|
    \]
for all $y\in X$. The set $\partial \phi_{\delta}(x)$ consists of all $\delta$-subgradient of $\phi$ at $x$.
\end{definition}

It is straightforward to observe that by setting $\delta=0$ we recover the standard definitions of subgradient and proximity operator.
By replacing the proximity operator with the inexact version defined in Definition~\ref{def:inexactProximal}, we redefine the proximal gradient path \eqref{eq:path}, and hence the Cauchy point, as
\begin{equation}
\tilde p_k(u,r):= u-x_k \quad \text{and} \quad \tilde x_{k}(u,r):= x_{k}+\tilde p_k(u,r),
\end{equation}
where $u\in \Proxrphi (x_k-rg_k,\delta)$. Analogously, we update the quantity $Q_k$ in \eqref{eq:model.decrease} to
\begin{equation}
    \tilde Q_k(u,r):=\inner{g_k}{\tilde p_k(u,r)}+\left(\phi(\tilde x_k(u,r)) - \phi(x_k)\right)
\end{equation}

We derive the close relationship between the $\delta$-subdifferntial and the $\delta$-proximity operator in Theorem~\ref{thm:delta.Prox.Thm}, but we first require the following technical lemma.
\if(0)
\begin{lemma}[Optimality Condition]
\label{lemma:optim.subg} 
The following holds for $x\in X$ and $\delta\ge 0$,
\[
  \phi(x)-\phi(y)\leq \delta \|x-y\| \quad\forall\, y\in X
  \qquad\iff\qquad
  0\in\partial_\delta \phi(x).
\]
\end{lemma}


\begin{proof}
This is a direct consequence of Definition~\ref{def:subgradient}.
\end{proof}

\begin{lemma}\label{lem:inexact.subg.prox}
Let $x,\, z \in X$ and $\delta\ge 0$. Then,
\[
  u\in z + \partial_\delta \phi(x)
  \qquad\iff\qquad
  u-z \in \partial_\delta \phi(x).
\]
\end{lemma}

\begin{proof}
We begin by observing that $u \in \partial_\delta \phi(x)+z$ if, and only if, $u=\tilde u+z$, where $\tilde u\in \partial_\delta\phi(x)$. Using Definition~\ref{def:subgradient}, the last condition is equivalent to
\begin{align*}
\phi(y)&\geq \phi(x)+\inner{\tilde u}{y-x}-\delta\|x-y\|\\
&= \phi(x)+\inner{u-z}{y-x}-\delta\|x-y\|
\end{align*}
for every $y\in X$, and this concludes the proof.
\end{proof}
\textcolor{red}{Do we need the proof of lemma 5.2? This is a result of Clason/Valkonen book? In fact, why not use the C\&V book results? 5.1 is the definition and 5.2 is trivial.}
\fi
\begin{lemma}\label{lem:composite.inexact}
Let $g:X\to\R$ be a continuously Fr\'{e}chet differentiable convex function,
\[
  H(x):= g(x) + \phi(x),
\]
and $\delta\ge 0$, then
\[
  \partial_\delta H(x) = \nabla g(x) + \partial_\delta \phi(x).
\]
Moreover, $x^*$ is a $\delta$-minimizer of $H$, i.e., $H(x^*)\le H(x) + \delta\|x-x^*\|$ for all $x\in X$, if and only if 
\[
  -\nabla g(x^*) \in \partial_\delta \phi(x^*).
\]
\end{lemma}
\begin{proof}
This is a direct consequence of \cite[Corollary 17.3]{clason2023introduction}.
%, we have
%\[
%0\in (\partial_\delta H(\cdot))(x^*) = \nabla g(x^*) + \partial_\delta\phi(x^*)
%\]
%and we conclude by applying Lemma~\ref{lem:inexact.subg.prox}.
\end{proof}
%\textcolor{red}{Do we need the proof here? It's directly from C\&V and might as well state it for nonconvex $g$.}
%It is very easy to see that in the previous lemma, if 
%\[
%-\nabla g(x^*) \in \partial_\delta \phi(x^*)
%\]
%then $x^*$ is a $\delta$-minimizer of $H(\cdot)$.

We now state and prove the main result of this section.

\begin{theorem}%[$\delta$-Prox]
\label{thm:delta.Prox.Thm}
Let $x\in X$ and $\delta\ge 0$. Then,
\[
  u\in \Proxrphi(x,\delta )
  \qquad\iff\qquad
  x \in (I+r\partial_\delta\phi)(u).
\]
\end{theorem}
\begin{proof}
Let
\(
\varphi(\cdot ) = \tfrac{1}{2r}\|\cdot -x\|^2  + \phi(\cdot ),
\)
and recall Definition~\ref{def:inexactProximal} implies $u\in \Proxrphi(x,\delta)$ satisfies 
\begin{equation}\label{eq:delta.prox.H}
    \varphi(u) \le \varphi(z) + \delta\|z-u\| \quad\forall\, z\in X
\end{equation}
i.e., $u$ is a $\delta$-minimizer of $\varphi$.
Applying Lemma~\ref{lem:composite.inexact}, expression \eqref{eq:delta.prox.H} implies
\[
-\nabla g(u)= r^{-1}(x-u)\in \partial_\delta\phi(u)
\quad \iff \quad 
x \in u+r\partial_\delta\phi(u) = (I+r\partial_\delta\phi)(u),
\]
concluding the proof.
% the last expression is equivalent to $0\in \partial_\delta(\tilde \phi(u))$. Thus
% \begin{align*}
% 0&\in \partial_\delta \tilde \phi(u) \overset{\text{Lemma }\ref{lemma:optim.subg}}= g + u-x + \partial_\delta \phi(u)
% \end{align*}
% which is equivalent, by Lemma \ref{lem:inexact.subg.prox}(2b), that
% \[
% x-u-g \in \partial_\delta \phi(u) \iff x-g \in (I+\partial_\delta\phi)(u)
% \]
% Therefore,
% \[
% u=\Prox_{\phi}(x,g,\delta ) \iff x-g \in (I+\partial_\delta\phi)(u)
% \]
\end{proof}

%It is noteworthy that when $\delta=0$, Theorem~\ref{thm:delta.Prox.Thm} reduces to the standard well-know result in the exact regime
%\[
%u=\Prox_{\phi}(x)
%\qquad\iff\qquad
%x \in (I+\partial\phi)(u).
%\]
 
The proximity operator is present in two components of Algorithm~\ref{alg:cap}, through the stationarity metric $h_k$ and in defining the Cauchy point using $Q_k$.
To ensure convergence, we require that $\delta>0$ and $u\in \Proxrphi(x_k-rg_k,\delta)$ are chosen so that the Cauchy point produces sufficient decrease.  
When using inexact proximity operators, the stationarity metric \eqref{eq:hk_exact}
becomes 
\begin{equation}
\label{eq:hk_inexact}
  \tilde h_k := \frac{1}{r_0}\|\tilde p_k(u,r_0)\|
  \qquad\text{for some}\qquad
  u\in\Proxrphi(x_k-r_0 g_k,\delta).
\end{equation}
To address the accuracy of $\tilde h_k$, we notice that the reverse triangle inequality ensures that
\[
  h_k \le \tilde h_k + |h_k-\tilde h_k|.
\] 
Consequently, by choosing $\delta>0$ so that
\begin{align}\label{eq:h.inexactness}
|h_k  -  \tilde h_k|\le \kgrad \min\{\tilde h_k,\Delta_k\},
\end{align}
holds, we ensure that
\[
  h_k \le (1+\kgrad)\tilde h_k.
\]
Hence, if the limit inferior of $\tilde h_k$ is zero, then so is the limit inferior of $h_k$.
Given the computable quantity $\tilde h_k$, we further modify the trust-region algorithm to ensure that the trial iterate $x_k^+$ satisfies
\begin{subequations}\label{eq:exact.inexact}
\begin{align}
  \| x_k^+-x_k\| &\le \krad \Delta_k \\
  m_k(x_k)-m_{k}( x_k^+) &\ge \kfcd  \tilde h_k\min\left\{\frac{\tilde  h_k}{1+\omega_k},\Delta_k\right\}.
\end{align}
\end{subequations}
Finally, we modify Assumption~\ref{assump:inexact.gradient} to account for $\tilde h_k$ as follows.

\begin{assumption}[Inexact Gradient]
\label{assump:inexact.gradient.prox}
The model $f_k: X \to \R$ has Lipschitz continuous gradient on an open set containing $\dom\, \phi$ and there exists a positive constant $\kgrad$, independent of $k$, such that
\[
\begin{aligned}
|h_k - \tilde h_k| &\le \kgrad \min\{\tilde h_k, \Delta_k\} \\
\|g_k - \nabla f(x_k)\| &\le \kgrad\min \{\tilde h_k,\Delta_k\}.
\end{aligned}
\]
\end{assumption}

With these changes we are able to produce a new version of Algorithm~\ref{alg:cap} that allows inexact computation of the proximity operator.
In particular, line~2 in Algorithm~\ref{alg:cap} is modified to {\em ``Choose $\tilde{h}_k$ and $m_k$ that satisfy Assumption~\ref{assump:inexact.gradient.prox}''}.
Notice that $\tilde h_k$ and $g_k$ must be computed in tandem to satisfy the conditions in Assumption~\ref{assump:inexact.gradient.prox}, which can be accomplished by a straight forward modification of \cite[Algorithm~4]{Baraldi2023}.
In order to ensure that the Cauchy point achieves sufficient decrease, we additionally enforce the proximal gradient descent condition
\begin{equation}\label{eq:decr.inexact}
  \tilde Q_k(u,r) \le -\frac{\kappa_{\rm dec}}{r}\|\tilde{p}_k(u,r)\|^2,
\end{equation}
where $\kappa_{\rm dec}$ is a positive constant that is independent of $k$.  Note that if $u=\Proxrphi(x_k-rg_k)$, then \eqref{eq:decr.inexact} is satisfied with $\kappa_{\rm dec}=1$ (cf.~Lemma~\ref{lem:qk}).  To demonstrate how we enforce these conditions, we restrict our attention to the case of weighted inner products.

\if(0)
\begin{algorithm}
\caption{Nonsmooth Trust-Region Algorithm: Inexact Proximal}\label{alg:cap2}
\begin{algorithmic}[1]
\Require $x_1\in \dom \psi$, $\Delta_1>0$, $0<\eta_1<\eta_2<1$, and $0<\gamma_1\leq \gamma_2 \leq \gamma_3$
%\Ensure $y = x^n$
\For{$k=1,2,\ldots$}
    \State \textbf{Inexact Prox:} Choose $\tilde h_k$ satisfying~\eqref{eq:h.inexactness} \label{alg:tilde.h.k}
    \State \textbf{Model Selection:} Choose $m_k$ that satisfies Assumption~\ref{assump:inexact.gradient.prox} \label{alg:assump.model.inexact}
    \State \textbf{Step Computation:} Compute $x_k^+\in X$ satisfying equation~\eqref{eq:exact.inexact} \label{alg:exact.inexact}
    \State \textbf{Computed Reduction:} Compute $\cred_k$ satisfying Assumption~\ref{assump:inexact.object}
    \State \textbf{Step Acceptance and Radius Update:} Compute $\rho_k$ as in \eqref{eq:rho}

    \If{$\rho_k<\eta_1$}
        \State $x_{k+1}\gets x_k$
        \State $\Delta_{k+1}\in [\gamma_1\Delta_k,\gamma_2\Delta_k]$

    \Else
        \State $x_{k+1}\gets x_k^+$
        \If{$\rho_k\in [\eta_1,\eta_2)$}
            \State $\Delta_{k+1}\in[\gamma_2\Delta_k,\Delta_k]$
        \Else
            \State $\Delta_{k+1}\in[\Delta_k,\gamma_3\Delta_k]$
        \EndIf
    \EndIf

\EndFor
\end{algorithmic}
\end{algorithm}
\fi





% To this end, we derive the following properties  of the $\delta$-proximal gradient map and $\delta$-subgradient.


% \textcolor{red}{
% \begin{enumerate}
%     \item State where the inexact prox comes into the algorithm - this would be the inexact gradient condition. 
%     \item Something to the effect of: in assumption 3.2, $h_k$ is replaced with $\tilde h_k$ (inexact prox) which takes in a tolerance $\delta$. We also require $|h_k  -  \tilde h_k|\le \kappa_{h}$. This is satisfied via \cite[Algorithm 4]{Baraldi2023}. 
% \end{enumerate}
% }





%\section{Properties of the $\delta$-Subgradient and $\delta$-Proximity Operator}
%\label{sec:properties.inexactness}




\section{Weighted Proximal Operators}
\label{sec:M.weighted.prox}
%For the remainder of the paper, we restrict our attention to the case that $X=X_M$.
%\begin{equation}\label{app.M.weighted.prox}
%\begin{aligned}
%&\Prox^M_{r \phi}(x,0,\delta) := \hdots \\
%&\left\{y:\frac{1}{2r}\|y - x\|_M^2 + \phi(y) \leq \Argmin_{z\in X}\left\{\frac{1}{2r}\|z - x\|_M^2 + \phi(z) +\delta\|z-y\|_M \right\}\right\}.
%\end{aligned}
%\end{equation}
To motivate this section, consider the finite dimensional case $X=X_M$.  When $\phi$ is separable, it is typically much easier to compute the proximity operator defined on $X_D$ (recall $D$ is a diagonal matrix), i.e.,
\[
  \Prox^D_{r \phi}(x) = \operatorname*{arg\,min}_{y\in X} \left\{\frac{1}{2r}\|y - x\|_D^2 + \phi(y)\right\},
\]
because the optimization problem defining $\Prox^D_{r\phi}(x)$ can be reduced to solving one-dimensional optimization problems for each component of $\Prox^D_{r\phi}(x)$.
For example, this is the case when $\phi(\cdot) \equiv \|\cdot\|_1$ or when the $\phi$ is the indicator function for bound constraints. 

We consider the more general setting of replacing $\Proxrphi$ with $\Proxrphi^a$ defined using the inner product induced by the bilinear form $a(\cdot,\cdot)$ and assume that $\Proxrphi^a$ has an analytical form.
To this end, we define an algorithm, listed as Algorithm~\ref{alg:inex.M.prox} that computes a $\delta$-proximity operator using $\Proxrphi^a$.
Algorithm~\ref{alg:inex.M.prox} is the usual $a$-weighted proximal gradient algorithm applied to compute $\Proxrphi(x)$ and consequently, the iterates $\{u_\ell\}$, ignoring the stopping conditions, converge strongly to $\Proxrphi(x)$ \cite[Corollary~28.9]{bauschke2017monotone}.
Notice that we employ a modified stopping condition that helps to ensure that the computed solution is a $\delta$-proximity operator.

\begin{algorithm}[htb!]
\caption{Weighted Proximal Gradient}
\begin{algorithmic}[1]
\Require{The point $x\in X$, the proximity parameter $r>0$, and $\varepsilon>0$}
\State $\ell\gets 0$
\State $u_0\gets \Prox^a_{r\phi}(x)$
%\While{$\delta < \frac{1}{r}\|(A-I)(u_\ell-u_{\ell+1})\|$}
\While{$\varepsilon < \|u_\ell-u_{\ell+1}\|_a$}
  \State{$u_{\ell+1}\gets \Prox_{r\phi}^a(u_{\ell}-A^{-1}(u_{\ell}-x))$}
  \State{$\ell\gets \ell+1$} 
\EndWhile
\end{algorithmic}
\label{alg:inex.M.prox}
\end{algorithm}


%It is worth mentioning that our algorithm requires that $D\neq M$, otherwise the search for an $\delta$ approximate to solution to the $M$-weighted proximal gradient, with $M=D$, would be possible by simply solving
%\[
%  \Prox^D_{r \phi}(x) = \operatorname*{arg\,min}_{y\in X} \left\{\frac{1}{2r}\|y - x\|_D^2 + \phi(y)\right\}.
%\]


%\textcolor{red}{Assuming conditions from v3 on $D$ and $M$ (and that $D - M$ is invertible), the d-prox is a strongly monotone operator for the $M$ inner product, which allows us to compute an error estimate between $h_k$ and $\tilde h_k$. This affects how we choose $\delta$. Relate this back to $Q_k$. }

To satisfy Assumption~\ref{assump:inexact.gradient.prox}, we must bound $|h_k-\tilde h_k|$, which we can bound in terms of the error in the $\delta$-proximity operator using the reverse triangle inequality, i.e.,
\[
  |h_k-\tilde h_k| \le r_0^{-1}\|\Proxrphi(x_k-r_0 g_k) - \tilde{x}_k(u,r_0)\|,
\]
where again $u\in\Proxrphi(x_k-r_0 g_k,\delta)$ for some $\delta > 0$.  
As we now demonstrate, Algorithm~\ref{alg:inex.M.prox} yields an element that approximates the true proximity operator, $\Proxrphi(x,\delta)$, to arbitrary precision.   For this result, we recall the definition $\varphi(\cdot):= \tfrac{1}{2r}\|\cdot-x\|^2+\phi(\cdot)$ from the proof of Theorem~\ref{thm:delta.Prox.Thm}. 
% This facilitates the analysis of our new proposed Algorithm~\ref{alg:cap2} to handle inexact proximal calculation, particularly in
% its lines \ref{alg:tilde.h.k}, \ref{alg:assump.model.inexact} and \ref{alg:exact.inexact}

%The matrices $M$ and $D$ both satisfy the basic properties of bilinear forms described in Section \ref{sec:notation}, which we use to show that there exists a $\delta$ for which we produce a $u_k$ close enough to the $\Proxphi^m$ via Algorithm~\ref{alg:inex.M.prox}. 
\begin{lemma}\label{app:lemma.tech}
Algorithm~\ref{alg:inex.M.prox} converges in finitely many iterations.  Moreover, if $\alpha_1 \le \sqrt{2}$ and Algorithm~\ref{alg:inex.M.prox} exits at iteration $\ell$, i.e., 
\begin{equation}\label{eq:lemma.tech.1}
  \|u_\ell - u_{\ell+1}\|_a \le \varepsilon,
\end{equation}
then the following error bound holds
\[
  \|u_\ell-\Proxrphi(x)\|\le \alpha_1^{-1/2}\left(1-\tfrac{1}{2}\alpha_1^{-2}\right)^{-1}\varepsilon.
\]
\end{lemma}
\begin{proof}
By \cite[Corollary~28.9]{bauschke2017monotone}, $u_\ell$ converges strongly and therefore there exists $\ell$ for which \eqref{eq:lemma.tech.1} holds for given $\epsilon>0$.
Denote the proximal gradient operator associated with the $a$-inner product by
\[
  G_a(y,t) = \tfrac{1}{t}\left(y-\Prox_{t\phi}^a\left(y-\tfrac{t}{r}A^{-1}(y-x)\right)\right)
\]
and note that $y\mapsto G_a(y,t)$ is strongly monotone for all $t\in(0,2r/\alpha_1^2)$
\cite[Lemma~2]{baraldi2024local}.
Consequently, $y\mapsto G_a(y,r)$ is strongly monotone since $\alpha_1\le\sqrt{2}$ and
\[
  a(G_a(u_\ell,r)-G_a(p,r),u_\ell-p) \ge \tfrac{1}{r}\left(1-\tfrac{1}{2}\alpha_1^{-2}\right)\|u_\ell-p\|_a,
\]
where $p=\Proxrphi(x)$.  The optimality of $p$ for $\varphi$ ensures that $G_a(p,r)=0$ and so
\[
  \tfrac{1}{r}\left(1-\tfrac{1}{2}\alpha_1^{-2}\right)\|u_\ell-p\|_a \le \|G_a(u_\ell,r)\|_a = \tfrac{1}{r}\|u_{\ell+1}-u_\ell\|_a.
\]
The result then follows from \eqref{eq:lemma.tech.1} and the equivalence of $\|\cdot\|_a$ and $\|\cdot\|$.
\end{proof}





%In the following lemma, we show that the error in the inexact proximity operator can be forced to zero under certain assumptions on the bilinear form $a$.
%One of the main steps in Algorithm~\ref{alg:cap2} the guarantee that equation~\eqref{eq:h.inexactness} holds under a finite number of steps. We prove this result in our next lemma, where we used our new subroutine, Algorithm~\ref{alg:inex.M.prox}, to 
%\begin{lemma}
%There exists $\delta>0$ such that Algorithm~\ref{alg:inex.M.prox}, with innerut $(x,g,r)=(x_{k},\nabla f_{k},r)$, yields $u_{\ell}$ satisfying equation~\eqref{eq:h.inexactness} under a finite number of iterations.
%\end{lemma}

%\begin{proof}
%    First, note that
%    \begin{align*}
%        |\tilde h_k-h_k|&=| \|\tilde u_\ell-x_k\|-\|\Proxrphi^M(x_k-rg_k)-x_k\|| \\
%        &\leq \|u_\ell-\Proxrphi^M(x_k-rg_k)\|,
%    \end{align*}
%where we applied the reverse of triangular inequality in the second line. We conclude by applying Lemma~\ref{app:lemma.tech}.
%\end{proof}

In Theorem~\ref{thm:inexact.M.prox}, we demonstrate that Algorithm~\ref{alg:inex.M.prox} applied to $x_k-r g_k$ outputs $u_{\ell+1}$ satisfying the following inequality
\[
\begin{aligned}
  \inner{g_k}{u_{\ell+1}-x_k}&+\tfrac{1}{2r}\|u_{\ell+1} - x_k\|^2 + \phi(u_{\ell+1}) \\
  &\le \inner{g_k}{z-x_k}+\frac{1}{2r}\|z - x_k\|^2 + \phi(z) +\delta\|z-u_{\ell+1}\|
\end{aligned}
\]
for every $z\in X$, or equivalently
\[
u_{\ell+1}\in \Proxrphi(x_k-rg_k,\delta). 
\]
Before presenting the main theorem of this section, we prove the following preliminary result, which we use to facilitate the proof of our main result.

\begin{lemma}\label{lem:M.weight.1}
Consider the sequence $\{u_\ell\}$ generated by Algorithm~\ref{alg:inex.M.prox}. Then,
\begin{equation}\label{eq:M.weight.1}
\frac{1}{r}(A-I)(u_\ell-u_{\ell+1}) \in \partial\varphi(u_{\ell+1}),
\end{equation}
which by definition is equivalent to
\begin{align}
\varphi(z) 
&\ge \varphi(u_{\ell+1}) + \frac{1}{r}\inner{(A-I)(u_\ell-u_{\ell+1})}{z-u_{\ell+1}}
\quad\forall\,z\in X.
\label{eq:diff}
\end{align}
\end{lemma}
\begin{proof}
Recall that $u_{\ell+1} = \Proxrphi^a(u_\ell-A^{-1}(u_\ell-x))$.
By Theorem~\ref{thm:delta.Prox.Thm}, we have that
\begin{align*}
\frac{1}{r}(u_\ell-u_{\ell+1}-A^{-1}(u_\ell-x))& \in \partial_A \phi(u_{\ell+1}) = A^{-1}\partial\phi(u_{\ell+1})
\end{align*}
and by adding $(1/r)A^{-1}(u_{\ell+1}-x)$ on both sides of the previous set inclusion (in the Minkowski sense), we obtain
\begin{align*}
\frac{1}{r}(u_\ell-u_{\ell+1}-A^{-1}(u_{\ell}-u_{\ell+1}))& \in \frac{1}{r}A^{-1}(u_{\ell+1}-x)+ A^{-1}\partial\phi(u_{\ell+1})\\
%&=D^{-1}M\partial_M\left[\frac{1}{2r}\|u_{k+1}-(x-rg)\|^2+\phi(u_{k+1}) \right]\\
&=A^{-1}\partial\varphi(u_{\ell+1}).
\end{align*}
This is equivalent to \eqref{eq:M.weight.1}, concluding the proof. 
\end{proof}

Finally, we present our main result, which shows that if $u_{\ell+1}$ satisfies the stopping conditions of Algorithm~\ref{alg:inex.M.prox}, then it is a $\delta$-proximity operator. 
\begin{theorem}\label{thm:inexact.M.prox}
If $u_{\ell+1}$ satisfies the stopping condition \eqref{eq:lemma.tech.1} with
\[
  \varepsilon \le r\delta\sqrt{\alpha_1} / (1+\alpha_2),
\]
then $u_{\ell+1}\in \Proxrphi(x,\delta)$, i.e., for all $z\in X$,
\begin{align*}
\varphi(z) + \delta \|z-u_{\ell+1}\|
&\ge \varphi(u_{\ell+1}).
\end{align*}
\end{theorem}

\begin{proof}
First note that the existence of $\alpha_1$ and $\alpha_2$ ensure that
\[
  \frac{1}{r}\|(A-I)(u_\ell-u_{\ell+1})\| \le \frac{1+\alpha_2}{r} \|u_\ell-u_{\ell+1}\| \le \frac{1+\alpha_2}{r\sqrt{\alpha_1}}\|u_\ell-u_{\ell+1}\|_a \le \frac{1+\alpha_2}{r\sqrt{\alpha_1}}\varepsilon \le \delta.
\]
Now, for any $z\in X$, we have that
\begin{align*}
\varphi(z) + \delta \|z-u_{\ell+1}\|&\ge \varphi(z) + \frac{1}{r}\|(A-I)(u_\ell-u_{\ell+1})\| \|z-u_{\ell+1}\| \\
&\ge \varphi(z) + \frac{1}{r}\inner{(A-I)(-u_\ell+u_{\ell+1})}{z-u_{\ell+1}}\\
&\ge \varphi(u_{\ell+1})
\end{align*}
where in the first line we applied the bound on $\delta$, in the second line we used the Cauchy-Schwarz inequality and for the final inequality we applied Lemma~\ref{lem:M.weight.1}.
\end{proof}





\section{Numerics}
\label{sec:numerics}

%\textcolor{blue}{1. Run Burgers control with "exact" PDE solves, but inexact L1 prox setting $kappa_grad = 1e-2, 1e-1, 1e0, 1e1, 1e2$.  Include table with iteration statistics (nfval, ngrad, nhess, nprox, etc).
%2. Run Burgers control with inexact PDE solves and L1 prox.  Include table with iteration history and objective/gradient tolerances.}

We apply our inexact weighted proximity operator within Algorithm~\ref{alg:cap} to solve optimal control of Burgers' equation:
\begin{equation}
    \min_{z\in L^2(\Omega)} \int_{\Omega}([S(z)]-w)^2(x)\dx + \frac{\alpha}{2}\int_{\Omega}z^2(x)\dx + \beta\int_{\Omega}|z|(x)\dx
\end{equation}
where $\Omega=(0,1)$ is the physical domain, $\alpha=10^{-4}$ and $\beta=10^{-2}$ are penalty parameters, $w(x)=-x^{2}$ is the target state, and $S(z)=u\in H^{1}(\Omega)$ solves the weak form of Burgers' equation
\begin{eqnarray*}
    -\nu u'' + uu' = z+f \quad \text{in } \Omega, \\
    u(0)=0, \quad u(1)=-1,
\end{eqnarray*}
where $f=2(\nu+x^3)$ and $\nu =0.08$. We discretize the state $u$ and $z$ using continuous piecewise linear finite elements on a uniform mesh with $n=512$ intervals.  To compute $S(z)$, we solve the discretized Burgers' equation using Newton's method globalized with a backtracking line search.  We exit the Newton iteration when the relative residual falls below $10^{-4}\sqrt{\epsilon_{\rm mach}}$, where $\epsilon_{\rm mach}$ is machine epsilon.  We will refer to PDE solves using this tolerance as ``exact'' PDE solves.

Given that the controls are in $L^2(\Omega)$, we employ the weighted dot product $\inner{\cdot}{\cdot}=\inner{\cdot}{\cdot}_M$, where $M\in\R^{n\times n}$ is the mass matrix and for Algorithm~\ref{alg:inex.M.prox}, we employ the dot product $a(\cdot,\cdot)=\inner{\cdot}{\cdot}_D$ weighted by the lumped mass matrix $D\in\R^{n\times n}$, i.e.,
\[
M=\frac{h}{6}\begin{pmatrix}
4 & 1 & \ldots & 0 & 0\\
1 & 4 & \ldots & 0 & 0\\
\vdots & \vdots & \ddots & \vdots &\vdots\\
0 & 0 & \ldots & 4 & 1\\
0 & 0 & \ldots & 1 & 4\\
\end{pmatrix} \in \mathbb{R}^{n\times n}\quad \text{and}\quad D=h\begin{pmatrix}
\frac{5}{6} & 0 & \ldots & 0 & 0\\
0 & 1 & \ldots & 0 & 0 \\
\vdots & \vdots & \ddots & \vdots & \vdots\\
0 & 0 & \ldots & 1 & 0 \\
0 & 0 & \ldots & 0 & \frac{5}{6} \\
\end{pmatrix}\in \mathbb{R}^{n\times n}.
\]
Recall that the $A$ operator generated by the bilinear form $a(\cdot,\cdot)$ is $M^{-1}D$. 
 For this $A$, $\alpha_1=1$ and $\alpha_2=3$.  Consequently, the preceding theory applies.
Furthermore, we approximate the $L^1$-norm by the quantity
\[
  \beta\int_\Omega |z|(x)\dx \approx \phi(z)=\beta h(\tfrac{5}{6} |z_1| + |z_2| + \ldots + |z_{n-1}| + \tfrac{5}{6}|z_n|).
\]
We notice that the $D$-weighted proximity operator of $\phi$ is the usual soft-thresholding operator
\[
  \Proxrphi^D(z) = \textup{sign}(z)\odot\max\{|z|-\beta r,0\}.
\]
\if(0)
\subsection{$L_1$-norm}
Assume that is the $L_1$-norm, i.e.,
\begin{align*}
    \phi(y):\mathbb{R}^n &\to \mathbb{R} \\
            y &\mapsto \|y\|_1:= \sum_{i=1}^{n}|y_i|
\end{align*}
where $y=(y_1,\ldots, y_n)$. Thus,
\begin{align*}
\Prox^D_{r \phi}(x) &= \Argmin_{y} \left\{\frac{1}{2r}\|y - x\|_D^2 + \phi(y)\right\} \\
&= \Argmin_{y} \left\{\frac{1}{2r}\sum_{i=1}^nd_{ii}(y_i-x_i)^2 + \sum_{i=1}^{n}|y_i|\right\} \\
&= \Argmin_{y} \left\{\sum_{i=1}^n\left[\frac{d_{ii}}{2r} (y_i-x_i)^2 + |y_i|\right]\right\} \\
& = (\ldots, \Argmin_{y_i\in \mathbb{R}} \left\{\frac{d_{ii}}{2r} (y_i-x_i)^2 + |y_i|\right\} ,\ldots )
\end{align*}

Now notice that
\begin{align*}
\Argmin \left\{ \frac{d_{ii}}{2r} (y_i-x_i)^2 + |y_i| \right\} &= \Argmin\left\{  \frac{1}{2} (y_i-x_i)^2 + \frac{r}{d_{ii}}|y_i| \right\} \\
&= \text{sign } (x_i)\max \left\{|x_i|-\frac{r}{d_{ii}} ,0\right\}
\end{align*}
\fi

In Table~\ref{tbl:1}, we summarize the performance of Algorithm~\ref{alg:cap} for different values of scaling ($\kgrad$) for the inexact gradient tolerance.
To approximately solve the trust-region subproblem \eqref{eq:tr-sub}, we employ the nonlinear conjugate gradient solver introduced in \cite[Algorithm~4]{baraldi2024efficient}.
The table includes the wallclock time in seconds ({\tt time (s)}), the number of trust-region iterations ({\tt iter}), the number of evaluations of $f$ ({\tt obj}), the number of evaluations of $\nabla f$ ({\tt grad}), the number of applications of the Hessian $\nabla^2 f$ ({\tt hess}), the number of evaluations of the proximity operator ({\tt prox}), and the average number of iterations of Algorithm~\ref{alg:inex.M.prox} ({\tt av-piter}).  As $\kgrad$ decreases, we require additional accuracy from our approximate proximity operator as computed by Algorithm~\ref{alg:inex.M.prox}.  As seen in Table~\ref{tbl:1}, our implementation of Algorithm~\ref{alg:cap} is robust to inexact proximity operators.
\begin{table}[!ht]
\centering
\begin{tabular}{l r r r r r r r}
$\kgrad$ & {\tt time (s)} & {\tt iter} & {\tt obj} & {\tt grad} & {\tt hess} & {\tt prox} & {\tt av-piter} \\
   \hline
 {\tt  1e2} & {\tt 0.4708} & {\tt 18} & {\tt 37} & {\tt 19} & {\tt 173} & {\tt 347} & {\tt  10.78} \\ 
 {\tt  1e1} & {\tt 0.4447} & {\tt 16} & {\tt 33} & {\tt 17} & {\tt 141} & {\tt 281} & {\tt  16.63} \\ 
 {\tt  1e0} & {\tt 0.5229} & {\tt 18} & {\tt 37} & {\tt 19} & {\tt 173} & {\tt 347} & {\tt  28.50} \\ 
 {\tt 1e-1} & {\tt 0.4247} & {\tt 15} & {\tt 31} & {\tt 16} & {\tt 125} & {\tt 248} & {\tt  47.07} \\ 
 {\tt 1e-2} & {\tt 0.5815} & {\tt 17} & {\tt 35} & {\tt 19} & {\tt 157} & {\tt 315} & {\tt  60.00} \\ 
 {\tt 1e-3} & {\tt 0.3498} & {\tt 13} & {\tt 27} & {\tt 15} & {\tt  93} & {\tt 183} & {\tt  53.15} \\ 
 {\tt 1e-4} & {\tt 0.4034} & {\tt 13} & {\tt 27} & {\tt 17} & {\tt  93} & {\tt 185} & {\tt  69.31} \\
 %{\tt 1e-5} & {\tt 0.5996} & {\tt 18} & {\tt 37} & {\tt 25} & {\tt 173} & {\tt 353} & {\tt 191.22} \\
 \hline
\end{tabular}
\caption{Results for the Burgers' equation for $\kgrad\in\{100,10,0.1,0.01,0.001,0.0001\}$}
\label{tbl:1}
\end{table}

To conclude, we incorporate inexact PDE solves with our inexact proximity operator computations.  In particular, we terminate the Newton iteration for solving Burgers' equation when the relative residual falls below
\[
  \min\{10^{-2},\tau\},
\]
where $\tau$ is computed by the trust-region algorithm and corresponds to the right-hand sides in Assumptions~\ref{assump:inexact.object} and \ref{assump:inexact.gradient}.  We do this fixing to $\kgrad=1$ and choosing $\kobj=10^3$.  Since the dominant cost of Newton's method is the linear system solves at each iteration, we compare the average number of linear system solves per iteration between our runs with exact and inexact PDE solves.  In particular, our method averaged 5.3125 linear system solves per trust-region iteration when using inexact PDE solves, compared with 7.7222 linear system solves when using exact PDE solves.  The reduction in linear system solves is a byproduct of our relaxed tolerances.  In particular, many of the PDE solves only require the relative residual to be smaller than $10^{-2}$.


\section{Conclusion and Future Work}

In this work, we introduced an inexact proximity operator---motivated by the $\delta$-Fr\'{e}chet subdifferential---for use within the inexact trust-region algorithm from \cite{Baraldi2023}.  Additionally, we extended the inexact trust-region algorithm, Algorithm~\ref{alg:cap}, from \cite{Baraldi2023}, to leverage our inexact proximity operator. Our numerical results suggest that our algorithm is robust to inexact proximity operator evaluations.
As future research, we hope to develop similar theory that extends beyond the weighted proximity operator problem studied here.





==> data/appendices.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Spring 2021.  
%
%
%  Author: Thesis Office
%  
%  Last Updated: 1/13/2021
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{appendices}
\titleformat{\chapter}{\centering\normalsize}{APPENDIX \thechapter}{0em}{\vskip .5\baselineskip\centering}
\renewcommand{\appendixname}{APPENDIX}

\input{data/appendix1}
\input{data/appendix2}

\end{appendices}

==> data/dedication.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Spring 2021.  
%
%
%  Author: Thesis Office
%  
%  Last Updated: 1/13/2021
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           DEDICATION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter*{DEDICATION}
\addcontentsline{toc}{chapter}{DEDICATION}  % Needs to be set to part, so the TOC doesnt add 'CHAPTER ' prefix in the TOC.



\begin{center}
\vspace*{\fill}
To my mother, father, grandfather, and grandmother. I'm filling in more space so that this extends to the next line. 
\vspace*{\fill}
\end{center}

\pagebreak{}


==> data/nomenclature.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Spring 2021.  
%
%
%  Author: Thesis Office
% 
%  Last Updated: 1/13/2021
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           NOMENCLATURE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter*{NOMENCLATURE}
\addcontentsline{toc}{chapter}{NOMENCLATURE}  % Needs to be set to part, so the TOC doesnt add 'CHAPTER ' prefix in the TOC.

%A note about aligning: These entries will align
%themselves according to the ampersand (&).
%No extra spaces are needed, as seen in some of
%the entries below.

%Example of the longtable environment.
\hspace*{-1.25in}
\vspace{12pt}
\begin{spacing}{1.0}
	\begin{longtable}[htbp]{@{}p{0.35\textwidth} p{0.62\textwidth}@{}}
	   % \begin{tabular}{@{}p{0.33\textwidth} p{0.62\textwidth}@{}}
		OGAPS	&	Office of Graduate and Professional Studies at Texas A\&M University\\	[2ex]
		B/CS		&	Bryan and College Station\\	[2ex] %[2ex] provides double space between each row
		TAMU			&	Texas A\&M University\\	[2ex]
		SDCC & San Diego Comic-Con\\ [2ex]
		EVIL & Every Villain is Lemons\\ [2ex]
		EPCC & Educator Preparation and Certification Center at Texas A\&M University - San Antonio\\ [2ex]
		FFT & Fast Fourier Transform\\ [2ex]
		ARIMA & Autoregressive Integrated Moving Average\\ [2ex]
		SSD & Solid State Drive\\ [2ex]
		HDD & Hard Disk Drive\\ [2ex]
		O\&M & Eller Oceanography and Meteorology Building\\ [2ex]
		DOS & Disk Operating System\\ [2ex]
		HDMI & High Definition Multimedia Interface\\ [2ex]
		$L^1$ & Space of absolutely Lebesgue integrable functions; i.e., $\int |f| < \infty$\\ [2ex]
		$L^2$ & Space of square-Lebesgue-integrable functions, i.e., $\int |f|^2 < \infty$\\ [2ex]
		$PC(S)$ & Space of piecewise-continuous functions on $S$\\ [2ex]
		GNU & GNU is Not Unix\\ [2ex]
		GUI & Graphical User Interface\\ [2ex]
		PID & Principal Integral Domain\\ [2ex]
		MIP & Mixed Integer Program\\ [2ex]
		LP & Linear Program\\ [2ex]
		%XXXXXXXX		&	This is an optional page. Random word to test how long the sentence can be? This is just for test purpose. The current setting aims to align left/right margin same as all other pages.\\	[2ex]
	   % \end{tabular}%
	\end{longtable}
\end{spacing}

\pagebreak{}

==> data/section1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Spring 2021.  
%
%
%  Author: Thesis Office
%  
%  Last Updated: 1/13/2021
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           SECTION I
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\pagestyle{plain} % No headers, just page numbers
\pagenumbering{arabic} % Arabic numerals
\setcounter{page}{1}


\chapter{\uppercase {Introduction and Literature Review}}

\section{Author's Message to the Student Using This Template For Their Thesis or Dissertation}

Howdy! This is the template for theses and dissertations written using \LaTeX for submission at Texas A\&M University. The Graduate and Professional School (GPS) is here to guide you in submitting your thesis or dissertation and can help you with questions about that process. This template shows the many features of \LaTeX, with many more available to the user.

There are numerous guides, references, and tutorials available on the Internet to help you. If you are stuck, don't be afraid to Google your issue, or you can contact Overleaf at welcome@overleaf.com. If you have questions about submitting or processing your document you can email the Thesis Office at thesis@tamu.edu


\subsection{Brief Usage of the Template}

This template is intended for use by STEM\footnote{Science, Technology, Engineering, and Mathematics. This is an example of a footnote. You can see that it is numbered and appended at the end of the page. Also, you can see the effect of having a multiline footnote.} students. If you are not a STEM student, this template is likely not for you.If you are not familiar with LaTeX, now is not the best time to learn.

The advantage of using this template over the Microsoft Word templates are numerous. First, there is a lot of control granted to the user in how the document looks. Of course, you are expected to still follow the guidelines set forth in the TAMU Thesis Manual. This template takes care of the margins, heading requirements, and orders the front matter for you.


\subsection*{Software to Install}

\textbf{MikTeX} or \textbf{ProTeXt} is the free software recommended for Windows PC users to
compile your \LaTeX ~ document. To compile for this document, XeLaTeX compiling engine
is used. There is currently an issue in which the package xetex-def does not install; see the file README.txt for a solution. Another software called \textbf{JabRef} is also recommended for bibliography/reference management; its usage is similar with EndNote.

\subsection*{Procedure to Compile \LaTeX ~ Document}

This template (and consequently, your document) will be compiled using XeLaTeX. To compile your document, do the following\footnote{Notice here that I also show off the itemize environment for unordered lists. Ordered lists use the enumerate environment.}:

\begin{itemize}
	\item In TeXstudio, go to the Tools menu, then select Commands, and click XeLaTeX.
	
	\item In Texmaker, go to the Tools menu and select XeLaTeX.
	
	\item For other editors, consult the help files included with the editor.
\end{itemize}

To view the output after the program is done compiling, press F7 in TeXstudio and TeXmaker or the appropriate hotkey for other editors. Be sure that the document is not open in another PDF reader, for your editor will not display it.

\subsection{How to Fill This Document}
The document structure is organized in the main .tex file, TAMUTemplate.tex,
which has the same name as the output PDF file. Content in each section is in the data folder. You can open the .tex files under the data folder to modify. Four sections
are added initially. To add in more sections into the \LaTeX document, open the
TAMUTemplate.tex file and go to \textbf{line 130} you can just delete the content in the data folder and fill your documents and then compile under TAMUTemplate.tex.)

\subsection{Reference Usage and Example}

Here we test the usage of references. The book\cite{REALCAR} 
is referred in this way. Actually, the option is available for you to change the default way how reference appears. The default and most commonly used option \cite{einstein} is displayed here \cite{Barn-JORVQ}.Both of these options are acceptable. 

Unrelated citations are referred here for the test of reference section only\cite{TAMU}. If you
find that the reference \cite{GIGEM} has more items than you need \cite{WAGFJ}, question marks will show up in place of a reference handle, like these \cite{Over9000}.

\subsection{Equations, Formulas, and Other Really Cool Math Things That \LaTeX ~ Can Do}

Equations can be written in \LaTeX ~ in one of two ways. First, you can have material displayed inline by enclosing the desired statement in dollar signs. For example, $e^{i\pi}+1=0$ is an inline math expression. Some longer expressions, especially those including sums, integrals, or large operators and objects can be displayed centered on their own line. In this \textbf{math mode}, you enclose the desired material in square brackets. For example,

\[ \sum_{j = 1} ^n \int f_j \ dx = \int \sum_{j = 1} ^n f_j \ dx \]
is a math mode expression. We can also have a series of expressions aligned at a symbol. This is particularly useful when you are showing details in solving an equation or evaluating an integral. The next block shows off the \textit{align*} environment. We use it here to show a distributive property of set intersections over unions. Observe how each line is aligned to the biconditional symbol. This makes reading steps easier, since a reader can go line by line and determine why each step is justified.

\begin{align*}
x \in A \cap \bigcup_{j} B_j &\iff x \in A \ \wedge \ x \in \bigcup_{j} B_j \\
&\iff x \in A \ \wedge \ x \in B_k \ \text{ for some k} \\
&\iff x \in \bigcup_{j} A \cap B_j
\end{align*}

There are many more commands and features available, but this document is too small to contain them.\footnote{Yes, I pulled a Fermat. But really, a Google search will likely help you find what you need to do.} Many guides are available on the Internet for your use.

%Have some material about the align environments. Include also the eqn environment.

\subsection{A Test Section}

This is just a test.This is what a subsection looks like. Below is a figure displaying some Haskell code in a compiler.

\begin{figure}[!ht]
\centering
	\includegraphics[scale=0.26]{Haskell1.jpg}
	\caption{Some Haskell code in a compiler.}
\end{figure}

This template has been designed for use in modern systems, but can perhaps be adapted to work on older systems, such as Windows 95. Below is a screenshot of a DOSBox console, an MS-DOS emulator designed to work on several platforms. Windows 95 can be installed into DOSBox, but it is not suggested.

\begin{figure}[ht!]
\centering
	\includegraphics[scale=0.55]{DOSBox1.jpg}
	\caption{The DOSBox console running in Windows 7. The contents of the mounted directory C: are displayed, with the active subdirectory DUKE3D.}
\end{figure}

\section{Specifications in This TAMU \LaTeX ~ Template}

All requirements for theses can be found in the most recent version of the Thesis Manual, available at the GPS website. The Thesis Office will be happy to assist you if you have questions about specific formatting. Questions specific to \LaTeX\ should be directed to \texttt{welcome@overleaf.com}.

 A copyright statement at the beginning of a section with reprinted material from a previously printed source is required. The screenshot below describes how to achieve this. Check the instruction files for more details.

\begin{figure}[ht!]
\centering
	\includegraphics[scale=0.65]{Footnote.png}
	\caption{The inclusion of a copyright statement as a footnote. The lines in yellow help to change to footnote marking scheme.}
\end{figure}

\subsection{Another Test Section}
There should be things here.

%\begin{algorithm}
%Stuff.
%\end{algorithm}

\subsubsection{Test}
Hello, is it me you're looking for?

\subsubsection{Test 2}
There are more things to do.

\subsection{Yet Another One}
 We insert a slew of figures in the remainder of the document to test the look of the List of Figures.

\begin{figure}[H]
	\centering
	\includegraphics[width=4.25in]{Mint_XFCE.png}
	\caption{Linux Mint 13 with the XFCE desktop environment.}
\end{figure}

These are more figures.

\begin{figure}[H]
	\centering
	\includegraphics[scale=0.45]{TOC2.png}
	\singlespace
	\caption{The ``Table of Contents" dialog box in Microsoft Word. This must be accessed to properly generate the Table of Contents when using the Recommended Template.}
\end{figure}

Yet another figure follows - the last for this section.

\begin{figure}[H]
	\centering
	\includegraphics[width=3.75in]{Rachl3.png}
	\singlespace
	\caption{Linear regression on three (top) and four (bottom) independent variables in base R.}
\end{figure}
 
 \subsection{No Surprises Here}
 Insert another song lyric here.



==> data/section2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Spring 2021.  
%
%
%  Author: Thesis Office
%  
%  Last Updated: 1/13/2021
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%                           SECTION II
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\chapter{PAGES WITH A FIGURE, A TABLE AND AN EQUATION}
\section{Figures: Placement, Size, and Captions}
This is a figure template.
\begin{figure}[ht]
\centering
\includegraphics[scale=0.75]{TAMUthesis_CMD_windows.png}
\caption[The command line compiler in Windows.]{The command line compiler in Windows. It is not suggested that you compile using this method. See compilation instructions in the README.}

\label{fig:CMD_1}

\end{figure}

Figure (and table) titles should be consistent through the document. All captions should be placed either above or below the object it describes. This is done by placing the \textit{caption} in the correct place. While continued figures are allowed by the Thesis Manual, it is not suggested that any continued figures be included in a \LaTeX\ document. The figure below is from Linux Mint, showing a portion of a desktop.

\begin{figure}[H]
	\centering
	\includegraphics[width = 5.75in]{Desktop.png}
	\caption{A typical desktop space in Linux Mint.}
\end{figure}

The figure below is taken from R. While there are packages available to import graphics from R, MATLAB, and similar software, it is probably best to export plots generated by these programs as a PNG file, and then import it via the \textit{includegraphics} command.

\begin{figure}[H]
	\centering
	\includegraphics[scale=0.55]{UnemDiffACF.png}
	\singlespace
	\caption{The autocorrelation function (ACF) of the differenced unemployment series. Seasonal adjustments may be needed.}
\end{figure}

It is suggested that you scale the figures so they fit within the margins. Almost all the figures included in this document for the sake of example have been scaled. It is best to use PNG and JPEG files as figures.

The last figure here is a screenshot from the Linux terminal.

\begin{figure}[H]
	\centering
	\includegraphics[width=4.75in]{Terminal1.png}
	\caption{The Linux terminal. The commands shown are from a two-dimensional mesh generator that triangulates a domain in the plane. Files containing nodes, elements, the polygon, and the edges are created.}
\end{figure}

\section{Table Placement, Size and Table Title}

Here is a table, displaying band and auxiliary scores from the 2011 Arcadia Festival of Bands held in Arcadia, CA \cite{ARCADIA}.

\begin{table}[h!]
	\centering

	\label{Band}
	\begin{tabular}{|l|l|l|}
		\hline
		School Name & Band Score & Auxiliary Score \\ \hline
		Rancho Bernardo & 96.15 & 89.15 \\ \hline
		Mt. Carmel & 95.30 & 83.55 \\ \hline
		Riverside King & 93.85 & 91.75 \\ \hline
		Diamond Bar & 93.20 & 88.60 \\ \hline
		El Dorado & 92.80 & 95.45 \\ \hline
		Chino & 92.65 & 91.45 \\ \hline
		Henry J. Kaiser & 92.60 & 87.55 \\ \hline
		Glendora & 92.60 & 89.15 \\ \hline
		Montebello & 90.50 & 82.70 \\ \hline
		Mira Mesa & 89.65 & 91.50 \\ \hline
	\end{tabular}
	\caption{Scores from the 2011 Arcadia Festival of Bands.}
\end{table}

The table is sorted by band score. There is more text here to demonstrate how the template handles spacing between tables and body text. Also note how the table caption is in a smaller font size than the body text.Text in the captions and appendices can be no smaller than size 7.

\section{Equations}

The following format is recommended to be used to display equations.

%Make other examples.
\begin{equation} \label{Equ.2.1}
y=c_1\cos(t)+c_2\sin(t)
\end{equation}
\begin{equation} \label{Equ.2.2}
e^{it}=\cos(t)+i\sin(t)
\end{equation}

Equation \ref{Equ.2.1} is the general solution to the differential equation $y''+y=0$. In the source code, the \textit{ref} command allows you to refer to an equation by a label you created. References must be made after the equation has been created; attempting to refer to an equation before it is defined results in a question mark placeholder. Some more sample equations are below. Notice the first set below is not numbered.
%%
\begin{align*}
\log (x^n) &= \log (x \cdot x \cdot \ldots \cdot x) \\
&= \log x + \log x + \ldots + \log x \\
&= n \log x
\end{align*}
\begin{equation} \label{Equ.2.3}
X^T X \mathbf{u} = X^T \mathbf{y}
\end{equation}
\begin{equation}\label{Equ.2.4}
u(x, t) = \int_{-\infty}^{\infty} G(x, \tau) \exp\left(-\frac{(t-\tau)^2}{4kt}\right) \ d\tau
\end{equation}
\begin{gather}
\mathcal{L}(f) = \int_{0}^{\infty} e^{-st} f(t) \ dt \\
\begin{split} \label{Equ.2.5}
\mathcal{F}(f) = \frac{1}{2\pi}\int_{-\infty}^{\infty} e^{i \omega x} f(x) \ dx
\end{split}
\end{gather}

You can use labels to refer to equations you create. \ref{Equ.2.5} is the \textbf{Laplace transform} used extensively in differential equations. \ref{Equ.2.3} is the matrix representation of the \textbf{normal equations} used in least-squares regression.

To have equations without labels appearing the right margin, simply add an asterisk to the name of the environment (equation, align, etc.) when making the declaration.


\section{Theorems and Proofs: Examples}

This section will show an example usage of the theorem and proof environments, typically used for mathematics students. To use these environments, you must have the package \textbf{amsthm} declared in the preamble of your document. For this template, this is already declared in the main file. You may choose to remove this declaration if your document will not make use of theorems and proofs.

Theorems can be numbered, as the one below is, or you can force a different label to appear. For example, you can state the Bolzano-Weierstass theorem and have the names appear as the theorem label. See the examples below.

Sometimes you may have a theorem with multiple parts or multiple conditions. You can use other list environments, such as enumerate, inside the theorem environment declared to list these conditions. The final example at the end of this block shows this with the Invertible Matrix Theorem, which has several equivalent statements.

\newtheorem{thm}{Theorem}
\begin{thm}
	Suppose $f$ is of class $\mathcal{C}^1$ and $g$ is of class $\mathcal{C}^2$, and that the compact set $D$ and its boundary satisfy the hypotheses of Green's Theorem.  Then
	\[ \iint \limits_D f\nabla^2 g \ dA = \oint_{\partial D} f(\nabla g) \cdot \mathbf{n} \ ds - \iint \limits_D \nabla f \cdot \nabla g \ dA . \]
\end{thm}

\begin{proof}
	Begin with the integral of $f\nabla g \cdot n$ taken over the boundary of D.  By the second vector form of Green's Theorem,
	\begin{align*}
	\oint_{\partial D} f\nabla g \cdot n \ ds &= \iint \limits_D \nabla \cdot (f\nabla g) \ dA \\
	&= \iint \limits_D f\nabla^2 g + \nabla f \cdot \nabla g \ dA.
	\end{align*}
	
	Rearranging yields the desired.
\end{proof}

\begin{thm}[Bolzano-Weierstrass]
	Every bounded real sequence has a convergent subsequence.
\end{thm}

\begin{thm}[Invertible Matrix Theorem\footnote{This is an incomplete list.}]
	For any square matrix $A$ with $n$ rows and columns, the following are equivalent.
	\begin{enumerate}
		\item $A$ is invertible.
		\item The equation $A\mathbf{x}=\mathbf{0}$ has only the trivial solution $\mathbf{x} = \mathbf{0}.$
		\item For any nonzero $\mathbf{b}, \ A\mathbf{x} = \mathbf{b}$ has exactly one solution.
		\item The columns of $A$ form a linearly independent set.
		\item Zero is not an eigenvalue of $A$.
		\item $A$ has full rank.
		\item The determinant of $A$ is not zero.
	\end{enumerate}
\end{thm}

There is currently no set format on how propositions and theorems should be laid out in the document. The idea is to remain consistent. It is best to not customize the appearance of theorems so that they can easily be distinguished from body text - just like figures, tables, and headings.

\section{Another Table Example}
For the sake of testing the appearance of the list of tables, a second table will be displayed here. This table displays a list of some major universities and their enrollments during fall 2015. This table is sorted in descending order of enrollment.
%The savenotes environment, loaded from the footnote package
%(which in turn is loaded from mdwtools)
%allows you to use footnotes in tables, if needed.
\begin{savenotes}
\begin{table}[h!]
	\centering
	\label{my-label}
	\begin{tabular}{|l|l|l|}
		\hline
		School & City and State & Fall 2015 Enrollment  \\ \hline
		Texas A\&M University\footnote{Gig 'em!} & College Station, TX & 64,376  \\ \hline
		Ohio State University\footnote{This number describes enrollments at the Columbus campus; enrollments at regional campuses in Lima, Mansfield, Marion, Newark, and Wooster are not counted.} & Columbus, OH & 58,322 \\ \hline
		Iowa State University & Ames, IA & 36,001 \\ \hline
		University of California, San Diego & La Jolla, CA & 33,735   \\ \hline
		University of West Florida & Pensacola, FL & 12,798 \\ \hline
		Massachusetts Institute of Technology & Cambridge, MA & 11,319   \\ \hline
	\end{tabular}
	\caption{Some major universities and their fall 2015 enrollments.}
\end{table}
\end{savenotes}

Naturally, tables and footnotes do not go together. If you attempted to write a footnote inside a table, there will be nothing at the bottom of the page, yet the footnote marker will still appear. To remedy this, the \textit{footnote} package has been loaded from the \textit{mdwtools} package. Check your TeX distribution to see if \textit{mdwtools} is installed. See the source code for how this is implemented.

Here are some blank floats.

\begin{figure}[!h]
	\caption{A blank float.}
\end{figure}

\begin{figure}[!h]
	\caption{Another blank float.}
\end{figure}

==> data/section3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Spring 2021.  
%
%
%  Author: Thesis Office
%  
%  Last Updated: 1/13/2021
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           SECTION III
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter{VERY, VERY, VERY LONG TITLE THAT FLOWS INTO A SECOND LINE FOR THE SAKE OF EXAMPLE}

Notice that the title of this section is long - much longer than the others. When you have long section titles, this template takes care of double spacing the lines in the title. If the title is long to fit in the table of contents, the template will single space the title.

\section{Yet Another Table}

Another table is placed here to show the effect of having tables in multiple sections. The list of tables should still double space between table titles, while single spacing long table titles.

%Fix table labeling.
\begin{table}[h!]
	\centering
	\begin{tabular}{|l|l|}
		\hline
		Dates & Attendance  \\ \hline
		August 8-10, 2008 & 3,523  \\ \hline
		August 14-16, 2009 & 4,003 \\ \hline
		July 9-11, 2010 & 5,049 \\ \hline
		August 5-7, 2011 & 6,891  \\ \hline
		August 10-12, 2012 & 9,464  \\ \hline
		August 16-18, 2013 & 11,077  \\ \hline
		July 18-20, 2014 & 14,686 \\ \hline
		July 31-August 2, 2015 & 18,411  \\ \hline
	\end{tabular}
	\caption{San Japan attendance. Data is taken from \cite{ANCONS}. I intentionally make the title of this table long so the single space effect is seen in the list of tables.}
\end{table}

You may be wondering why San Japan was chosen. There are a few reasons as to why I did this:

\begin{enumerate}
\item It is one of the fastest-growing anime conventions in Texas.
\item Filler.
\item I wanted a good variety of table examples.
\item Because conventions are cool.
\end{enumerate}

The \textit{enumerate} environment was used to generated an ordered list above.

\section{Section Test Example}
We insert another figure here, just for kicks.

\begin{figure}[h!]
	\centering
	\includegraphics[width = 6.0in]{LowPass_Filter_Design.png}
	\caption{A low pass filter design.}
\end{figure}

\subsection{Filler, Filler, Filler}

This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document.

\begin{figure}[h!]
	\centering
	\includegraphics[width=3.75in]{Workspace1.png}
	\caption{A typical Texmaker workspace in Windows 7. The right sidebar displays the current file's structure according to the subsections in place.}
\end{figure}

This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document.

\begin{figure}[h!]
	\centering
	\includegraphics[width=3.5in]{Rachl1.png}
	\caption{Some commands in R.}
\end{figure}

\subsection{Subsection Test Example}
Test subsection for TOC display

\subsection{Subsection Test Example 2}
This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document.

\begin{figure}[h!]
	\centering
	\includegraphics[scale=0.85]{TAM_Logo1.png}
	\caption{The logo of a familiar university.}
\end{figure}

\begin{figure}[!h]
	\caption{Yet another blank float that has no purpose. This is only to test the appearance of the Lists of Figures and the List of Tables.}
\end{figure}

\subsection{Section Summary}
  
This holds the summary. Well, not really a summary - there was a lot of filler in this section.

\begin{figure}[h!]
	\centering
	\includegraphics[width=6.5in]{Filter1.png}
	\caption{A signal and the result after a basic filter. The FFT was used to create the plot on the right.}
\end{figure}

\section{Section Test Example 3}
Test section for toc display only.

\begin{figure}[!h]
	\caption{There is nothing to see here.}
\end{figure}

\begin{figure}[!h]
	\caption{There is another float here. I wonder what could be here? Guess what? Nothing! There is no material in this float.}
\end{figure}

\subsection{Subsection Test 1}
Test subsection for toc display only.

\subsection{Subsection Test 2}
Test subsection for toc display only.

==> data/section4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Spring 2021.  
%
%
%  Author: Thesis Office
%  
%  Last Updated: 1/13/2021
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           SECTION IV
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\chapter{SUMMARY AND CONCLUSIONS \label{cha:Summary}}

The summary goes here, along with your conclusions. The title of this final chapter/section must contain the words ``summary'' or ``conclusions.''

Here, I attempt to fill the section with more figures, possibly more tables. The inclusion of these floats is to manipulate the list of figures and list of tables in order to see when the inconsistent spacing begins. It is important to remember that any images you wish to use are placed in the appropriate directory inside the folder in which the project is kept. In the original template, all the images used as figures here are placed in the subdirectory \textit{graphics}, as declared in the preamble of \textit{TAMUTemplate.tex}. If you wish to use any other directories, be sure to declare them in the preamble of \textit{TAMUTemplate.tex}. See the figure below on how to declare directories.

\begin{figure}[h!]
	\centering
	\includegraphics[scale=0.95]{GraphicDir.png}
	\caption{Declaring graphics directories.}
\end{figure}

This version of the template now has a section to place any packages that you are using - see the figure below.

\begin{figure}[!h]
	\centering
	\includegraphics[scale=0.95]{CustomPackage.png}
	\caption{The place to declare any packages you require that I have not already declared. This simplifies debugging.}
\end{figure}

More figures will be inserted, with some text between them.

\begin{figure}[!h]
	\centering
	\includegraphics[scale=0.85]{CartesianCoordinate.png}
	\caption{Two points on the unit circle and their corresponding position vectors.}
\end{figure}

This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document.

\begin{figure}[!h]
	\centering
	\includegraphics[width=4.25in]{CompileChange.png}
	\caption{Changing the method of compilation for XeLaTeX in TeXstudio.}
\end{figure}

This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document.

\begin{figure}[!h]
	\centering
	\includegraphics[width = 4.825in]{Changelog.png}
	\caption{A portion of the changelog in the README for this document. This is located in the root directory.}
\end{figure}

This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document.

This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document. This section has filler text. These words serve no meaning except to fill a few lines in the document.

\section{Challenges}
Section here is to test toc display only.

\section{Further Study}
Section here is to test toc display only.



==> def_Renato.tex <==
% % Set left margin - The default is 1 inch, so the following
% % command sets a 1.25-inch left margin.
% %\setlength{\oddsidemargin}{0.25in}
% %\oddsidemargin .15cm
% %\evensidemargin .15cm
% \oddsidemargin .5cm
% \evensidemargin .5cm

% % Set width of the text - What is left will be the right margin.
% % In this case, right margin is 8.5in - 1.25in - 6in = 1.25in.
% \setlength{\textwidth}{6.0in}
% %\textwidth 16.5cm

% % Set top margin - The default is 1 inch, so the following
% % command sets a 0.75-inch top margin.
% %\setlength{\topmargin}{-0.25in}
% \topmargin 0.5cm

% % Set height of the header
% \setlength{\headheight}{.5cm}

% % Set vertical distance between the header and the text
% \setlength{\headsep}{0.5cm}

% % Set height of the text
% \setlength{\textheight}{22.5cm}

% % Set vertical distance between the text and the
% % bottom of footer
% \setlength{\footskip}{0.4in}

\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{latexsym}
\usepackage{amssymb}
\usepackage{framed}
%\usepackage{algorithm,algorithmic}

\newtheorem{thm}{Theorem}[section]
%\newtheorem{theorem}{Theorem}[section]
\newtheorem{theorem}[thm]{Theorem}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{corollary}[thm]{Corollary}
\newtheorem{definition}[thm]{Definition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{example}[thm]{Example}
\newtheorem{rem}[thm]{Remark}
\newtheorem{remark}[thm]{Remark}
\newtheorem{problem}[thm]{Problem}
\newtheorem{question}[thm]{Question}
\newtheorem{exercise}[thm]{Exercise}
\newtheorem{application}[thm]{Application}
\newtheorem{observation}[thm]{Observation}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\beqas}{\begin{eqnarray*}}
\newcommand{\eeqas}{\end{eqnarray*}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
% \newcommand{\bal}{\begin{align}}
% \newcommand{\eal}{\end{align}}
% \newcommand{\bals}{\begin{align*}}
% \newcommand{\eals}{\end{align*}}
\newcommand{\gap}{\hspace*{2em}}
\newcommand{\sgap}{\hspace*{1em}}
\newcommand{\vgap}{\vspace{.1in}}
\newcommand{\nn}{\nonumber}
\newcommand{\bRe}{\bar \Re}
\newcommand{\IR}{\makebox{\sf I \hspace{-9.5 pt} R \hspace{-7.0pt} }}
\newcommand{\defeq}{\stackrel{\triangle}{=}}
\newcommand{\Ik}{{\mathcal{I}}_k}
\newcommand{\Ikprime}{{\mathcal{I}}_{k'}}
\setcounter{page}{1}
\def\eqnok#1{(\ref{#1})}
\def\proof{\noindent{\textit{Proof}}: \ignorespaces}
\def\remark{\par{\it Remark}: \ignorespaces}
\def\endproof{{\ \hfill\hbox{%
      \vrule width1.0ex height1.0ex
    }\parfillskip 0pt}\par}
\def\endremark{{\ \hfill\hbox{%
      \vrule width1.0ex height1.0ex
    }\parfillskip 0pt}\par}

\newcommand{\tos}{\rightrightarrows}
\newcommand{\R}{\mathbb{R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cX}{{\cal X}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cZ}{{\cal Z}}
\newcommand{\Z}{{\cal Z}}
\newcommand{\lam}{{\lambda}}
\newcommand{\blam}{{\bar \lambda}}
\newcommand{\A}{{\cal A}}
\newcommand{\tA}{{\tilde A}}
\newcommand{\tC}{{\tilde C}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cK}{{\cal K}}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\ind}[1]{I_{#1}}
\newcommand{\inds}[1]{I^*_{#1}}
\newcommand{\supp}[1]{\sigma_{#1}}
\newcommand{\supps}[1]{\sigma^*_{#1}}
\newcommand{\simplex}[1]{\Delta_{#1}}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\Si}[1]{{\cal S}^{#1}}
\newcommand{\Sip}[1]{{\cal S}^{#1}_{+}}
\newcommand{\Sipp}[1]{{\cal S}^{#1}_{++}}
\newcommand{\inner}[2]{\langle #1,#2\rangle}
\newcommand{\Inner}[2]{\big \langle #1\,,#2 \big \rangle}

\newcommand{\ttheta}{{\tilde \theta}}
\newcommand{\cl}{\mathrm{cl}\,}
\newcommand{\co}{\mathrm{co}\,}
\newcommand{\argmin}{\mathrm{argmin}\,}
\newcommand{\cco}{{\overline{\co}}\,}
\newcommand{\ri}{\mathrm{ri}\,}
\newcommand{\inte}{\mathrm{int}\,}
\newcommand{\interior}{\mathrm{int}\,}
\newcommand{\bd}{\mathrm{bd}\,}
\newcommand{\rbd}{\mathrm{rbd}\,}
\newcommand{\cone}{\mathrm{cone}\,}
\newcommand{\aff}{\mathrm{aff}\,}
\newcommand{\lin}{\mathrm{lin}\,}
\newcommand{\lineal}{\mathrm{lineal}\,}
\newcommand{\epi}{\mathrm{epi}\,}
\newcommand{\sepi}{\mbox{\rm epi}_s\,}
\newcommand{\dom}{\mathrm{dom}\,}
\newcommand{\Dom}{\mathrm{Dom}\,}
\newcommand{\Argmin}{\mathrm{Argmin}\,}
\newcommand{\lsc}{\mathrm{lsc}\,}
\newcommand{\di}{\mbox{\rm dim}\,}
\newcommand{\EConv}[1]{\mbox{\rm E-Conv}(\Re^{#1})}
\newcommand{\EConc}[1]{\mbox{\rm E-Conc}(\Re^{#1})}
\newcommand{\Conv}[1]{\mbox{\rm Conv}(\R^{#1})}
\newcommand{\mConv}[1]{\overline{\mbox{\rm Conv}}_\mu\,(\R^{#1})}
\newcommand{\cball}[2]{\mbox{$\bar {\it B}$}(#1;#2)}
\newcommand{\oball}[2]{\mbox{\it B}(#1;#2)}
\newcommand*{\E}{\mathbb{E}}
\newcommand{\expect}[1]{\E\left[#1\right]}
\newcommand{\cexpect}[2]{\E_{#2}\left[#1\right]}
%\newcommand{\Subl}[2]{{\cal L}_{\le #1}(#2)}
%\newcommand{\sSubl}[2]{{\cal L}_{< #1}(#2)}
\newcommand{\Subl}[2]{{#2}^{-1}[-\infty,#1]}
\newcommand{\sSubl}[2]{{#2}^{-1}[-\infty,#1)}
\newcommand{\bConv}[1]{\overline{\mbox{\rm Conv}}\,(\R^{#1})}
\newcommand{\bEConv}[1]{\mbox{\rm E-C}\overline{\mbox{\rm onv}}\,(\Re^{#1})}
\newcommand{\asympt}[1]{{#1}'_{\infty}}
\newcommand{\sym}[1]{{\cal S}^{#1}}
\newcommand{\spa}{\,:\,}
\newcommand{\barco}{\overline{\mbox{co}}\,}
\newcommand{\tx}{\tilde x}
\newcommand{\ty}{\tilde y}
\newcommand{\tT}{\tilde T}
\newcommand{\tz}{\tilde z}
\newcommand{\tu}{\tilde u}
\newcommand{\tq}{\tilde q}
\newcommand{\tv}{\tilde v}
%\newcommand{\th}{\tilde h}
\newcommand{\tf}{\tilde f}
\newcommand{\psis}{\psi_s}
\newcommand{\psin}{\psi_n}
\newcommand{\ts}{\tilde\sigma}
\newcommand{\tgamma}{\tilde \gamma}
\newcommand{\la}{\langle\,}
\newcommand{\ra}{\,\rangle}
\def\iff{\Leftrightarrow}
\def\solution{\noindent{\bf Solution}. \ignorespaces}
\def\endsolution{{\ \hfill\hbox{%
      \vrule width1.0ex height1.0ex
          }\parfillskip 0pt}\par}
\def\NN{{\mathbb{N}}}



